Dynamical instabilities in disc-planet interactions

Protoplanetary discs may become dynamically unstable due to structure induced by an embedded giant planet. In this thesis, I discuss the stability of such systems and explore the consequence of instability on planetary migration. I begin with non-self-gravitating, low viscosity discs and show that giant planets induce shocks inside its co-orbital region, leading to a profile unstable to vortex formation around a potential vorticity minimum. This instability is commonly known as the vortex or Rossby wave instability. Vortex-planet interaction lead to episodic phases of migration, which can be understood in the framework of type III migration. I then examine the effect of disc self-gravity on gap stability. The linear theory of the Rossby wave instability is extended to include disc gravity, which shows that self-gravity is effective at stabilising the vortex instability at small azimuthal wavenumber. This is consistent with the observation that more vortices develop with increasing disc mass in hydrodynamic simulations. Vortices in self-gravitating discs also resist merging, and is most simply understood as pair-vortices undergoing mutual horsehoe turns upon encounter. I show that in sufficiently massive discs vortex modes are suppressed. Instead, global spiral instabilities develop which are associated with a potential vorticity maximum at the gap edge. These edge modes can be physically understood as a result of unstable interaction between the gap edge and the exterior disc through gravity. I show the spiral arms can provide a positive torque on the planet, leading to fast migration outwards. I confirm the above results, obtained from razor-thin disc models, persist in three-dimensions.

==> Chapter1/rings2.tex <==
%\chapter{Ring structures in disc-planet interactions}\label{rings}
%\ifpdf
%    \graphicspath{{Rings/Figs/PNG/}{Rings/Figs/PDF/}{Rings/Figs/}}
%\else
     \graphicspath{{Rings/Figs/EPS/}{Rings/Figs/}}
%\fi
\section{Basic equations and model}\label{modeleq}
We consider a planet of mass $M_p$ orbiting a central star 
of mass $M_*.$  We adopt a cylindrical coordinate system $(r,\theta,z)$
where $z$ is the vertical coordinate increasing in the direction normal to the disc plane
for which the unit vector is ${\hat{\bf k}}.$ 
The governing hydrodynamic equations
in a frame uniformly rotating with angular velocity $\Omega_p{\hat{\bf k}}$ are the continuity 
equation
\begin{align}\label{continuity}
\frac{D\Sigma}{Dt}=-\Sigma\nabla\cdot\mathbf{v},
\end{align}
and the equation of motion
\begin{align}\label{momentum}
\frac{D\mathbf{v}}{Dt}+2\Omega_p\hat{\mathbf{k}}\wedge\mathbf{v} = 
-\frac{1}{\Sigma}\nabla P - \nabla\Phi_{\mathrm{eff}},
\end{align}
where $D/Dt$ is the total derivative, the vertically integrated pressure  $P=c_s(r)^2\Sigma$ with
$c_s=h(GM_*/r)^{1/2}.$ 
Here $\Sigma$ is the surface density, ${\bf v}$ is the velocity and the effective
gravitational and centrifugal  potential is
given by
\begin{align}
\Phi_{\mathrm{eff}} = -\frac{GM_*}{r} - \frac{GM_p}{\sqrt{r^2+r_p^2+2rr_p\cos(\theta-\theta_p)+\epsilon^2}}-\frac{1}{2}\Omega_p^2r^2.
\end{align}
Here the cylindrical coordinates of the planet are $(r_p,\theta_p,0)$
 and the  softening length $\epsilon = 0.6hr_p$
 with  $h$ being the disc aspect ratio.\\
 
 \subsection {Vortensity conservation}\label{secvort}
The vortensity  being the ratio of the  $z$ component of the  vorticity  (hereafter just  called the vorticity)
 to the surface density is
defined to be 
\begin{equation}\label{vortensity}
\eta =  \frac{\omega}{\Sigma} \equiv \frac{\omega_r+2\Omega_p}{\Sigma},
\end{equation}
where $\omega_r=\hat{\mathbf{z}}\cdot\nabla\wedge\mathbf{v}$ is the relative
vorticity seen in the rotating frame.
 It is well known that In barotropic flows without shocks,
it follows from (\ref{continuity}) and (\ref{momentum}) that the  vortensity
$\eta = \omega/\Sigma$  is
conserved for a  fluid particle. 
When an isothermal equation of state with variable sound speed as is used 
here is adopted, vortensity is no longer strictly conserved.
However, the sound speed varies on a global scale
so that  when   phenomena are considered on a local scale,  vortensity is 
 conserved to a good approximation in the absence of shocks.

\section{Ring structures in disc-planet interactions}\label{rings} 
In this section we  present hydrodynamic simulations to
show that narrow  surface density rings are brought about as  a consequence
of the fact that highly peaked 
vortensity  ( being the ratio of the vorticity to the surface density) 
 rings are produced by flow through quasi-steady shocks
located close to  the planet. For
sufficiently massive planets, the associated vortensity generation occurs as fluid
elements execute a horse-shoe turn in the coorbital region. 
Focusing on such
cases, we construct  a simple model that enables an estimate of the shock
location to be made together with rate of the vortensity
generation as material flows through it. Our model is in good agreement with
numerical simulations and confirms the process of
vortensity generation within a planet's co-orbital region  which later
plays an important role in modifying  the flow structure there. 
\subsection{Hydrodynamic simulations}\label{sec2}
For convenience we adopt dimensionless units such that the initial
orbital radius of the planet is $r_p=2.$ In these units the 
the radial computation domain  for the simulations described in this
section is  $r=[1,3]$.
The disc  has an  initially uniform surface density $\Sigma=\Sigma_0.$ 
%Boundary conditions corresponding to outgoing waves were adopted.
We remark that
ring formation occurs as a result of  shocks near the planet and therefore is
unaffected by boundary conditions. 
 For the simulations described in this section the planet is held fixed
 on its initial circular orbit   with Keplerian angular velocity
$\Omega_p=\sqrt{GM_*/r_p^3}$ which also defines the rotation of the coordinate system.  Time is expressed in units
of the orbital period $2\pi/\Omega_p$ defines the dimensionless time we aopt. 
The planet mass is increased gradually from zero such that it attains its full
value after  five orbital periods.\\
\indent We use the FARGO code to solve for the disc response
\citep{masset00a,masset00b}. FARGO evolves the hydrodynamic
equations in global cylindrical co-ordinates centred on the central
object. We used a non-rotating frame for the simulations described
here. Indirect terms arising from the non-inertial frame is included
in the potential. The code uses a finite-difference scheme with van Leer upwind
and hence is second-order accurate in space, similar to the
ZEUS code \citep{stone92} but it employs a modified algorithm for
azimuthal transport that allows for large time steps. 
We take $2\pi$-periodic boundary condition in
the azimuth and wave damping boundary conditions at disc boundaries
\citep{valborro06}. 

%% The planet moves under the disc, primary and
%%  indirect potentials and its motion integrated with a 5th order
%%  Runge-Kutta method. \\
%% \section{Numerical setup}\label{numerics}
%%  \indent The system of interest consists of a planet orbiting a central
%%  star in thin disc. We use polar co-ordinates $(r,\phi)$ centred on the
%%  primary in a non-rotating frame (unless otherwise stated). Units are such that the gravitational
%%  constant $G=1$ and primary mass $M_*=1$, then the Keplerian
%%  orbital period at $r=1$ is $2\pi$. The two-dimensional hydrodynamic
%%  equations read 
%%  \begin{align}\label{hydro_equations}
%%  &\frac{\p\Sigma}{\p t} + \nabla\cdot(\Sigma\mathbf{v})=0,\\
%%  & \frac{\p v_r}{\p t} +\mathbf{v}\cdot\nabla
%%   v_r-\frac{v_\phi^2}{r}=-\frac{1}{\Sigma}\frac{\p P}{\p
%%     r}-\frac{\p\Phi}{\p r}+\frac{f_r}{\Sigma},\\
%%   &\frac{\p v_\phi}{\p t} +\mathbf{v}\cdot\nabla
%%   v_\phi+\frac{v_\phi v_r}{r}=-\frac{1}{\Sigma r}\frac{\p P}{\p
%%     \phi}-\frac{1}{r}\frac{\p\Phi}{\p\phi}+\frac{f_r}{\Sigma},
%%  \end{align}
%%  where $\Sigma$ is the disc surface density, $\mathbf{v}=(v_r,v_\phi)$ the
%%  fluid velocity and $P$ the vertically integrated pressure. We
%%  adopt a locally isothermal (non-barotropic) equation of state
%%  \begin{align}\label{eq_of_state}
%%  P=c_s^2(r)\Sigma.
%%  \end{align}
%%  The sound speed is $c_s=hv_k$ where $h=H/r$ is the constant
%%  aspect ratio and $v_k=r^{-1/2}$ is the Keplerian speed. 
%%  $\Phi$ is the total potential including primary,
%%  planet (with softening length $\epsilon=0.6H$) and indirect
%%  terms. Disc self-gravity is not included in the 
%%  calculation. $f_r$ and $f_\phi$ are viscous forces proportional
%%  to the uniform kinematic viscosity $\nu=\nu_0\times10^{-5}$.
%%  Details of the two source terms can be found in \cite{masset02}.\\
% \subsection{Disc and planet}
% \indent Our fiducial disc extends from $r=0.4-4.0$ and has initially
% uniform density $\Sigma=\Sigma_0\times10^{-4}$, azimuthal
% velocity is then $v_\phi=v_k\sqrt{1-h^2}$ and $v_r=-3\nu/2r$ (i.e. the
% standard accretion disc). The planet has fixed mass
% $M_p=2.8\times10^{-4}$, corresponding to Saturn if $M_*$ is
% the Solar mass, initially placed in circular Keplerian orbit at
% $r_p=2$, where the orbital period is $P_0=2\pi\times2^{3/2}$ and is
% our unit of time. The full planet potential is applied from $t=0$.\\
% \indent We choose $\Sigma_0=7.0$ based on preliminary simulations (see
% below) in order to achieve rapid migration when $\nu_0=1.0$ (a typical
% value used in such studies, e.g. \cite{masset03,valborro07}). However,
% this report will focus on inviscid discs with $\nu_0=0$; although numerical
% viscosity is needed for shocks. Excluding self-gravity
% is not well-justified as the Toomre parameter $Q=\kappa c_s/\pi
% G\Sigma\sim 5.6 $ at $r=2$. The current setup allows
% relatively high resolution simulations and one to focus on the
% disc-planet aspect, but self-gravity is an important issue that needs to
% be included for consistent studies of Type III migration.


*****{`\bf some references to code....softening..convergence..etc...}***********
 
\subsection{ Vortensity generation by the shocks 
induced by a Saturn mass planet}\label{fiducial}
\indent We first consider  case with $M_p=2.8\times10^{-4}M_*$ corresponding
to a Saturn mass planet around a solar mass star.
 For these calculations the
resolution was $N_r\times N_\phi=1024\times3072$,  corresponding to 
grid radial and azimuthal grid spacings of   $\Delta r\simeq
0.02r_h$ and $r\Delta\phi\simeq0.05r_h$ respectively, where
$r_h$ is the planet's Hill radius in dimensionless units.

 Fig.\ref{vortxy_020} shows the vortensity field at
$t=7.07$ close to the planet. Vortensity is
generated/destroyed as material passes through the two spiral shocks.
 For the outer shock, vortensity
generation occurs for fluid elements executing a
horse-shoe turn ($|r-r_p|\lesssim r_h$) while  vortensity is reduced for
fluid that passes by the planet.  But the change is smaller in magnitude
in the latter case.
 The
situation is similar for the inner shock, but some post-shock material
with increased vortensity continues to pass by the planet. This stream begins at
$r\simeq -r_h$ but such feature is absent at the outer
shock,suggesting a lack of symmetry about $r=r_p$, possibily resulting from
the non-uniform vortensity background being $\propto r^{-3/2}$.
  Note that although a pre-shock fluid element that would be  on a horse-shoe trajectory,
may in fact pass by the planet after crossing the shock, it is
clear that vortensity rings originate from passage through shock fronts interior
to the  co-orbital  region that would correspond to the horseshoe region
for free particle motion.

 The streams of high vortensity eventually move around the whole orbit outlining the
entire co-orbital region. Fig. \ref{vortxy_020} shows  that they are generated
along a small  part of the shock front  with length  $l\sim r_h$. This  results in
thin rings with  a similar  radial width.
The fact that they originate from horse-shoe
material can  enhance the contrast  as post-shock
inner disc horse-shoe material is mapped  from $r-x$ to  $r+x$ 
to become
adjacent to post-shock   outer disc material passing by the planet.

\begin{figure}
\center
\includegraphics[scale=0.5]{vortxy_020b.ps}\caption{Vortensity
generation and destruction across shocks induced by a Saturn-mass
planet in an inviscid disc. The plot shows log(vortensity) $=\log{\omega/\Sigma}$.
Regions of increased vortensity are clearly visible as half horseshoes
above and below the planet. The increase occurs as material passes through
parts of the shock fronts that extend  into  the coorbital region.}
\label{vortxy_020} 
\end{figure}
\begin{figure}
\center
\includegraphics[scale=0.4]{coorb_plot_0.ps}\caption{Long-term
  evolution of co-orbital properties for a Saturn-mass planet held on
  fixed orbit. Vorticity, density and vortensity 
  perturbations are expressed   relative to their  values at $t=0$.} \label{coorb_plot_0}
\end{figure}

{\bf brief discussion of long term behaviour of co-orbital
  vortensity/vorticity/density}

\subsection{ Location of the  vortensity generation region for different planet masses}
\indent The process of  formation of vortensity rings discussed 
 here differs from  that observed
in \cite{koller03} and \cite{li05}, where the rings are generated by shocks outside
the co-orbital region. This is because the authors used a
smaller planet mass. 
To illustrate  the effect of reducing the mass, we ran low resolution
simulations ($N_r\times N_\phi = 256\times768$) for $M_p\times10^{4}=1,\,2.8$ and
$10$. Fig. \ref{compare2_020} compares azimuthally averaged
vortensity perturbations induced in each case after $14.14$ orbits. 
The intermediate and high mass cases are
qualitatively similar, having $\Delta(\omega/\Sigma)$ maxima at
$r-r_p\sim\pm 2r_h$ and minima at $r-r_p\sim3 r_h$. The magnitude of
$\Delta(\omega/\Sigma)$ increases with $M_p$ because higher masses
induce 
 higher Mach number shocks. As the half-width of the horseshoe region
is $2.5 r_h$
 for such masses (refs), vortensity rings
are co-orbital features.
\begin{figure}
\center
\includegraphics[scale=0.4]{compare2_020.ps}\caption{Azimuthally averaged vortensity
  perturbation for different planet masses.} \label{compare2_020}
\end{figure}
The low mass $M_p=10^{-4}$ case has much smaller
$|\Delta(\omega/\Sigma)|$. There is a vortensity maximum at $r-r_p=-3r_h$
but nothing of similar magnitude at $r-r_p>0$. 
 \cite{paardekooper09}
found the co-orbital half-width, in the limit of zero softening
for low mass planets, to be:
\begin{align}
x_s=1.68(M_p/h)^{1/2}r_p.
\end{align}
For $M_p=10^{-4},\,h=0.05$, $x_s=2.33r_h$. For
non-zero softening, the actual $x_s$ is smaller. Hence, vortensity
rings for low mass planets occur outside the  co-orbital region as is
confirmed in our simulations and they are very much weaker. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% HIGH RESOLUTION RESULTS FOR VORTENSITY GENERATION V.S. M_P
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \delta m = -5\times10^{-5} for M_p = 10^{-4}
%% \delta m = -2\times10^{-4} for M_p = 2.8\times10^{-4}
%% \delta m = +5\times10^{-4} for M_p = 10^{-3}
%% the 1d vortensity plot is very similar to low resolution case (picture
%% at /data/stardisk/mkl23/hyades/vorticity/compare2_040.ps). in the
%% above, only radial derivative part of voriticy is used. the low
%% resolution stuff presented above used full expression for
%% vorticity, there is little difference between the two. low
%% resolution was needed to examine long term evolution/equilibrium
\subsection{ A semi-analytic model for coorbital 
vortensity generation by shocks}\label{model}
\indent We now  construct a semi-analytic model describing the process of
shock-generation of vortensity.  In this way we gain an understanding
of the physical processes involved and later how they lead to 
strong torques and fast migration of the planet and under what conditions
simulations  can represent them acurately.

More specifically we model the outer
spiral shock in Fig. \ref{vortxy_020}. To do this we need the  pre-shock flow field,  the shock front
location  and then to evaluate the vortensity change undergone  by
material as it passes through the shock.
We now consider these in detail 

\subsection{Flow field}
\indent We first simplify the geometry by adopting the shearing box
approximation \cite[e.g.][]{paardekooper09}. As we are concerned with
the flow near the planet, we consider a local Cartesian co-ordinate
system $(x,y)$ co-rotating with the planet at angular
speed $\Omega_p$ and with origin at its centre of mass. Without the planet, the velocity field is
Keplerian $\mathbf{v}=(0,-3\Omega_p x/2)$. 
In order to deal with the pre-shock flow we make the assumption that pressure effects can be ignored
 compared to planet potential.  This ballistic  approximation is appropriate for 
 a slowly varying  supersonic flow as is expected to be appropriate for the pre-shock
 fluid. The   velocity $\mathbf{v}$  satisfies the local form of
 equation ( \ref{momentum} ) with  $P=0$ and the effective
 potential
 \begin{align}
\Phi_{\mathrm{eff}} =  - \frac{GM_p}{\sqrt{x^2+y^2+\epsilon^2}}-\frac{3}{2}\Omega_p^2x^2
\end{align}
and thus follows from particle dynamics.
We write a fluid particle's trajectory in a steady state flow  in the form
 as  $ x=x(y)$ and the corresponding velocity field
 as $\mathbf{v}=\mathbf{v}(y).$
 Noting that  on a particle trajectory we have 
 $\frac{D}{Dt}=v_y\frac{d}{dy}$,  it follows from the local form of (\ref{momentum}) 
 that on a  particle trajectory we have the following system of three simultaineous
 first order differential equations:
\begin{align}
\label{semi-an}\frac{dv_y^2}{dy}&=-4\Omega_pv_x-\frac{2M_py}{(x^2+y^2+\epsilon^2)^{3/2}}= Q,\\
\frac{d}{dy}\left(v_xv_y^2\right)&=v_xQ+2\Omega_pv_y^2 
+v_y\left[3\Omega_p^2x-\frac{M_px}{(x^2+y^2+\epsilon^2)^{3/2}}\right],\\
\frac{d}{dy}\left(xv_y^2\right)&=xQ+v_xv_y.
\label {semi-an1}\end{align}
We  use these to solve for the state vector
$\mathbf{U}(y)=[v_y^2,\,v_xv_y^2,\,xv_y^2]$ in $x>0$ for a particular
particle. The boundary condition is 
\begin{align}
(v_y,\, v_x,\, x)\to(-3\Omega_p x_0/2, \, 0, \, x_0) \,\,\mathrm{as}\,\,
y\to\infty , 
\end{align}
where $x_0$ is the particle's unperturbed path. 
The totality of paths obtained by considering a continuous range of $x_0$
then constitutes the flow field.  Having obtained the velocity field, we 
use  vortensity conservation to obtain $\Sigma$. The density is then
\begin{equation}
\Sigma(x,y) = \frac{2\Sigma_0}{\Omega_p}(\omega_r+2\Omega_p),
\end{equation}
where the unperturbed absolute vorticity is
$\omega_r =\Omega_p/2.$  Numerically, we
calculated the relative vorticity  by relating it to the circulation through 
\begin{equation}
\omega_r\simeq\frac{1}{\Delta A}\oint\mathbf{v}\cdot\mathbf{dl}
\end{equation}
where the integration is taken over a closed loop about the point of
interest and $\Delta A$ is the enclosed area. This avoids
errors due to  numerical
differentiation on the uneven grid in $(x,y)$  generated by solving the above system.
\subsection{Location of the shock front}
\indent The physical reason for shock formation is the fact that the
planet presents an obstacle to the flow. Where the relative flow is subsonic,  the
presence of this obstacle can be communicated to the fluid via sound
waves emitted by the planet. In regions where the relative flow is supersonic,  the fluid is unaware
of the planet via sound waves (but  the planet's
gravity is felt).  We estimate the location of the boundary separating these two regions
by  specifying an appropriate characteristic curve or ray defining a sound wave.  
This is a natural location for shocks. Applying this
idea to Keplerian flow, \cite{papaloizou04} obtained a good match
between the predicted theoretical shock front and the wakes associated with a low mass
planet. For general velocity field $\mathbf{v}$, the characteristic
curves satisfy the equation 
\begin{align}\label{shock_front}
\frac{dy_s}{dx} =
\frac{\hat{v}_y^2-1}{\hat{v}_x\hat{v}_y-\sqrt{\hat{v}_x^2+\hat{v}_y^2-1}},
\end{align}
where $\hat{v}_i= v_i/c_s$. The  positive sign of the square root
has been chosen so that the curves have negative slope
in the domain $x>0$   with $v_y<0.$  As the fluid flows
from super-sonic ($y>y_s$) to sub-sonic ($y<y_s$), fluid located at 
 $y=y_s$  begins
to know about the planet through pressure waves \citep{papaloizou04}. In
Keplerian flow, the rays defining the shock fronts originate from the  sonic points at
$x=\pm2H/3,\,y=0$. In a  general flow,  sonic points where  ($|\mathbf{v}|=c_s$),
at which the rays may start,
lie on  curves and can occur for $x<2hr_p/3$.  The starting
sonic point for   solving  Eq. ( \ref{shock_front}) that we eventually  adopted has
 $x=0$ and the value of  $y >0$ that is furthest possible
from the planet.
\subsection{Vorticity and vortensity changes across a shock}
\indent The jump in absolute vorticity $[\omega]$ is readily obtained by
resolving the fluid motion parallel and perpendicular to the shock
front  \citep[eg.][]{kevlahan97}. As we do not solve the energy equation,
and shocks are locally  isothermal our expression differs from
those of  \citet{kevlahan97}   accordingly a brief derivation of $[\omega]$ is
presented in  Appendix B. The result for a steady shock is
\begin{align}\label{vorticity_jump}
[\omega]=-\frac{(M^2-1)^2}{M^2}\frac{\p v_\perp}{\p S}+(M^2-1)\omega
-\left(\frac{M^2-1}{v_\perp}\right)\frac{\p c_s^2}{\p S},
\end{align}
where $v_\perp$ is the pre-shock  velocity perpendicular to the
 $M=v_\perp/c_s$ is perpendicular Mach number
and $c_s=hr^{-1/2}$ is the sound speed. $\p/\p S$ is derivative
along the shock. It is  important to note that for (\ref{vorticity_jump}) to hold,
 the direction of increasing $S,$ the direction of positive  $v_{\perp},$
 and the vertical direction should form
a right handed triad.
The local
isothermal equation of state produces the last term on RHS of
Eq. (\ref{vorticity_jump}). Because of the slow variation of $c$  
its contribution is not important in this application. \\ 
\indent The vortensity jump $[\omega/\Sigma]$ follows immediately from
Eq. (\ref{vorticity_jump}) as
\begin{align}\label{vortensity_jump}
\left[\frac{\omega}{\Sigma}\right]=-\frac{(M^2-1)^2}{\Sigma M^4}\frac{\p
  v_\perp}{\p S}-\left(\frac{M^2-1}{\Sigma M^2v_\perp}\right)\frac{\p c_s^2}{\p S},
\end{align}
which reduces to the expression derived by \cite{li05} if
$c_s=\mathrm{constant}$. The sign of  $[\omega/\Sigma]$ depends mainly on the gradient of
$v_\perp$ (or $M$) along the shock. As in our case  $v_\perp<0,$ the width of the  increased vortensity
rings produced is determined by  the length along the shock where $|M|$ is
increasing.  %% . Since $v_\perp<0$, increasing
%% shock strength along it implies vortensity generation.
Note that $[\omega/\Sigma]$ does not depend explicity on the  pre-shock vortensity,
unlike the absolute vorticity jump.


\subsection{Comparison of the results of the semi-analytic model with numerical simulations}
 We  now compare the results of hydrodynamic simulations
with those obtained from the model.  
 First we illustrate the particle paths that constitute
 the flow field together with the  shock
fronts obtained by assuming coincidence with the characteristic curves
that are obtained from the semi-analytic model 
in Fig. \ref{shock_curve2_}.
A polynomial fit to the simulation shock front is also
shown.
 Particle paths cross for $x > r_h,\,y < -2r_h$
 so  that the neglect of pressure becomes invalid.  Accordingly  the
solution to equation(\ref{shock_front})  should not be trusted in this
region.  Fortunately, vortensity generation occurs at a distance from the planet that is  within 
$1-1.5r_h$, where pre-shock particle paths do not cross.\\
\begin{figure}
\center
\includegraphics[scale=0.4]{shock_curve2_.ps}\caption{Solid lines: particle paths from the reduced zero-pressure
momentum equations (equations \ref{semi-an} - \ref{semi-an1}); thick lines: curves composed of sonic points
 on which $|\mathbf{v}|=c_s$;
dotted lines: theoretical shock fronts; dash-dot line: solution to equation ( \ref{shock_front}) for Keplerian flow; dashed line: 
polynomial fit to simulation shock front. The actual shock front begins  at a sonic point 
around $x=0.2r_h.$}
\label{shock_curve2_}
\end{figure}
%%
\indent The key quantity  determining vortensity generation is the
perpendicular Mach number. Fig. \ref{sc3_machsq_020} compares $M$ from
simulation and model.  Although the semi-analytic model gives a shock  Mach number
that is somewhat smaller than found from the simulation, all curves have $|M|$
increasing from $x=0\to 1.3r_h$ which is the important domain for vortensity
generation.  Thus  equation(\ref{vortensity_jump})
 implies  vortensity generation in all cases. Note that in the significant domain
  $x \in [0\to 1.3r_h]$ the Mach numbers deviate by less than 50\%.
\begin{figure}
\center
\includegraphics[scale=0.4]{sc3_machsq_020.ps}\caption{Perpendicular
  Mach number $M$ along the outer spiral shock  illustrated in
  Fig. \ref{vortxy_020}. Asterisks: simulation data; dotted line:  Mach number obtained 
  from the simulation shock
  and the semi-analytic flow; solid line: Mach number 
  obtained from the  semi-analytic shock front and flow.}
\label{sc3_machsq_020}
\end{figure}
%%
 In Fig. \ref{mp2.8} we illustrate various  combinations of
semi-analytic modeling  and simulation data that have been used to
estimate the  vortensity jump
across the shock.
 The qualitative   quantitative similarities  
 between the various curves confirms that the
vortensity generation  occurs  within the Hill sphere in coorbital
material that is shocked as it undergoes horseshoe turns.
 
 Assuming that material is mapped from $x\to -x$ as it switches to
the inner leg of its horse-shoe orbit,  we expect the outer spiral
shock to produce a vortensity ring peaked at $r-r_p\sim -0.5r_h$ of
width $O(r_h)$ ($=O(H)$), with a similar discussion
applying to the inner shock which is expected to produce
a vortensity ring peaked at $r-r_p\sim 0.5r_h$ . Thus,
thin vortensity rings are natural features of the co-orbital
region.

 We have  also tested our model for $M_p=2\times10^{-4}$ in
Fig. \ref{mp2}.  In this case there is still  a good qualitative 
match between the simulation and  the model.
This   is the case even though  lowering $M_p$  makes  the zero-pressure
approximation, adopted to determine the semi-analytic flow field, less good. 
Decreasing $M_p$ shifts vortensity generation
away from the planet in the semi-analytic model, as  is also observed in 
the hydrodynamic simulation
(Fig. \ref{compare2_020}). In this case, there is no vortensity
generation in $r-r_p<0.5r_h$ but vortensity rings are are still
co-orbital ( with  peaks at $\sim0.7r_h$).\\ 
We remark that steep
vortensity gradients are associated with 
dynamical instabilities \citep[e.g.][]{papaloizou85} and this is
explored in more detail below. 
\begin{figure}
\center
\subfigure[\label{mp2.8}]{\includegraphics[scale=0.4]{vort_jump1}}
\subfigure[\label{mp2}]{\includegraphics[scale=0.4]{vort_jump2}}
\caption{Semi-analytic  and actual vortensity jumps across a shock in the
  co-orbital region. Asterisks are measured from the simulations. The
  dashed lines were obtained by using pre-shock simulation data coupled
  with the jump condition  specified by equation( \ref{vortensity_jump}). The  dotted lines 
  were obtained using the semi-analytic flow field together with
  the location of the  shock front obtained from the simulation.  The  solid
  curves  correspond to the semi-analytic model for both the flow field and shock front.}\label{vort_jump}
\end{figure}
%%
%\begin{figure}
%\center
%\subfigure[$M_p=2.8\times10^{-4}$]{\includegraphics[scale=.33]{jump_machsq_lin.ps}}
%\subfigure[$M_p=2\times10^{-4}$\label{jump_machsq_lin_m2}]{\includegraphics[scale=.33]{jump_machsq_lin_m2.ps}}
%\caption{$M^2$ along the outer spiral shock (horizontal axis is $x$
  %co-ordinate along shock). Solid line is measured from simulation,
  %with the dashed curve as a polynomial fit, and dotted line is the
  %linear model.\label{jump_mach_lin}}
%\end{figure}
%\begin{figure}[!h]
%\center
%\subfigure[$M_p=2.8\times10^{-4}$]{\includegraphics[scale=.33]{jump_vortensity_lin.ps}}
%\subfigure[$M_p=2\times10^{-4}$]{\includegraphics[scale=.33]{jump_vortensity_lin_m2.ps}}
%\caption{Vortensity jump across outer spiral shock. Asterisks are measured
  %from simulation, solid line is expected jump given pre-shock data
  %from simulation and using the analytic jump expression, dotted curve
  %is prediction from linear model.\label{jump_vortensity_lin}}
%\end{figure}
\subsection{Azimuthally averaged  vortensity profile}
 Here we use our semi-analytic shearing
box model to  estimate the azimuthally averaged vortensity
profile. In order to
make progress we make the following simplifying 
assumptions:
\begin{enumerate}
\item Vortensity is only changed across the shock and conserved
  elsewhere ( see section \ref{secvort}). 
\item Symmetric spiral shocks. We assume $[\omega/\Sigma]$ for $x<0$
  (inner spiral shock) is the 
 same as for the outer spiral shock.  This is consistent with
  the shearing-box approximation. 
\item We use the shearing box model desccribed above   to
  obtain $[\omega/\Sigma]$, then apply the implied 
change to the background vortensity
  profile of the global model, being given by 
 $\omega_0=r^{-3/2}/2\Sigma_0.$
\end{enumerate}
\indent We note in Fig. \ref{mp2.8}, the horizontal axis corresponds
to the $x$-coordinate of the shock front. A fluid element which shocks
at a particular 
 $x$ originated from a location $(x_0,\,y>0).$   For $x_0 <
x_s\equiv2.5r_h$  the trajectory  starts 
 on a horseshoe orbit. We assume the shock
does not change this  so that such particles are mapped to
$-x_0$ after it executing  the horseshoe turn. 
Such particles   
experience $[\omega/\Sigma]>0$ so that the inner vortensity ring is
attributed to the outer spiral shock and the outer ring to the inner
spiral shock  as is  observed in
simulations (see Fig. \ref{vortxy_020}).
 Particles with $x_0>x_s$ continue to circulate after the
shock. Both librating and circulating particles can be re-shocked so
we expect the vortensity peaks and troughs to increase
 in amplitude to some extent. Eventually after a few returns
the system may approach a steady state for which 
${\partial v_{\perp}}/{\partial S}\rightarrow 0$
However, 
we shall not investigate this in detail  here
but  simply consider  the initial ring formation as a result
of the first shocking. 


Our procedure is as follows. The post-shock vortensity of a
particle originating from $x_0>0,y>0$ is
\begin{align}
\left(\frac{\omega}{\Sigma}\right)_{x} =
\left(\frac{\omega_0}{\Sigma_0}\right)_{x_0}
 +\left[\frac{\omega}{\Sigma}\right]_{x}. 
\end{align}
 If the location where the particle is shocked
  satisfies  $x < x_s$ it
will be located at $(-x_0,\,|y/r_h|\gg1)$ after it executes a horseshoe turn.
If $x >x_s$ it continues to circulate and  will be located at
$(x_0,\,y<0)$. Thus,
\begin{align}
\left(\frac{\omega}{\Sigma}\right)_{x} = \left\{ 
\begin{array}{l l}
  \left(\omega/\Sigma\right)_{-x_0} & \quad \mbox{$x_0<x_s$}\\
  \left(\omega/\Sigma\right)_{x_0} & \quad \mbox{$x_0>x_s$.}\\
\end{array} \right.
\end{align}
A similar argument is applied to the inner shock. 
 We
then transform to the global cylindrical co-ordinates  using $x_0\to x_0 +
r_p$. 

 The vortensity profile for $M_p=2.8\times10^{-4}$ obtained from the
semi-analytic model
is shown in Fig. \ref{sc3_vort1d_v4}. The central region
corresponds to particles whose vortensity is not modified by shocks.
However, strictly  speaking 
the  vortensity distribution changes because particles switch between
$r_p\pm x_0$ conserving  their vortensity and the background 
(unperturbed) vortensity
distribution 
is non-uniform. This is a minor effect that is expected to lead to
a uniiform distribution due
to phase mixing. To deal with  this,
     we adopt the simple procedure of replacing the
vortensity  everywhere in this region with the 
unperturbed  vortensity at the planet's location,
$r_p^{-3/2}/2\Sigma_0$. 
Fig. \ref{sc3_vort1d_v4}  shows that we expect sharp
vortensity rings adjacent to the planet, with troughs exterior to
them.

 In Fig. \ref{vort1d_temporary} we compare the the semi-analytic
results   to the
simulation data, the snapshot being chosen  at the  point when  the rings 
first occupy the complete 
azimuth. The semi-analytic  model reproduces the essential features, 
for example
vortensity peaks and troughs with the  correct relative positions, but 
the distribution is 
slightly shifted towards the planet  
(by $0.2r_h$).
The model does not reproduce  the troughs very well  due to
inadequate modelling of the  pre-shock flow and the shock position. 
\begin{figure}
\center
\includegraphics[trim=0cm 0cm 0cm 1cm,clip,scale=0.33]{sc3_vort1d_.ps}\caption{Theoretical
Shock-modifed vortensity distribution near a
  $M_p=2.8\times10^{-4}$ planet calculated using
the semi-analytic model.
The  solid line is a polynomial fit across the
circulating/librating region.}
\label{sc3_vort1d_v4}
\end{figure}
\begin{figure}
\center
\includegraphics[scale=0.33]{vort1d_temporary.ps}\caption{As in
  Fig. \ref{sc3_vort1d_v4} but as a function of the number of 
  Hill radii away from planet, and
    with a comparision to simulation data.}
\label{vort1d_temporary}
\end{figure}
\section{Dynamical stability of vortensity rings}\label{stability}
Having established the form of the  vortensity rings
 and the mechanism
for producing them, 
we go on to  study the linear stability of the shock-modified
protoplanetary disc model described above.
This is an important issue as instability can lead to their breaking
up into mobile non-axisymmetric structures which can
affect the migration of the planet significantly.

 The linear stability 
of inviscid baratropic  axisymmetric
rings  and discs without a planet 
 is well developed \citep{papaloizou84,papaloizou85,papaloizou89}.
The extension to a 
non-barotropic  equation of state was  undertaken more recently
 \citep{lovelace99,li00}. This work  indicates that  sharply peaked
  surface density or  vortensity features in the  disc  are  asociated with dynamical
instabilities. It is directly relevant to the types of configuration
that we have found to be produced by the disc planet interactions
described above. For example 
\cite{valborro07} considered the linear instability of gap edges
and connected it to  vortex formation there. 

Here we  consider a different
 parameter   for which highly peaked vortensity features appear in
the coorbital (horseshoe)  region. In order to be able to do this
we need to be able to define an appropriate background  equilibrium 
axisymmetric structure
to perturb. We here show that this is possible. 
\subsection{Basic background  state}
 The
basic state   should be axisymmetric and time independent with no radial velocity
($\p/\p\phi=\p/\p t=u_r=0$). To set this up we  suppose the
vortensity profile $\eta(r)$ is known (e.g. via shock modelling as above) 
and that accordingly we have 
\begin{align}\label{vortensity_definition}
\eta(r) = \frac{1}{r\Sigma}\frac{d}{dr}\left(r^2\Omega\right),
\end{align}
The radial momentum equation gives
\begin{align}\label{hydrostatic}
r\Omega^2 = \frac{1}{\Sigma}\frac{dP}{dr} + \frac{GM_*}{r^2}
\end{align}
Using these together with the locally isothermal equation of state,
  $P=h^2GM_*\Sigma/r,$ $h$ being the constant aspect ratio, we obtain a single equation
for $\Sigma$ in the form
\begin{align}\label{basic_density}
h^2\frac{d^2\ln{\Sigma}}{dr^2} = \frac{h^2-1}{r^2} -
\frac{2h^2}{r}\frac{d\ln{\Sigma}}{dr} +
\frac{2\Sigma\eta}{GM_*} \sqrt{\frac{1-h^2}{r}+h^2\frac{d\ln{\Sigma}}{dr}}
\end{align}
We solve Eq. (\ref{basic_density}) for $\Sigma$    with  $\eta(r)$ 
taken as an azimuthal average from the fiducial
simulation described in (\S\ref{fiducial}) at a time at which vortensity rings have
developed. These structures are essentially axisymmetric  
apart from in the close neighbourhood of the planet. They are  illustrated
 in Fig. \ref{vort_055}.
 We solve
Eq. (\ref{basic_density})  subject to  the boundary conditions that $\Sigma=\Sigma_0=1$ at
$r=1.1$, and $r=3.$  These conditions are consistent with the fact that
 shock-modification of the surface density profile only
occurs near the planet ($r=2$).\\
\begin{figure}
\center
\includegraphics[scale=0.50]{vort_055.ps}
\caption{A contour plot of $\ln{\Sigma/\omega}$ when the vortensity ring like structures
have formed in the coorbital region. These are almost axisymmetric apart from in the
region very close to the planet.
\label{vort_055}}
\end{figure}

 A comparison  between hydrostatic surface density  
and angular velocity profiles
 obtained by solving Eq. (\ref{basic_density}) with those obtained  as azimuthal averages from
 the corresponding simulation is illustrated in
Fig. \ref{custom_dens} and Fig. \ref{custom_urad}.  The agreement is generally very good  
indicating that the adoption  of the basic axisymmetric state  defined by the simulation
specific vorticity profile,  together with Eq. (\ref{hydrostatic}),  for stability analysis
should be a valid procedure.    Fig. \ref{custom_dens} shows that  vortensity rings reside 
in the horseshoe region just
inside the gap. At  a surface density extremum Eq. (\ref{basic_density})
implies that
\begin{align*}
h^2\frac{d^2\ln{\Sigma}}{dr^2} = \frac{h^2-1}{r^2} +
\frac{2\Sigma\eta}{GM_*}\sqrt{\frac{1-h^2}{r}}.
\end{align*}  
Since $h\ll1$, if $\eta$ is sufficiently
large then $d^2\Sigma/dr^2 > 0$. Hence vortensity maxima will coincide with
surface density minima.
 In our basic state, local minima and maxima are separated by $O(H)$ ($\simeq
0.1r_p$).
 As vortensity rings originate from
spiral shocks, Eq. ( \ref{basic_density}) demonstrates the  link
between shocks and gap formation. Sufficiently massive planets induce 
strong shocks, implying larger vortensity maxima, and hence deeper
density minima or gaps. 
\begin{figure}
\center
\subfigure[$\Sigma$\label{custom_dens}]{\includegraphics[scale=0.33]{compare2_custom_dens.ps}}
\subfigure[$\Omega/\Omega_k$\label{custom_urad}]{\includegraphics[scale=0.33]{compare2_custom_urad.ps}}
\caption{A comparison of the surface density and angular velocity profiles 
obtained by solving Eq. (\ref{basic_density}) with the same quantities obtained as  azimuthal averages
from the simulation. The vortensity profile common to both approaches is also shown.}
\end{figure}
\subsection{Linearized equations}
\indent We now  obtain the governing equation for locally isothermal
perturbations  by linearizing the  continuity equation and the equation of motion
\begin{align}\label{euler}
&\frac{\p\Sigma}{\p t} + \nabla\cdot{(\Sigma\mathbf{u})} = 0\\
&\frac{\p\mathbf{u}}{\p t} + \mathbf{u}\cdot\nabla\mathbf{u} =
-\frac{1}{\Sigma}\nabla P -\nabla\Phi,\label{momeq}
\end{align}
where $P=c^2\Sigma$   with $c^2=h^2GM_*/r.$ The  effective potential$\Phi$ is
fixed. We  set
\begin{align}
(\Sigma, u_r, u_\phi) \to (\Sigma, 0, u_\phi)+(\delta\Sigma(r), \delta u_r(r), 
\delta u_\phi(r))\times\exp{i(\sigma t + m\phi)},
\end{align}
where, the first term on the right hand side corresponds to
the basic background state, 
 $\sigma$ is a complex frequency and $m,$ the azimuthal mode number,  is a positive
integer. 
The linearised  equation  of motion (Eq. \ref{momeq}) gives
\begin{align}
\delta u_r &= -\frac{h^2}{r(\kappa^2 - \bar{\sigma}^2)}
\left(i\bar{\sigma}\frac{dW}{dr} + \frac{2im\Omega W}{r}\right)\label{velocities1}\\
\delta u_\phi &= \frac{h^2}{r(\kappa^2 - \bar{\sigma}^2)}
\left(\Sigma\eta\frac{dW}{dr} + \frac{m\bar{\sigma}}{r}W\right)\label{velocities2}
\end{align}
where
$W \equiv \delta\Sigma/\Sigma$
is the fractional density perturbation,
$\kappa^2 = 2\Omega\Sigma\eta$
is the epicyclic frequency  expressed in terms of the  vortensity $\eta,$ and
$\bar{\sigma} \equiv \sigma +m\Omega(r) = \sigma_R + m\Omega(r) + i\gamma$ 
is the Doppler-shifted frequency with  $\sigma_R$ and $\gamma$ being real. 


Substituting  Eq. (\ref{velocities1})---(\ref{velocities2}) into
the linearised continuity equation
\begin{align}
i\bar{\sigma} W = -\frac{1}{r\Sigma}\frac{d}{dr}\left(r\Sigma\delta
  u_r\right) - \frac{im}{r}\delta u_\phi
\end{align} 
yields  a  governing equation for $W$  of the form
%\begin{align}\label{goveq}
$$ 
 \frac{d}{dr}\left(\frac{\Sigma}{\kappa^2 -\bar{\sigma}^2}\frac{dW}{dr}\right)
+\hspace{4cm} $$
\begin{align}\label{goveq}
%\frac{d}{dr}\left(\frac{\Sigma}{\kappa^2 -
%    \bar{\sigma}^2}\frac{dW}{dr}\right)+
  \left\{\frac{m}{\bar{\sigma}}\frac{d}{dr}
 \left[\frac{\kappa^2}{r\eta(\kappa^2-\bar{\sigma}^2)}\right]
     -\frac{r\Sigma}{GM_*h^2}
 -\frac{m^2\Sigma}{r^2(\kappa^2-\bar{\sigma}^2)}\right\}W = 0.
\end{align}

This  equation leads to  an eigenvalue problem   for the complex eigenvalue $\sigma.$ 
 Co-rotation 
resonance occurs at $\bar{\sigma} = 0$ which requires
$\gamma =0$ for it to be on the real axis. 
Then for the equation  to remain regular,  the gradient of the  terms in
square brackets must vanish at corotation. This results in the requirement that
the gradient of $\eta r$ vanish there. Because the sound speed varies
with radius, this is slightly different from
the condition that the gradient of $\eta$ should vanish which applies
in the barotropic strictly isothermal case \citep{papaloizou84,papaloizou85,papaloizou89}.
But because  $\eta$ varies vary rapidly in the region of interest and 
 the modes we consider are  locally confined in radius, this difference is of no
essential consequence.
 Linblad resonaces occur at
$\kappa^2-\bar{\sigma}^2 = 0$. However, as is well known, and can be seen from
formulating a governing equation for $\delta u_r$ rather than $W,$
  these do not result in a singularity.

\subsubsection{Simplification of the governing ODE}
\indent It is useful to simplify Eq. (\ref{goveq})  to gain further
insight. To to this we consider  modes localized around the corotation circle
 such that the condition 
$\kappa^2\gg|\bar{\sigma}^2|$ is satisfied. Beyond this region
the mode amplitude is presumed to be exponentially small.
 Now, recognising  that $GM_*h^2/r = c^2$, the
ratio of the second to last to last  term in Eq. (\ref{goveq}) is
\begin{align*}
\frac{r^2\kappa^2}{m^2c^2}\sim\frac{1}{m^2h^2}.
\end{align*}
For a thin disc $h\ll1$, so if we consider $m=O(1)$ this ratio is
large and the last term in Eq. (\ref{goveq})  can be neglected. This is
 also motivated by the fact that only low $m$ modes (vortices)  are
observed in simulations. 
 Doing this and replacing $\kappa^2-|\bar{\sigma}^2|$ by $\kappa^2$,
 Eq. (\ref{goveq}) reduces to the simplified form
\begin{align}\label{goveq2}
\frac{d}{dr}\left(\frac{rc^2\Sigma}{\kappa^2}\frac{dW}{dr}\right)
  +\left\{\frac{m}{\bar{\sigma}}\frac{d}{dr}
 \left[\frac{c^2}{\eta}\right]
     -r\Sigma\right\}W = 0.
\end{align}
We comment that in this form  Eq. \ref{goveq2} is valid
for any fixed $c$  profile.
\subsubsection{Necesity of extrema}
 Mutiplying Eq. \ref{goveq2}
by $W^*$ and intergrating bewteen $[\,r_1,r_2]$ assuming, consistent
with a sharp exponential decay, that  $W=0$ or
$dW/dr=0$ at these  boundaries we find that
\begin{align}\label{neccessary}
\int^{r_2}_{r_1}\frac{m}{\bar{\sigma}}\left(\frac{c^2}{\eta}\right)^\prime|W|^2dr
=\int^{r_2}_{r_1}r\Sigma|W|^2 dr + \int^{r_2}_{r_1}\frac{r\Sigma
  c^2}{\kappa^2}|W^\prime|^2 dr
\end{align}
where derivatives are indicated with a prime. Since the  right hand side is real, 
the imaginary part
of the left and side must vanish. For general complex $\sigma$ this implies that
\begin{align}\label{vortmin}
\gamma\int^{r_2}_{r_1}\frac{m}{(\sigma_R+m\Omega)^2+\gamma^2}
\left(\frac{c^2}{\eta}\right)^\prime|W|^2dr
=0.
\end{align}
 Thus for a growing mode ($\gamma\neq0$) to exist we need
$(c^2/\eta)^\prime =0$ at some $r$ in $[\,r_1,r_2]$. 
For
our disc, $c^2$ varies on a scale  $O(r)$, but $\eta$ varies on  a scale  $H\ll r$, thus given
that the range of relative 
 variation of the vortensity  $\eta$ is of order unity, we infer that this quantity
 needs to  have stationary points in order  for there to be unstable 
 modes. In the baratropic case \cite{papaloizou89} have shown that vortensity
maxima are stable while minima are associated with instabilities. 
 We expect these conclusions to  apply here
also  because of the  local nature of the modes of interest.  We can approximate 
$c^2\sim\mathrm{const.}$,  or equivalently  adopt a barotropic equation of
state locally without changing the character of the problem.
 Referring back to Fig. \ref{custom_dens} it is clear
that  our basic state satisfies the neccessary criterion for
instability.\\
%\begin{figure}
%\center
%\includegraphics[scale=0.25]{F.ps}
%\caption{$F$\label{F}}
%\end{figure}
%% BELOW IS FIRST ATTEMPT, SIMPLE MODEL
%% \indent Let us consider modes with real eigenfrequency $\sigma_R = -m\Omega(r_0)$ such 
%% that $(c^2/\eta)^\prime = 0$ at $r_0$, and growth rate
%% $|\gamma|\ll\Omega_0$ so it may be ignored for the following estimate. Far away
%% from the gap, where vortensity gradients are small the term $r\Sigma W$ imply exponential solutions. In these outer regions we assume 
%% \begin{align}
%% W = \left\{ 
%% \begin{array}{l l}
%%   \exp{\lambda x} & \quad x < 0\\
%%   \exp{-\lambda x} & \quad x > 0\\
%% \end{array} \right.
%% \end{align}
%% where $x\equiv r-r_0$ and $1/\lambda=O(H)$ is the decay length-scale. Exponentials can not be joined smoothly at $x=0$ so 
%% the solutions only apply, say, for $|x|>\delta$. When $|x|<\delta$, vortensity term dominates and we balance
%% \begin{align}\label{goveq2b}
%% \frac{d}{dr}\left(\frac{rc^2\Sigma}{\kappa^2}\frac{dW}{dr}\right)
%%   =-\frac{m}{\bar{\sigma}}\frac{d}{dr}
%%  \left[\frac{c^2}{\eta}\right]W.
%% \end{align}
%% In the vincinity of $x=0$ we approximate
%% \begin{align}
%% \bar{\sigma} &= m(\Omega^\prime_0 x + \Omega^{\prime\prime}_0x^2/2 + \ldots)\\
%% \left(\frac{1}{r\eta}\right)^\prime &= \left(\frac{1}{r\eta}\right)^{\prime\prime}_0 x  + 
%% \left(\frac{1}{r\eta}\right)^{\prime\prime\prime}_0x^2/2 + \ldots 
%% \end{align}
%% Since Eq. \ref{goveq2b} is a second order ODE we specify the boundary conditions $W_0 = 1,\, W^\prime_0 = 0$. The first
%% is due to arbitary normalisation of the eigenmodes; the second for symmetry about $x=0$. Then, evaluating Eq. \ref{goveq2b}
%% at $x=0$ gives
%% \begin{align}
%% \left(\frac{1}{2\Omega\eta}\right)_0 W^{\prime\prime}_0 = -\frac{1}{\Omega^\prime_0}\left(\frac{1}{r\eta}\right)^{\prime\prime}_0,
%% \end{align}
%% where $\kappa^2 = 2\Omega\Sigma\eta$ and $c^2 = h^2/r$ was used. Applying Taylor expansion, the approximate solution is (dropping subscript 0)
%% \begin{align}
%% W &= 1 + K^2x^2,\\
%% K^2 &\equiv - \frac{\Omega\eta}{\Omega^\prime}\left(\frac{1}{r\eta}\right)^{\prime\prime}.
%% \end{align}
%% If the disturbance maximise at $x=0$ we require $K^2<0$. Since $\Omega^\prime<0$ this requires 
%% $(1/r\eta)^{\prime\prime} < 0$, or approximately a vortensity minimum. As $|K^2|$ increase, the disturbance becomes
%% concentrated near $x=0$. Imposing continuity of $W$ and $W^\prime$ at the transition point $x=\pm\delta$ to the exponential 
%% solutions gives 
%% \begin{align*}
%% \delta^2 + \frac{2}{\lambda}\delta + \frac{1}{K^2} = 0,
%% \end{align*}
%% with solution
%% \begin{align}\label{delta}
%% \lambda\delta = -1 + \sqrt{1-\lambda^2/K^2},
%% \end{align}
%% so that $\delta\lambda\to0$ as $|K^2|\to\infty$. As the vortensity profile becomes more extreme, the transition width decreases compared
%% to exponential decay length-scale. However, in performing the analysis it was implicitly assumed that the transition width was small. Hence
%% $-K^2$ needs to be sufficiently large for self-consistent solutions to Eq. \ref{delta}. This means co-rotational modes described above can only
%% exist in discs with sufficiently extreme vortensity profiles. Finally, although the azimuthal wave number $m$ does not appear explicitly, 
%% we have already assumed low $m$ modes in Eq. \ref{goveq2}. \\
%% \indent The vortensity minimum of the inner gap edge, for the standard disc, is at $r_0\simeq1.7$, assuming
%% $\lambda = 1/nH$, Eq. \ref{delta} gives
%% \begin{align*}
%% \lambda\delta \simeq \sqrt{1+0.7/n^2} -1.
%% \end{align*}
%% E.g. if $n=2$ then $\lambda\delta \sim 0.1$. The transition width will typically be a fraction of the local scale height. 
%% \subsubsection{Existence of local modes}     
%% \indent In parts of analysis above we assumed co-rotational modes are
%% localised. We demonstrate this explicitly by searching for non-neutral
%% modes centred about vortensity minimum $r_0=1.7$ of our standard
%% disc. Locally the disc profile is approximated by 
%% \begin{align*}
%% \Sigma &= \Sigma_0 + \Sigma^\prime_0 x ,\\
%% \eta & = \eta_0 +\frac{1}{2}\eta^{\prime\prime} x^2 ,\\
%% \kappa^2 &= \kappa^2_0 + \frac{1}{2}\kappa^{2\prime\prime}_0 x^2,\\
%% \bar{\sigma} &= m\Omega^\prime_0 x +i\gamma,
%% \end{align*}
%% where $x=r-r_0$ and we assumed $\sigma_R + m\Omega_0 = 0$. We checked
%% that vortensity minima corresponds to minima in $\kappa^2$. Writing
%% out Eq. \ref{goveq2} in the standard form $AW^{\prime\prime} + B
%% W^\prime +CW=0$, and expanding the coefficients to zeroth order in $x$ we
%% find (dropping subscript $0$):
%%   \begin{align}  
%%   W^{\prime\prime} + \frac{\Sigma^\prime}{\Sigma}W^\prime
%%   -\frac{\kappa^2}{c^2}W =0,
%%   \end{align}
%%  which has solutions $W\propto\exp{kx}$ with
%%  \begin{align}
%%  k=\frac{1}{2}\left(-\frac{\Sigma^\prime}{\Sigma}\pm
%%    \sqrt{\left(\frac{\Sigma^\prime}{\Sigma}\right)^2 +
%%    4\frac{\kappa^2}{c^2}}\right)  
%%  \end{align}
\subsection{Numerical solution of the eigenvalue problem}
 We  have solved the eigenvalue problem
for the  full equation  (\ref{goveq}) using a 
shooting method  that employs an adaptive Runge-Kutta integrator 
and a  multi-dimensional Newton method \citep{press92}. 
 For low $m$ ($\leq 3$)  unstable modes mainly comprise an evanescent disturbance
 near co-rotation and the simple  boundary condition $W = 0$ applied
at the inner boundary $r/r_p=0.55$ and the outer boundary $r/r_p=1.5$ produces  
good results. 
\begin{figure}
\center
\subfigure[Inner edge]{\includegraphics[scale=0.25]{s1h005_WBC0_m3_in.ps}}
\subfigure[Outer edge]{\includegraphics[scale=0.25]{s1h005_WBC0_m3_out.ps}}
\caption{$m=3$ eigenmodes obtained  with the  boundary condition $W=0.$
The background vortensity profile is also shown.\label{s1h005}}
\end{figure}
As  $m$ increases,  the  Linblad resonances approach  $r=r_p$.
and a  significant portion of the mode is wave-like 
requiring  the application of  outgoing  radiation boundary conditions.   
We determined these  using the  WKBJ  approximation (see eg.  Korycanski \& Pollack 1993). 
\subsubsection{Eigenmode calculations}
We have determined unstable eigenmodes using the above procedures for   $1 \ge m \le ??. $
We recall that the simulations indicate the ultimate  dominance of small $m$ values.
One class of mode is associated with the inner vortensity ring while another
is associated with the outer ring.

 As a typical example of the behaviour that is found for low $m,$ each type  of eigenmode  for  $h=0.05$ and  $m=3$ 
is shown in Fig. \ref{s1h005}. The background vortensity profile is also shown.
The instabilities  are associated with the  vortensity minima at the inner
and outer  gap edge, as has also been 
observed by \cite{li05} in simulations. 
  the modes are evanescent around co-rotation and the  vortensity peaks 
behave like wall through which the instability scarcely penetrates.
 The mode decays away from $r=r_p$. For $m=3$
Lindblad resonances occur at $r_L/r_p=0.76,\,1.21$  from which 
waves travelling away from co-rotation are emitted. 
 However,
the oscillatory amplitude is at most $\simeq 20\%$ of that at $r=r_p$. Hence for  low-$m$ 
the dominant effect of the instability will be due to perturbations near co-rotation. 
Increasing $m$ brings $r_L$ even closer to $r_p$, waves  then propagate through the gap. 
 The growth time-scale of the inner mode with $m=3$ is  $\sim14P_{orb},$
$P_{orb}$ being the orbital period of the planet.  The outer mode
has a growth rate that is about three times faster.  Very similar
results and growth rates were found  for $m=1$  and $m=2$. 


After the onset of linear instability and the formation of several vortices,
it has been observed that non linear effects 
cause them to eventually 
merge into a single vortex (refs).  This eventually interacts with the planet. 
In the fiducial simulation,
rapid migration begins at $55P_{orb}$ which is compatable with the characteristic  growth 
times found  from linear theory. \\
Fig. \ref{s1h005}  indicates that 
the outer edge is more unstable than inner edge. 
The vortensity peaks are of similar
height, but the inner minimum in  $r\eta$  is less pronounced 
 than outer because of the background profile. In this sense the outer edge
profile is more extreme, and hence less stable.

{\bf *****Perhaps a plot for higher m values can be included}
%\subsection{Comparison of inner/outer edges}
%\subsection{Growth rates and azimuthal wave number}
%\subsection{Application to disc-planet problem}
%\ifpdf
%  \pdfbookmark[2]{bookmark text is here}{And this is what I want bookmarked}
%\fi
% ------------------------------------------------------------------------
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Chapter1/ringsnew.tex <==
%\chapter{Ring structures in disc-planet interactions}\label{rings}
%\ifpdf
%    \graphicspath{{Rings/Figs/PNG/}{Rings/Figs/PDF/}{Rings/Figs/}}
%\else
     \graphicspath{{Rings/Figs/EPS/}{Rings/Figs/}}
%\fi
\section{Basic equations and model}\label{modeleq}
We consider a planet of mass $M_p$ orbiting a central star 
of mass $M_*.$  We adopt a cylindrical coordinate system $(r,\phi,z)$
where $z$ is the vertical coordinate increasing in the direction normal to the disc plane
for which the unit vector is ${\hat{\bf k}}.$ 
The governing hydrodynamic equations
in a frame uniformly rotating with angular velocity $\Omega_p{\hat{\bf k}}$ are the continuity 
equation
\begin{align}\label{continuity}
\frac{D\Sigma}{Dt}=-\Sigma\nabla\cdot\mathbf{v},
\end{align}
and the equation of motion
\begin{align}\label{momentum}
\frac{D\mathbf{v}}{Dt}+2\Omega_p\hat{\mathbf{k}}\wedge\mathbf{v} = 
-\frac{1}{\Sigma}\nabla P - \nabla\Phi_{\mathrm{eff}},
\end{align}
where $D/Dt$ is the total derivative, the vertically integrated pressure  $P=c_s(r)^2\Sigma$ with
$c_s=h(GM_*/r)^{1/2}.$ 
Here $\Sigma$ is the surface density, ${\bf v}$ is the velocity and the effective
gravitational and centrifugal  potential is
given by
\begin{align}
\Phi_{\mathrm{eff}} = -\frac{GM_*}{r} - \frac{GM_p}{\sqrt{r^2+r_p^2
+2rr_p\cos(\phi-\phi_p)+\epsilon^2}}-\frac{1}{2}\Omega_p^2r^2.
\end{align}
Here the cylindrical coordinates of the planet are $(r_p,\phi_p,0)$
 and the  softening length $\epsilon = 0.6hr_p$
 with  $h$ being the disc aspect ratio.\\
 
 \subsection {Vortensity conservation}\label{secvort}
The vortensity  being the ratio of the  $z$ component of the  vorticity  (hereafter just  called the vorticity)
 to the surface density is
defined to be 
\begin{equation}\label{vortensity}
\eta =  \frac{\omega}{\Sigma} \equiv \frac{\omega_r+2\Omega_p}{\Sigma},
\end{equation}
where $\omega_r=\hat{\mathbf{z}}\cdot\nabla\wedge\mathbf{v}$ is the relative
vorticity seen in the rotating frame.
 It is well known that In barotropic flows without shocks,
it follows from (\ref{continuity}) and (\ref{momentum}) that the  vortensity
$\eta = \omega/\Sigma$  is
conserved for a  fluid particle. 
When an isothermal equation of state with variable sound speed as is used 
here is adopted, vortensity is no longer strictly conserved.
However, the sound speed varies on a global scale
so that  when   phenomena are considered on a local scale,  vortensity is 
 conserved to a good approximation in the absence of shocks.

\section{Ring structures in disc-planet interactions}\label{rings} 
In this section we  present hydrodynamic simulations to
show that narrow  surface density rings are brought about as  a consequence
of the fact that highly peaked 
vortensity  ( being the ratio of the vorticity to the surface density) 
 rings are produced by flow through quasi-steady shocks
located close to  the planet. For
sufficiently massive planets, the associated vortensity generation occurs as fluid
elements execute a horse-shoe turn in the coorbital region. 
Focusing on such
cases, we construct  a simple model that enables an estimate of the shock
location to be made together with rate of the vortensity
generation as material flows through it. Our model is in good agreement with
numerical simulations and confirms the process of
vortensity generation within a planet's co-orbital region  which later
plays an important role in modifying  the flow structure there. 
\subsection{Hydrodynamic simulations}\label{sec2}
For convenience we adopt dimensionless units such that the initial
orbital radius of the planet is $r_p=2.$ In these units the 
the radial computation domain  for the simulations described in this
section is  $r=[1,3]$.
The disc  has an  initially uniform surface density $\Sigma=\Sigma_0.$ 
Boundary conditions corresponding to outgoing waves were adopted.
We remark that
ring formation occurs as a result of  shocks near the planet and therefore is
unaffected by boundary conditions. 
 For the simulations described in this section the planet is held fixed
 on its initial circular orbit   with Keplerian angular velocity
$\Omega_p=\sqrt{GM_*/r_p^3}$ which also defines the rotation of the coordinate system.  Time is expressed in units
of the orbital period $2\pi/\Omega_p$ defines the dimensionless time we adopt.
The unit of mass is taken to be the central mass $M_*$ which
for working purposes may be considered to be $1M_{\odot}.$ 
The planet mass is increased gradually from zero such that it attains its full
value after  five orbital periods.
\indent We use the FARGO code to solve for the disc response
\citep{masset00a,masset00b}. FARGO evolves the hydrodynamic
equations in global cylindrical co-ordinates centred on the central
object. We used a non-rotating frame for the simulations described
here. Indirect terms arising from the non-inertial frame is included
in the potential. The code uses a finite-difference scheme with van Leer upwind
and hence is second-order accurate in space, similar to the
ZEUS code \citep{stone92} but it employs a modified algorithm for
azimuthal transport that allows for large time steps. 
We take $2\pi$-periodic boundary condition in
the azimuth and wave damping boundary conditions at disc boundaries
\citep{valborro06}. 

*****{`\bf some references to code....softening..convergence..etc...}***********
  
\subsection{ Vortensity generation by the shocks 
induced by a Saturn mass planet}\label{fiducial}
\indent We first consider  case with $M_p=2.8\times10^{-4}M_*$ corresponding
to a Saturn mass planet around a solar mass star.
 For these calculations the
resolution was $N_r\times N_\phi=1024\times3072$,  corresponding to 
grid radial and azimuthal grid spacings of   $\Delta r\simeq
0.02r_h$ and $r\Delta\phi\simeq0.05r_h$ respectively, where
$r_h$ is the planet's Hill radius in dimensionless units.

 Fig.\ref{vortxy_020} shows the vortensity field at
$t=7.07$ close to the planet. Vortensity is
generated/destroyed as material passes through the two spiral shocks.
 For the outer shock, vortensity
generation occurs for fluid elements executing a
horse-shoe turn ($|r-r_p|\lesssim r_h$) while  vortensity is reduced for
fluid that passes by the planet.  But the change is smaller in magnitude
in the latter case.
 The
situation is similar for the inner shock, but some post-shock material
with increased vortensity continues to pass by the planet. This stream begins at
$r\simeq -r_h$ but such feature is absent at the outer
shock,suggesting a lack of symmetry about $r=r_p$, possibily resulting from
the non-uniform vortensity background being $\propto r^{-3/2}$.
  Note that although a pre-shock fluid element that would be  on a horse-shoe trajectory,
may in fact pass by the planet after crossing the shock, it is
clear that vortensity rings originate from passage through shock fronts interior
to the  co-orbital  region that would correspond to the horseshoe region
for free particle motion.

 The streams of high vortensity eventually move around the whole orbit outlining the
entire co-orbital region. Fig. \ref{vortxy_020} shows  that they are generated
along a small  part of the shock front  with length  $l\sim r_h$. This  results in
thin rings with  a similar  radial width.
The fact that they originate from horse-shoe
material can  enhance the contrast  as post-shock
inner disc horse-shoe material is mapped  from $r-x$ to  $r+x$ 
to become
adjacent to post-shock   outer disc material passing by the planet.

\begin{figure}
\center
\includegraphics[scale=0.5]{vortxy_020.ps}\caption{Vortensity
generation and destruction across shocks induced by a Saturn-mass
planet in an inviscid disc. The plot shows log(vortensity) $=\log{\omega/\Sigma}$.
Regions of increased vortensity are clearly visible as half horseshoes
above and below the planet. The increase occurs as material passes through
parts of the shock fronts that extend  into  the coorbital region.}
\label{vortxy_020} 
\end{figure}
\begin{figure}
\center
\includegraphics[scale=0.4]{coorb_plot_0.ps}\caption{Long-term
  evolution of co-orbital properties for a Saturn-mass planet held on
  fixed orbit. Vorticity, density and vortensity 
  perturbations are expressed   relative to their  values at $t=0$.
{\bf ***I think torques and coorbital mass deficits should be removed 
here and the axis relabelled*******}} \label{coorb_plot_0}
\end{figure}

\subsection{ Location of the  vortensity generation region for different planet masses}
\indent The process of  formation of vortensity rings discussed 
 here differs from  that observed
in \cite{koller03} and \cite{li05}, where the rings are generated by shocks outside
the co-orbital region. This is because the authors used a
smaller planet mass. 
To illustrate  the effect of reducing the mass, we ran low resolution
simulations ($N_r\times N_\phi = 256\times768$) for $M_p\times10^{4}=1,\,2.8$ and
$10$. Fig. \ref{compare2_020} compares azimuthally averaged
vortensity perturbations induced in each case after $14.14$ orbits. 
The intermediate and high mass cases are
qualitatively similar, having $\Delta(\omega/\Sigma)$ maxima at
$r-r_p\sim\pm 2r_h$ and minima at $r-r_p\sim3 r_h$. The magnitude of
$\Delta(\omega/\Sigma)$ increases with $M_p$ because higher masses
induce 
 higher Mach number shocks. As the half-width of the horseshoe region
is $2.5 r_h$
 for such masses (refs), vortensity rings
are co-orbital features.
\begin{figure}
\center
\includegraphics[scale=0.4]{compare2_020.ps}\caption{Azimuthally averaged vortensity
  perturbation for different planet masses.} \label{compare2_020}
\end{figure}
\indent The low mass $M_p=10^{-4}$ case has much smaller
$|\Delta(\omega/\Sigma)|$. There is a vortensity maximum at $r-r_p=-3r_h$
but nothing of similar magnitude at $r-r_p>0$. 
 \cite{paardekooper09}
found the co-orbital half-width, in the limit of zero softening
for low mass planets, to be:
\begin{align}
x_s=1.68(M_p/h)^{1/2}r_p.
\end{align}
For $M_p=10^{-4},\,h=0.05$, $x_s=2.33r_h$. For
non-zero softening, the actual $x_s$ is smaller. Hence, vortensity
rings for low mass planets occur outside the  co-orbital region as is
confirmed in our simulations and they are very much weaker. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% HIGH RESOLUTION RESULTS FOR VORTENSITY GENERATION V.S. M_P
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \delta m = -5\times10^{-5} for M_p = 10^{-4}
%% \delta m = -2\times10^{-4} for M_p = 2.8\times10^{-4}
%% \delta m = +5\times10^{-4} for M_p = 10^{-3}
%% the 1d vortensity plot is very similar to low resolution case (picture
%% at /data/stardisk/mkl23/hyades/vorticity/compare2_040.ps). in the
%% above, only radial derivative part of voriticy is used. the low
%% resolution stuff presented above used full expression for
%% vorticity, there is little difference between the two. low
%% resolution was needed to examine long term evolution/equilibrium
\subsection{ A semi-analytic model for coorbital 
vortensity generation by shocks}\label{model}
\indent We now  construct a semi-analytic model describing the process of
shock-generation of vortensity.  In this way we gain an understanding
of the physical processes involved and later how they lead to 
strong torques and fast migration of the planet and under what conditions
simulations  can represent them acurately.

More specifically we model the outer
spiral shock in Fig. \ref{vortxy_020}. To do this we need the  pre-shock flow field,  the shock front
location  and then to evaluate the vortensity change undergone  by
material as it passes through the shock.
We now consider these in detail 

\subsection{Flow field}
\indent We first simplify the geometry by adopting the shearing box
approximation \cite[e.g.][]{paardekooper09}. As we are concerned with
the flow near the planet, we consider a local Cartesian co-ordinate
system $(x,y)$ co-rotating with the planet at angular
speed $\Omega_p$ and with origin at its centre of mass. Without the planet, the velocity field is
Keplerian $\mathbf{v}=(0,-3\Omega_p x/2)$. 
In order to deal with the pre-shock flow we make the assumption that pressure effects can be ignored
 compared to planet potential.  This ballistic  approximation is appropriate for 
 a slowly varying  supersonic flow as is expected to be appropriate for the pre-shock
 fluid. The   velocity $\mathbf{v}$  satisfies the local form of
 equation ( \ref{momentum} ) with  $P=0$ and the effective
 potential
 \begin{align}
\Phi_{\mathrm{eff}} =  - \frac{GM_p}{\sqrt{x^2+y^2+\epsilon^2}}-\frac{3}{2}\Omega_p^2x^2
\end{align}
and thus follows from particle dynamics.
We write a fluid particle's trajectory in a steady state flow  in the form
 as  $ x=x(y)$ and the corresponding velocity field
 as $\mathbf{v}=\mathbf{v}(y).$
 Noting that  on a particle trajectory we have 
 $\frac{D}{Dt}=v_y\frac{d}{dy}$,  it follows from the local form of (\ref{momentum}) 
 that on a  particle trajectory we have the following system of three simultaineous
 first order differential equations:
\begin{align}
\label{semi-an}\frac{dv_y^2}{dy}&=-4\Omega_pv_x-\frac{2M_py}{(x^2+y^2+\epsilon^2)^{3/2}}= Q,\\
\frac{d}{dy}\left(v_xv_y^2\right)&=v_xQ+2\Omega_pv_y^2 
+v_y\left[3\Omega_p^2x-\frac{M_px}{(x^2+y^2+\epsilon^2)^{3/2}}\right],\\
\frac{d}{dy}\left(xv_y^2\right)&=xQ+v_xv_y.
\label {semi-an1}\end{align}
We  use these to solve for the state vector
$\mathbf{U}(y)=[v_y^2,\,v_xv_y^2,\,xv_y^2]$ in $x>0$ for a particular
particle. The boundary condition is 
\begin{align}
(v_y,\, v_x,\, x)\to(-3\Omega_p x_0/2, \, 0, \, x_0) \,\,\mathrm{as}\,\,
y\to\infty , 
\end{align}
where $x_0$ is the particle's unperturbed path. 
The totality of paths obtained by considering a continuous range of $x_0$
then constitutes the flow field.  Having obtained the velocity field, we 
use  vortensity conservation to obtain $\Sigma$. The density is then
\begin{equation}
\Sigma(x,y) = \frac{2\Sigma_0}{\Omega_p}(\omega_r+2\Omega_p),
\end{equation}
where the unperturbed absolute vorticity is
$\omega_r =\Omega_p/2.$  Numerically, we
calculated the relative vorticity  by relating it to the circulation through 
\begin{equation}
\omega_r\simeq\frac{1}{\Delta A}\oint\mathbf{v}\cdot\mathbf{dl}
\end{equation}
where the integration is taken over a closed loop about the point of
interest and $\Delta A$ is the enclosed area. This avoids
errors due to  numerical
differentiation on the uneven grid in $(x,y)$  generated by solving the above system.
\subsection{Location of the shock front}
\indent The physical reason for shock formation is the fact that the
planet presents an obstacle to the flow. Where the relative flow is subsonic,  the
presence of this obstacle can be communicated to the fluid via sound
waves emitted by the planet. In regions where the relative flow is supersonic,  the fluid is unaware
of the planet via sound waves (but  the planet's
gravity is felt).  We estimate the location of the boundary separating these two regions
by  specifying an appropriate characteristic curve or ray defining a sound wave.  
This is a natural location for shocks. Applying this
idea to Keplerian flow, \cite{papaloizou04} obtained a good match
between the predicted theoretical shock front and the wakes associated with a low mass
planet. For general velocity field $\mathbf{v}$, the characteristic
curves satisfy the equation 
\begin{align}\label{shock_front}
\frac{dy_s}{dx} =
\frac{\hat{v}_y^2-1}{\hat{v}_x\hat{v}_y-\sqrt{\hat{v}_x^2+\hat{v}_y^2-1}},
\end{align}
where $\hat{v}_i= v_i/c_s$. The  positive sign of the square root
has been chosen so that the curves have negative slope
in the domain $x>0$   with $v_y<0.$  As the fluid flows
from super-sonic ($y>y_s$) to sub-sonic ($y<y_s$), fluid located at 
 $y=y_s$  begins
to know about the planet through pressure waves \citep{papaloizou04}. In
Keplerian flow, the rays defining the shock fronts originate from the  sonic points at
$x=\pm2H/3,\,y=0$. In a  general flow,  sonic points where  ($|\mathbf{v}|=c_s$),
at which the rays may start,
lie on  curves and can occur for $x<2hr_p/3$.  The starting
sonic point for   solving  Eq. ( \ref{shock_front}) that we eventually  adopted has
 $x=0$ and the value of  $y >0$ that is furthest possible
from the planet.
\subsection{Vorticity and vortensity changes across a shock}
\indent The jump in absolute vorticity $[\omega]$ is readily obtained by
resolving the fluid motion parallel and perpendicular to the shock
front  \citep[eg.][]{kevlahan97}. As we do not solve the energy equation,
and shocks are locally  isothermal our expression differs from
those of  \citet{kevlahan97}   accordingly a brief derivation of $[\omega]$ is
presented in  Appendix B. The result for a steady shock is
\begin{align}\label{vorticity_jump}
[\omega]=-\frac{(M^2-1)^2}{M^2}\frac{\p v_\perp}{\p S}+(M^2-1)\omega
-\left(\frac{M^2-1}{v_\perp}\right)\frac{\p c_s^2}{\p S},
\end{align}
where $v_\perp$ is the pre-shock  velocity perpendicular to the
 $M=v_\perp/c_s$ is perpendicular Mach number
and $c_s=hr^{-1/2}$ is the sound speed. $\p/\p S$ is derivative
along the shock. It is  important to note that for (\ref{vorticity_jump}) to hold,
 the direction of increasing $S,$ the direction of positive  $v_{\perp},$
 and the vertical direction should form
a right handed triad.
The local
isothermal equation of state produces the last term on RHS of
Eq. (\ref{vorticity_jump}). Because of the slow variation of $c$  
its contribution is not important in this application. \\ 
\indent The vortensity jump $[\omega/\Sigma]$ follows immediately from
Eq. (\ref{vorticity_jump}) as
\begin{align}\label{vortensity_jump}
\left[\frac{\omega}{\Sigma}\right]=-\frac{(M^2-1)^2}{\Sigma M^4}\frac{\p
  v_\perp}{\p S}-\left(\frac{M^2-1}{\Sigma M^2v_\perp}\right)\frac{\p c_s^2}{\p S},
\end{align}
which reduces to the expression derived by \cite{li05} if
$c_s=\mathrm{constant}$. The sign of  $[\omega/\Sigma]$ depends mainly on the gradient of
$v_\perp$ (or $M$) along the shock. As in our case  $v_\perp<0,$ the width of the  increased vortensity
rings produced is determined by  the length along the shock where $|M|$ is
increasing.  %% . Since $v_\perp<0$, increasing
%% shock strength along it implies vortensity generation.
Note that $[\omega/\Sigma]$ does not depend explicity on the  pre-shock vortensity,
unlike the absolute vorticity jump.


\subsection{Comparison of the results of the semi-analytic model with numerical simulations}
 We  now compare the results of hydrodynamic simulations
with those obtained from the model.  
 First we illustrate the particle paths that constitute
 the flow field together with the  shock
fronts obtained by assuming coincidence with the characteristic curves
that are obtained from the semi-analytic model 
in Fig. \ref{shock_curve2_}.
A polynomial fit to the simulation shock front is also
shown.
 Particle paths cross for $x > r_h,\,y < -2r_h$
 so  that the neglect of pressure becomes invalid.  Accordingly  the
solution to equation(\ref{shock_front})  should not be trusted in this
region.  Fortunately, vortensity generation occurs at a distance from the planet that is  within 
$1-1.5r_h$, where pre-shock particle paths do not cross.\\
\begin{figure}
\center
\includegraphics[scale=0.4]{shock_curve2_.ps}\caption{Solid lines: particle paths from the reduced zero-pressure
momentum equations (equations \ref{semi-an} - \ref{semi-an1}); thick lines: curves composed of sonic points
 on which $|\mathbf{v}|=c_s$;
dotted lines: theoretical shock fronts; dash-dot line: solution to equation ( \ref{shock_front}) for Keplerian flow; dashed line: 
polynomial fit to simulation shock front. The actual shock front begins  at a sonic point 
around $x=0.2r_h.$}
\label{shock_curve2_}
\end{figure}
%%
\indent The key quantity  determining vortensity generation is the
perpendicular Mach number. Fig. \ref{sc3_machsq_020} compares $M$ from
simulation and model.  Although the semi-analytic model gives a shock  Mach number
that is somewhat smaller than found from the simulation, all curves have $|M|$
increasing from $x=0\to 1.3r_h$ which is the important domain for vortensity
generation.  Thus  equation(\ref{vortensity_jump})
 implies  vortensity generation in all cases. Note that in the significant domain
  $x \in [0\to 1.3r_h]$ the Mach numbers deviate by less than 50\%.
\begin{figure}
\center
\includegraphics[scale=0.4]{sc3_machsq_020.ps}\caption{Perpendicular
  Mach number $M$ along the outer spiral shock  illustrated in
  Fig. \ref{vortxy_020}. Asterisks: simulation data; dotted line:  Mach number obtained 
  from the simulation shock
  and the semi-analytic flow; solid line: Mach number 
  obtained from the  semi-analytic shock front and flow.}
\label{sc3_machsq_020}
\end{figure}
%%
 In Fig. \ref{mp2.8} we illustrate various  combinations of
semi-analytic modeling  and simulation data that have been used to
estimate the  vortensity jump
across the shock.
 The qualitative   quantitative similarities  
 between the various curves confirms that the
vortensity generation  occurs  within the Hill sphere in coorbital
material that is shocked as it undergoes horseshoe turns.
 
 Assuming that material is mapped from $x\to -x$ as it switches to
the inner leg of its horse-shoe orbit,  we expect the outer spiral
shock to produce a vortensity ring peaked at $r-r_p\sim -0.5r_h$ of
width $O(r_h)$ ($=O(H)$), with a similar discussion
applying to the inner shock which is expected to produce
a vortensity ring peaked at $r-r_p\sim 0.5r_h$ . Thus,
thin vortensity rings are natural features of the co-orbital
region.

 We have  also tested our model for $M_p=2\times10^{-4}$ in
Fig. \ref{mp2}.  In this case there is still  a good qualitative 
match between the simulation and  the model.
This   is the case even though  lowering $M_p$  makes  the zero-pressure
approximation, adopted to determine the semi-analytic flow field, less good. 
Decreasing $M_p$ shifts vortensity generation
away from the planet in the semi-analytic model, as  is also observed in 
the hydrodynamic simulation
(Fig. \ref{compare2_020}). In this case, there is no vortensity
generation in $r-r_p<0.5r_h$ but vortensity rings are are still
co-orbital ( with  peaks at $\sim0.7r_h$).\\ 
We remark that steep
vortensity gradients are associated with 
dynamical instabilities \citep[e.g.][]{papaloizou85} and this is
explored in more detail below. 
\begin{figure}
\center
\subfigure[\label{mp2.8}]{\includegraphics[scale=0.4]{vort_jump1}}
\subfigure[\label{mp2}]{\includegraphics[scale=0.4]{vort_jump2}}
\caption{Semi-analytic  and actual vortensity jumps across a shock in the
  co-orbital region. Asterisks are measured from the simulations. The
  dashed lines were obtained by using pre-shock simulation data coupled
  with the jump condition  specified by equation( \ref{vortensity_jump}). The  dotted lines 
  were obtained using the semi-analytic flow field together with
  the location of the  shock front obtained from the simulation.  The  solid
  curves  correspond to the semi-analytic model for both the flow field and shock front.}\label{vort_jump}
\end{figure}
%%
%\begin{figure}
%\center
%\subfigure[$M_p=2.8\times10^{-4}$]{\includegraphics[scale=.33]{jump_machsq_lin.ps}}
%\subfigure[$M_p=2\times10^{-4}$\label{jump_machsq_lin_m2}]{\includegraphics[scale=.33]{jump_machsq_lin_m2.ps}}
%\caption{$M^2$ along the outer spiral shock (horizontal axis is $x$
  %co-ordinate along shock). Solid line is measured from simulation,
  %with the dashed curve as a polynomial fit, and dotted line is the
  %linear model.\label{jump_mach_lin}}
%\end{figure}
%\begin{figure}[!h]
%\center
%\subfigure[$M_p=2.8\times10^{-4}$]{\includegraphics[scale=.33]{jump_vortensity_lin.ps}}
%\subfigure[$M_p=2\times10^{-4}$]{\includegraphics[scale=.33]{jump_vortensity_lin_m2.ps}}
%\caption{Vortensity jump across outer spiral shock. Asterisks are measured
  %from simulation, solid line is expected jump given pre-shock data
  %from simulation and using the analytic jump expression, dotted curve
  %is prediction from linear model.\label{jump_vortensity_lin}}
%\end{figure}
\subsection{Azimuthally averaged  vortensity profile}
 Here we use our semi-analytic shearing
box model to  estimate the azimuthally averaged vortensity
profile. In order to
make progress we make the following simplifying 
assumptions:
\begin{enumerate}
\item Vortensity is only changed across the shock and conserved
  elsewhere ( see section \ref{secvort}). 
\item Symmetric spiral shocks. We assume $[\omega/\Sigma]$ for $x<0$
  (inner spiral shock) is the 
 same as for the outer spiral shock.  This is consistent with
  the shearing-box approximation. 
\item We use the shearing box model desccribed above   to
  obtain $[\omega/\Sigma]$, then apply the implied 
change to the background vortensity
  profile of the global model, being given by 
 $\omega_0=r^{-3/2}/2\Sigma_0.$
\end{enumerate}
\indent We note in Fig. \ref{mp2.8}, the horizontal axis corresponds
to the $x$-coordinate of the shock front. A fluid element which shocks
at a particular 
 $x$ originated from a location $(x_0,\,y>0).$   For $x_0 <
x_s\equiv2.5r_h$  the trajectory  starts 
 on a horseshoe orbit. We assume the shock
does not change this  so that such particles are mapped to
$-x_0$ after it executing  the horseshoe turn. 
Such particles   
experience $[\omega/\Sigma]>0$ so that the inner vortensity ring is
attributed to the outer spiral shock and the outer ring to the inner
spiral shock  as is  observed in
simulations (see Fig. \ref{vortxy_020}).
 Particles with $x_0>x_s$ continue to circulate after the
shock. Both librating and circulating particles can be re-shocked so
we expect the vortensity peaks and troughs to increase
 in amplitude to some extent. Eventually after a few returns
the system may approach a steady state for which 
${\partial v_{\perp}}/{\partial S}\rightarrow 0$
However, 
we shall not investigate this in detail  here
but  simply consider  the initial ring formation as a result
of the first shocking. 


Our procedure is as follows. The post-shock vortensity of a
particle originating from $x_0>0,y>0$ is
\begin{align}
\left(\frac{\omega}{\Sigma}\right)_{x} =
\left(\frac{\omega_0}{\Sigma_0}\right)_{x_0}
 +\left[\frac{\omega}{\Sigma}\right]_{x}. 
\end{align}
 If the location where the particle is shocked
  satisfies  $x < x_s$ it
will be located at $(-x_0,\,|y/r_h|\gg1)$ after it executes a horseshoe turn.
If $x >x_s$ it continues to circulate and  will be located at
$(x_0,\,y<0)$. Thus,
\begin{align}
\left(\frac{\omega}{\Sigma}\right)_{x} = \left\{ 
\begin{array}{l l}
  \left(\omega/\Sigma\right)_{-x_0} & \quad \mbox{$x_0<x_s$}\\
  \left(\omega/\Sigma\right)_{x_0} & \quad \mbox{$x_0>x_s$.}\\
\end{array} \right.
\end{align}
A similar argument is applied to the inner shock. 
 We
then transform to the global cylindrical co-ordinates  using $x_0\to x_0 +
r_p$. 

 The vortensity profile for $M_p=2.8\times10^{-4}$ obtained from the
semi-analytic model
is shown in Fig. \ref{sc3_vort1d_v4}. The central region
corresponds to particles whose vortensity is not modified by shocks.
However, strictly  speaking 
the  vortensity distribution changes because particles switch between
$r_p\pm x_0$ conserving  their vortensity and the background 
(unperturbed) vortensity
distribution 
is non-uniform. This is a minor effect that is expected to lead to
a uniiform distribution due
to phase mixing. To deal with  this,
     we adopt the simple procedure of replacing the
vortensity  everywhere in this region with the 
unperturbed  vortensity at the planet's location,
$r_p^{-3/2}/2\Sigma_0$. 
Fig. \ref{sc3_vort1d_v4}  shows that we expect sharp
vortensity rings adjacent to the planet, with troughs exterior to
them.

 In Fig. \ref{vort1d_temporary} we compare the the semi-analytic
results   to the
simulation data, the snapshot being chosen  at the  point when  the rings 
first occupy the complete 
azimuth. The semi-analytic  model reproduces the essential features, 
for example
vortensity peaks and troughs with the  correct relative positions, but 
the distribution is 
slightly shifted towards the planet  
(by $0.2r_h$).
The model does not reproduce  the troughs very well  due to
inadequate modelling of the  pre-shock flow and the shock position. 
\begin{figure}
\center
\includegraphics[trim=0cm 0cm 0cm 1cm,clip,scale=0.33]{sc3_vort1d_.ps}\caption{Theoretical
Shock-modifed vortensity distribution near a
  $M_p=2.8\times10^{-4}$ planet calculated using
the semi-analytic model.
The  solid line is a polynomial fit across the
circulating/librating region.}
\label{sc3_vort1d_v4}
\end{figure}
\begin{figure}
\center
\includegraphics[scale=0.33]{vort1d_temporary.ps}\caption{As in
  Fig. \ref{sc3_vort1d_v4} but as a function of the number of 
  Hill radii away from planet, and
    with a comparision to simulation data.}
\label{vort1d_temporary}
\end{figure}
\section{Dynamical stability of vortensity rings}\label{Dynstab}
Having established the form of the  vortensity rings
 and the mechanism
for producing them, 
we go on to  study the linear stability of the shock-modified
protoplanetary disc model described above.
This is an important issue as instability can lead to their breaking
up into mobile non-axisymmetric structures which can
affect the migration of the planet significantly.

 The linear stability 
of inviscid baratropic  axisymmetric
rings  and discs without a planet 
 is well developed \citep{papaloizou84,papaloizou85,papaloizou89}.
The extension to a 
non-barotropic  equation of state was  undertaken more recently
 \citep{lovelace99,li00}. This work  indicates that  sharply peaked
  surface density or  vortensity features in the  disc  are  asociated with dynamical
instabilities. It is directly relevant to the types of configuration
that we have found to be produced by the disc planet interactions
described above. For example 
\cite{valborro07} considered the linear instability of gap edges
and connected it to  vortex formation there. 

Here we  consider a different
 parameter   for which highly peaked vortensity features appear in
the coorbital (horseshoe)  region. In order to be able to do this
we need to be able to define an appropriate background  equilibrium 
axisymmetric structure
to perturb. We here show that this is possible. 
\subsection{Basic background  state}
 The
basic state   should be axisymmetric and time independent with no radial velocity
($\p/\p\phi=\p/\p t=u_r=0$). To set this up we  suppose the
vortensity profile $\eta(r)$ is known (e.g. via shock modelling as above) 
and that accordingly we have 
\begin{align}\label{vortensity_definition}
\eta(r) = \frac{1}{r\Sigma}\frac{d}{dr}\left(r^2\Omega\right),
\end{align}
The radial momentum equation gives
\begin{align}\label{hydrostatic}
r\Omega^2 = \frac{1}{\Sigma}\frac{dP}{dr} + \frac{GM_*}{r^2}
\end{align}
Using these together with the locally isothermal equation of state,
  $P=h^2GM_*\Sigma/r,$ $h$ being the constant aspect ratio, we obtain a single equation
for $\Sigma$ in the form
\begin{align}\label{basic_density}
h^2\frac{d^2\ln{\Sigma}}{dr^2} = \frac{h^2-1}{r^2} -
\frac{2h^2}{r}\frac{d\ln{\Sigma}}{dr} +
\frac{2\Sigma\eta}{GM_*} \sqrt{\frac{1-h^2}{r}+h^2\frac{d\ln{\Sigma}}{dr}}
\end{align}
We solve Eq. (\ref{basic_density}) for $\Sigma$    with  $\eta(r)$ 
taken as an azimuthal average from the fiducial
simulation described in (\S\ref{fiducial}) at a time at which vortensity rings have
developed. These structures are essentially axisymmetric  
apart from in the close neighbourhood of the planet. They are  illustrated
 in Fig. \ref{vort_055}.
 We solve
Eq. (\ref{basic_density})  subject to  the boundary conditions that $\Sigma=\Sigma_0=1$ at
$r=1.1$, and $r=3.$  These conditions are consistent with the fact that
 shock-modification of the surface density profile only
occurs near the planet ($r=2$).\\
\begin{figure}
\center
\includegraphics[scale=0.50]{vort_055.ps}
\caption{A contour plot of $\ln{\Sigma/\omega}$ when the vortensity ring like structures
have formed in the coorbital region. These are almost axisymmetric apart from in the
region very close to the planet.
\label{vort_055}}
\end{figure}

 A comparison  between hydrostatic surface density  
and angular velocity profiles
 obtained by solving Eq. (\ref{basic_density}) with those obtained  as azimuthal averages from
 the corresponding simulation is illustrated in
Fig. \ref{custom_dens} and Fig. \ref{custom_urad}.  The agreement is generally very good  
indicating that the adoption  of the basic axisymmetric state  defined by the simulation
specific vorticity profile,  together with Eq. (\ref{hydrostatic}),  for stability analysis
should be a valid procedure.    Fig. \ref{custom_dens} shows that  vortensity rings reside 
in the horseshoe region just
inside the gap. At  a surface density extremum Eq. (\ref{basic_density})
implies that
\begin{align*}
h^2\frac{d^2\ln{\Sigma}}{dr^2} = \frac{h^2-1}{r^2} +
\frac{2\Sigma\eta}{GM_*}\sqrt{\frac{1-h^2}{r}}.
\end{align*}  
Since $h\ll1$, if $\eta$ is sufficiently
large then $d^2\Sigma/dr^2 > 0$. Hence vortensity maxima will coincide with
surface density minima.
 In our basic state, local minima and maxima are separated by $O(H)$ ($\simeq
0.1r_p$).
 As vortensity rings originate from
spiral shocks, Eq. ( \ref{basic_density}) demonstrates the  link
between shocks and gap formation. Sufficiently massive planets induce 
strong shocks, implying larger vortensity maxima, and hence deeper
density minima or gaps. 
\begin{figure}
\center
\subfigure[$\Sigma$\label{custom_dens}]{\includegraphics[scale=0.33]{compare2_custom_dens.ps}}
\subfigure[$\Omega/\Omega_k$\label{custom_urad}]{\includegraphics[scale=0.33]{compare2_custom_urad.ps}}
\caption{A comparison of the surface density and angular velocity profiles 
obtained by solving Eq. (\ref{basic_density}) with the same quantities obtained as  azimuthal averages
from the simulation. The vortensity profile common to both approaches is also shown.}
\end{figure}
\subsection{Linearized equations}
\indent We now  obtain the governing equation for locally isothermal
perturbations  by linearizing the  continuity equation and the equation of motion
\begin{align}\label{euler}
&\frac{\p\Sigma}{\p t} + \nabla\cdot{(\Sigma\mathbf{u})} = 0\\
&\frac{\p\mathbf{u}}{\p t} + \mathbf{u}\cdot\nabla\mathbf{u} =
-\frac{1}{\Sigma}\nabla P -\nabla\Phi,\label{momeq}
\end{align}
where $P=c^2\Sigma$   with $c^2=h^2GM_*/r.$ The  effective potential$\Phi$ is
fixed. We  set
\begin{align}
(\Sigma, u_r, u_\phi) \to (\Sigma, 0, u_\phi)+(\delta\Sigma(r), \delta u_r(r), 
\delta u_\phi(r))\times\exp{i(\sigma t + m\phi)},
\end{align}
where, the first term on the right hand side corresponds to
the basic background state, 
 $\sigma$ is a complex frequency and $m,$ the azimuthal mode number,  is a positive
integer. 
The linearised  equation  of motion (Eq. \ref{momeq}) gives
\begin{align}
\delta u_r &= -\frac{h^2}{r(\kappa^2 - \bar{\sigma}^2)}
\left(i\bar{\sigma}\frac{dW}{dr} + \frac{2im\Omega W}{r}\right)\label{velocities1}\\
\delta u_\phi &= \frac{h^2}{r(\kappa^2 - \bar{\sigma}^2)}
\left(\Sigma\eta\frac{dW}{dr} + \frac{m\bar{\sigma}}{r}W\right)\label{velocities2}
\end{align}
where
$W \equiv \delta\Sigma/\Sigma$
is the fractional density perturbation,
$\kappa^2 = 2\Omega\Sigma\eta$
is the epicyclic frequency  expressed in terms of the  vortensity $\eta,$ and
$\bar{\sigma} \equiv \sigma +m\Omega(r) = \sigma_R + m\Omega(r) + i\gamma$ 
is the Doppler-shifted frequency with  $\sigma_R$ and $\gamma$ being real. 


Substituting  Eq. (\ref{velocities1})---(\ref{velocities2}) into
the linearised continuity equation
\begin{align}
i\bar{\sigma} W = -\frac{1}{r\Sigma}\frac{d}{dr}\left(r\Sigma\delta
  u_r\right) - \frac{im}{r}\delta u_\phi
\end{align} 
yields  a  governing equation for $W$  of the form
%\begin{align}\label{goveq}
$$ 
 \frac{d}{dr}\left(\frac{\Sigma}{\kappa^2 -\bar{\sigma}^2}\frac{dW}{dr}\right)
+\hspace{4cm} $$
\begin{align}\label{goveq}
%\frac{d}{dr}\left(\frac{\Sigma}{\kappa^2 -
%    \bar{\sigma}^2}\frac{dW}{dr}\right)+
  \left\{\frac{m}{\bar{\sigma}}\frac{d}{dr}
 \left[\frac{\kappa^2}{r\eta(\kappa^2-\bar{\sigma}^2)}\right]
     -\frac{r\Sigma}{GM_*h^2}
 -\frac{m^2\Sigma}{r^2(\kappa^2-\bar{\sigma}^2)}\right\}W = 0.
\end{align}

This  equation leads to  an eigenvalue problem   for the complex eigenvalue $\sigma.$ 
 Co-rotation 
resonance occurs at $\bar{\sigma} = 0$ which requires
$\gamma =0$ for it to be on the real axis. 
Then for the equation  to remain regular,  the gradient of the  terms in
square brackets must vanish at corotation. This results in the requirement that
the gradient of $\eta r$ vanish there. Because the sound speed varies
with radius, this is slightly different from
the condition that the gradient of $\eta$ should vanish which applies
in the barotropic strictly isothermal case \citep{papaloizou84,papaloizou85,papaloizou89}.
But because  $\eta$ varies vary rapidly in the region of interest and 
 the modes we consider are  locally confined in radius, this difference is of no
essential consequence.
 Linblad resonaces occur at
$\kappa^2-\bar{\sigma}^2 = 0$. However, as is well known, and can be seen from
formulating a governing equation for $\delta u_r$ rather than $W,$
  these do not result in a singularity.

\subsubsection{Simplification of the governing ODE}
\indent It is useful to simplify Eq. (\ref{goveq})  to gain further
insight. To to this we consider  modes localized around the corotation circle
 such that the condition 
$\kappa^2\gg|\bar{\sigma}^2|$ is satisfied. Beyond this region
the mode amplitude is presumed to be exponentially small.
 Now, recognising  that $GM_*h^2/r = c^2$, the
ratio of the second to last to last  term in Eq. (\ref{goveq}) is
\begin{align*}
\frac{r^2\kappa^2}{m^2c^2}\sim\frac{1}{m^2h^2}.
\end{align*}
For a thin disc $h\ll1$, so if we consider $m=O(1)$ this ratio is
large and the last term in Eq. (\ref{goveq})  can be neglected. This is
 also motivated by the fact that only low $m$ modes (vortices)  are
observed in simulations. 
 Doing this and replacing $\kappa^2-|\bar{\sigma}^2|$ by $\kappa^2$,
 Eq. (\ref{goveq}) reduces to the simplified form
\begin{align}\label{goveq2}
\frac{d}{dr}\left(\frac{rc^2\Sigma}{\kappa^2}\frac{dW}{dr}\right)
  +\left\{\frac{m}{\bar{\sigma}}\frac{d}{dr}
 \left[\frac{c^2}{\eta}\right]
     -r\Sigma\right\}W = 0.
\end{align}
We comment that in this form  Eq. \ref{goveq2} is valid
for any fixed $c$  profile.
\subsubsection{Necesity of extrema}
 Mutiplying Eq. \ref{goveq2}
by $W^*$ and intergrating bewteen $[\,r_1,r_2]$ assuming, consistent
with a sharp exponential decay, that  $W=0$ or
$dW/dr=0$ at these  boundaries we find that
\begin{align}\label{neccessary}
\int^{r_2}_{r_1}\frac{m}{\bar{\sigma}}\left(\frac{c^2}{\eta}\right)^\prime|W|^2dr
=\int^{r_2}_{r_1}r\Sigma|W|^2 dr + \int^{r_2}_{r_1}\frac{r\Sigma
  c^2}{\kappa^2}|W^\prime|^2 dr
\end{align}
where derivatives are indicated with a prime. Since the  right hand side is real, 
the imaginary part
of the left and side must vanish. For general complex $\sigma$ this implies that
\begin{align}\label{vortmin}
\gamma\int^{r_2}_{r_1}\frac{m}{(\sigma_R+m\Omega)^2+\gamma^2}
\left(\frac{c^2}{\eta}\right)^\prime|W|^2dr
=0.
\end{align}
 Thus for a growing mode ($\gamma\neq0$) to exist we need
$(c^2/\eta)^\prime =0$ at some $r$ in $[\,r_1,r_2]$. 
For
our disc, $c^2$ varies on a scale  $O(r)$, but $\eta$ varies on  a scale  $H\ll r$, thus given
that the range of relative 
 variation of the vortensity  $\eta$ is of order unity, we infer that this quantity
 needs to  have stationary points in order  for there to be unstable 
 modes. In the baratropic case \cite{papaloizou89} have shown that vortensity
maxima are stable while minima are associated with instabilities. 
 We expect these conclusions to  apply here
also  because of the  local nature of the modes of interest.  We can approximate 
$c^2\sim\mathrm{const.}$,  or equivalently  adopt a barotropic equation of
state locally without changing the character of the problem.
 Referring back to Fig. \ref{custom_dens} it is clear
that  our basic state satisfies the neccessary criterion for
instability.\\
%\begin{figure}
%\center
%\includegraphics[scale=0.25]{F.ps}
%\caption{$F$\label{F}}
%\end{figure}
%% BELOW IS FIRST ATTEMPT, SIMPLE MODEL
%% \indent Let us consider modes with real eigenfrequency $\sigma_R = -m\Omega(r_0)$ such 
%% that $(c^2/\eta)^\prime = 0$ at $r_0$, and growth rate
%% $|\gamma|\ll\Omega_0$ so it may be ignored for the following estimate. Far away
%% from the gap, where vortensity gradients are small the term $r\Sigma W$ imply exponential solutions. In these outer regions we assume 
%% \begin{align}
%% W = \left\{ 
%% \begin{array}{l l}
%%   \exp{\lambda x} & \quad x < 0\\
%%   \exp{-\lambda x} & \quad x > 0\\
%% \end{array} \right.
%% \end{align}
%% where $x\equiv r-r_0$ and $1/\lambda=O(H)$ is the decay length-scale. Exponentials can not be joined smoothly at $x=0$ so 
%% the solutions only apply, say, for $|x|>\delta$. When $|x|<\delta$, vortensity term dominates and we balance
%% \begin{align}\label{goveq2b}
%% \frac{d}{dr}\left(\frac{rc^2\Sigma}{\kappa^2}\frac{dW}{dr}\right)
%%   =-\frac{m}{\bar{\sigma}}\frac{d}{dr}
%%  \left[\frac{c^2}{\eta}\right]W.
%% \end{align}
%% In the vincinity of $x=0$ we approximate
%% \begin{align}
%% \bar{\sigma} &= m(\Omega^\prime_0 x + \Omega^{\prime\prime}_0x^2/2 + \ldots)\\
%% \left(\frac{1}{r\eta}\right)^\prime &= \left(\frac{1}{r\eta}\right)^{\prime\prime}_0 x  + 
%% \left(\frac{1}{r\eta}\right)^{\prime\prime\prime}_0x^2/2 + \ldots 
%% \end{align}
%% Since Eq. \ref{goveq2b} is a second order ODE we specify the boundary conditions $W_0 = 1,\, W^\prime_0 = 0$. The first
%% is due to arbitary normalisation of the eigenmodes; the second for symmetry about $x=0$. Then, evaluating Eq. \ref{goveq2b}
%% at $x=0$ gives
%% \begin{align}
%% \left(\frac{1}{2\Omega\eta}\right)_0 W^{\prime\prime}_0 = -\frac{1}{\Omega^\prime_0}\left(\frac{1}{r\eta}\right)^{\prime\prime}_0,
%% \end{align}
%% where $\kappa^2 = 2\Omega\Sigma\eta$ and $c^2 = h^2/r$ was used. Applying Taylor expansion, the approximate solution is (dropping subscript 0)
%% \begin{align}
%% W &= 1 + K^2x^2,\\
%% K^2 &\equiv - \frac{\Omega\eta}{\Omega^\prime}\left(\frac{1}{r\eta}\right)^{\prime\prime}.
%% \end{align}
%% If the disturbance maximise at $x=0$ we require $K^2<0$. Since $\Omega^\prime<0$ this requires 
%% $(1/r\eta)^{\prime\prime} < 0$, or approximately a vortensity minimum. As $|K^2|$ increase, the disturbance becomes
%% concentrated near $x=0$. Imposing continuity of $W$ and $W^\prime$ at the transition point $x=\pm\delta$ to the exponential 
%% solutions gives 
%% \begin{align*}
%% \delta^2 + \frac{2}{\lambda}\delta + \frac{1}{K^2} = 0,
%% \end{align*}
%% with solution
%% \begin{align}\label{delta}
%% \lambda\delta = -1 + \sqrt{1-\lambda^2/K^2},
%% \end{align}
%% so that $\delta\lambda\to0$ as $|K^2|\to\infty$. As the vortensity profile becomes more extreme, the transition width decreases compared
%% to exponential decay length-scale. However, in performing the analysis it was implicitly assumed that the transition width was small. Hence
%% $-K^2$ needs to be sufficiently large for self-consistent solutions to Eq. \ref{delta}. This means co-rotational modes described above can only
%% exist in discs with sufficiently extreme vortensity profiles. Finally, although the azimuthal wave number $m$ does not appear explicitly, 
%% we have already assumed low $m$ modes in Eq. \ref{goveq2}. \\
%% \indent The vortensity minimum of the inner gap edge, for the standard disc, is at $r_0\simeq1.7$, assuming
%% $\lambda = 1/nH$, Eq. \ref{delta} gives
%% \begin{align*}
%% \lambda\delta \simeq \sqrt{1+0.7/n^2} -1.
%% \end{align*}
%% E.g. if $n=2$ then $\lambda\delta \sim 0.1$. The transition width will typically be a fraction of the local scale height. 
%% \subsubsection{Existence of local modes}     
%% \indent In parts of analysis above we assumed co-rotational modes are
%% localised. We demonstrate this explicitly by searching for non-neutral
%% modes centred about vortensity minimum $r_0=1.7$ of our standard
%% disc. Locally the disc profile is approximated by 
%% \begin{align*}
%% \Sigma &= \Sigma_0 + \Sigma^\prime_0 x ,\\
%% \eta & = \eta_0 +\frac{1}{2}\eta^{\prime\prime} x^2 ,\\
%% \kappa^2 &= \kappa^2_0 + \frac{1}{2}\kappa^{2\prime\prime}_0 x^2,\\
%% \bar{\sigma} &= m\Omega^\prime_0 x +i\gamma,
%% \end{align*}
%% where $x=r-r_0$ and we assumed $\sigma_R + m\Omega_0 = 0$. We checked
%% that vortensity minima corresponds to minima in $\kappa^2$. Writing
%% out Eq. \ref{goveq2} in the standard form $AW^{\prime\prime} + B
%% W^\prime +CW=0$, and expanding the coefficients to zeroth order in $x$ we
%% find (dropping subscript $0$):
%%   \begin{align}  
%%   W^{\prime\prime} + \frac{\Sigma^\prime}{\Sigma}W^\prime
%%   -\frac{\kappa^2}{c^2}W =0,
%%   \end{align}
%%  which has solutions $W\propto\exp{kx}$ with
%%  \begin{align}
%%  k=\frac{1}{2}\left(-\frac{\Sigma^\prime}{\Sigma}\pm
%%    \sqrt{\left(\frac{\Sigma^\prime}{\Sigma}\right)^2 +
%%    4\frac{\kappa^2}{c^2}}\right)  
%%  \end{align}
\subsection{Numerical solution of the eigenvalue problem}
 We  have solved the eigenvalue problem
for the  full equation  (\ref{goveq}) using a 
shooting method  that employs an adaptive Runge-Kutta integrator 
and a  multi-dimensional Newton method \citep{press92}. 
 For low $m$ ($\leq 3$)  unstable modes mainly comprise an evanescent disturbance
 near co-rotation and the simple  boundary condition $W = 0$ applied
at the inner boundary $r/r_p=0.55$ and the outer boundary $r/r_p=1.5$ produces  
good results. 
\begin{figure}
\center
\subfigure[Inner edge]{\includegraphics[scale=0.25]{s1h005_WBC0_m3_in.ps}}
\subfigure[Outer edge]{\includegraphics[scale=0.25]{s1h005_WBC0_m3_out.ps}}
\caption{$m=3$ eigenmodes obtained  with the  boundary condition $W=0.$
The background vortensity profile is also shown.\label{s1h005}}
\end{figure}
As  $m$ increases,  the  Linblad resonances approach  $r=r_p$.
and a  significant portion of the mode is wave-like 
requiring  the application of  outgoing  radiation boundary conditions.   
We determined these  using the  WKBJ  approximation (see eg.  Korycanski \& Pollack 1993). 
\subsubsection{Eigenmode calculations}
We have determined unstable eigenmodes using the above procedures for   $1 \ge m \le ??. $
We recall that the simulations indicate the ultimate  dominance of small $m$ values.
One class of mode is associated with the inner vortensity ring while another
is associated with the outer ring.

 As a typical example of the behaviour that is found for low $m,$ each type  of eigenmode  for  $h=0.05$ and  $m=3$ 
is shown in Fig. \ref{s1h005}. The background vortensity profile is also shown.
The instabilities  are associated with the  vortensity minima at the inner
and outer  gap edge, as has also been 
observed by \cite{li05} in simulations. 
  the modes are evanescent around co-rotation and the  vortensity peaks 
behave like wall through which the instability scarcely penetrates.
 The mode decays away from $r=r_p$. For $m=3$
Lindblad resonances occur at $r_L/r_p=0.76,\,1.21$  from which 
waves travelling away from co-rotation are emitted. 
 However,
the oscillatory amplitude is at most $\simeq 20\%$ of that at $r=r_p$. Hence for  low-$m$ 
the dominant effect of the instability will be due to perturbations near co-rotation. 
Increasing $m$ brings $r_L$ even closer to $r_p$, waves  then propagate through the gap. 
 The growth time-scale of the inner mode with $m=3$ is  $\sim14P_{orb},$
$P_{orb}$ being the orbital period of the planet.  The outer mode
has a growth rate that is about three times faster.  Very similar
results and growth rates were found  for $m=1$  and $m=2$. 


After the onset of linear instability and the formation of several vortices,
it has been observed that non linear effects 
cause them to eventually 
merge into a single vortex (refs).  This eventually interacts with the planet. 
In the fiducial simulation,
rapid migration begins at $55P_{orb}$ which is compatable with the characteristic  growth 
times found  from linear theory. \\
Fig. \ref{s1h005}  indicates that 
the outer edge is more unstable than inner edge. 
The vortensity peaks are of similar
height, but the inner minimum in  $r\eta$  is less pronounced 
 than outer because of the background profile. In this sense the outer edge
profile is more extreme, and hence less stable.

{\bf *****Perhaps a plot for higher m values can be included}
%\subsection{Comparison of inner/outer edges}
%\subsection{Growth rates and azimuthal wave number}
%\subsection{Application to disc-planet problem}
%\ifpdf
%  \pdfbookmark[2]{bookmark text is here}{And this is what I want bookmarked}
%\fi
% ------------------------------------------------------------------------
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Chapter3/_region_.tex <==
\message{ !name(hydro2.tex)}
\message{ !name(hydro2.tex) !offset(-2) }
\section{Nonlinear hydrodynamic simulations}\label{hydro}


We present nonlinear 
hydrodynamic simulations of disc-planet models with $1.2 \leq
Q_o \leq 2$, corresponding to disc masses $0.079M_* \geq M_d \geq
0.047M_*$. Most simulations use a viscosity of $\nu=10^{-5}$
or equivalently $\alpha = O(10^{-3})$, which has been
 typically adopted for protoplanetary discs. 
This value has  also been found to
 suppress vortex instabilities \citep{valborro07}.
We adopt gravitational softening  parameter 
 $\epsilon_{g0}=0.3$. The planet is
set on a fixed circular 
orbit at $r_p=5$ in order  to focus on gap stability.
We briefly explore the effects of varying 
viscosity and softening lengths later in this section and
planetary migration in the next section.  


\subsection{Numerical method}
The hydrodynamic equations are evolved with the FARGO code
\citep{masset00}. FARGO is an explicit finite-difference code similar 
to ZEUS \citep{stone92} but customised for disc-planet interactions. 
It circumvents the time step limit imposed by the rotational velocity
at the inner boundary by splitting the azimuthal velocity into mean
and perturbed parts,  azimuthal transport being   performed on each 
separately. Self-gravity for FARGO was implemented and tested by
\cite{baruteau08}. Two-dimensional self-gravity can be calculated
using Fast Fourier Transform \citep{binney87}. This requires the
radial domain to be logarithmically spaced and doubled in extent. The
planet potential is introduced at $25P_0$ and its gravitational
potential ramped up  over $10P_0$, where $P_0$ is the Keplerian period
at $r=5$. 
%where $P_0=2\pi/\Omega_k(r_p)$ at $t=0$. 


The disc is divided into $N_r\times N_\varphi = 768\times2304$  grid
points in radius 
and azimuth giving a resolution of $\Delta r/H = 16.7$. The grid cells
are nearly square, with $\Delta  r/r\Delta\phi = 1.1$. We impose 
open boundaries at $r_i$ and non-reflecting boundaries at $r_o$
\citep{godon96}. The latter has also been used in the  self-gravitating
disc-planet simulations of \cite{zhang08}. As argued above, 
because edge modes are
physically driven by an internal edge, we do not expect boundary
conditions to significantly affect whether or not they exist. Indeed, 
simulations with open outer boundaries, or damping boundaries \citep{valborro06}
all show development of edge modes.  
%*************
%
%{\bf Have open outer boundaries been considered ??}
%
%************
\subsection{Overview}
We first present an overview of the effect of edge  dominated modes on
disc-planet systems. Fig. \ref{qm_density} shows the relative surface
density perturbation ($\Delta\Sigma/\Sigma$) for $Q_o=1.2,\,1.5$ and
2.0. The profile formed in these cases has local   
$\mathrm{max}(Q)= 3.3, \, 4.2,\,5.3$ near the outer gap edge and the average $Q$ for  $r\in [6,r_o]$ is
$1.6,\,2.0,\,2.6$. Although  the edge mode is associated with the  local
vortensity maximum (located close to  $\mathrm{max}(Q)$ for gap profiles),
it requires coupling to the external smooth disc via
self-gravity. Hence, edge modes only develop if $Q$ in these smooth regions
is sufficiently small, otherwise global disturbances cannot be
constructed.       


The case $Q_o=2.0$ gives a standard result for gap-opening planets,  
typically requiring planetary masses comparable or above that of Saturn. 
For that mass a partial gap of depth $\sim
50\%$ is formed,  a  steady state attained and remains stable to the
end of the simulation. This serves as a stable case for comparison
with more massive discs. This simulation was repeated with
$\nu=10^{-6}$, in which case we identified  both vortex and edge
modes. The standard viscosity $\nu=10^{-5}$ thus suppress both types
of instabilities for $Q_o=2$.  Although we adopted  $\nu=10^{-5}$ to avoid 
complications from vortex modes, we note that they are stabilised 
for sufficiently massive  discs anyway (e.g. $Q_o=1.5,\, \nu=10^{-6}$ do not show
vortices, see section \ref{motivation}). 


Gap edges become unstable for $Q_m\leq 1.5$ when $\nu= 10^{-5}.$
As implied by linear analysis, the $m=2$ edge mode
dominates when  $Q_o=1.5$ and it  saturates by $t=100P_0.$
It is more prominent in the outer disc, and over-densities deform the gap edge
into an eccentric ring.  The under-density in the gap also becomes  more
non-axisymmetric, being deeper where the gap is wider.  
%away from the high density wakes produced by the planet.
The inner disc remains fairly circular, though non-axisymmetric disturbance ($m=3$) 
can be identified. 
Note the global nature of the edge modes in the outer
disc: spiral arms can be traced back to disturbances at the gap edge
rather than the planet. Consider the spiral disturbance at the outer
gap edge just upstream of the planet where $\Delta\Sigma/\Sigma$ is
locally maximum. Moving along this spiral outwards,
$\Delta\Sigma/\Sigma$ reaches a local minimum at $(x,y)=(6,-4)$ before
increasing again. This is suggestive of the outer disc spirals being
induced by the edge disturbance.  


When the effect of  disc self-gravity is increased to the 
$Q_o=1.2$ case,  there is significant
disruption to the outer gap edge, it is no longer clearly
identifiable. The $m=1$ edge mode  becomes  dominant in the outer
disc, although overall it  still appears to carry  an $m=2$
disturbance because of the perturbation due to the planet.
The inner disc becomes
visibly eccentric with an $m=2$ edge mode disturbance. The shocks due
to edge modes can comparable strength to those induced by the planet. 

\begin{figure*}
\centering
%\subfigure[$Q_m=2.0$]{
\includegraphics[width=0.32\textwidth,clip=true,trim=1.5cm 0cm 0cm 0cm]{figures/v1NRBCnu5_polar_dens050.ps}%}  
%\subfigure[$Q_m=1.5$]{
\includegraphics[width=0.32\textwidth,clip=true,trim=1.5cm 0cm 0cm 0cm]{figures/v3NRBCnu5_polar_dens050.ps}%}
%\subfigure[$Q_m=1.2$]{
\includegraphics[width=0.32\textwidth,clip=true,trim=1.5cm 0cm 0cm 0cm]{figures/v4NRBCnu5_polar_dens050.ps}%} 
%\subfigure[$Q_m=1.0$]{\includegraphics[width=0.23\textwidth]{v2NRBCnu5_polar_dens050.ps}}  
\caption{Surface density perturbations (relative to $t=0$) at
  $t\sim 100P_0$ as a function the minimum value of Toomre $Q$ in the
  disc, $Q_o$. From left to right: $Q_o=2.0,\,1.5,\,1.2$. 
\label{qm_density}}
\end{figure*}

%\begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth]{figures/m2_growth_outer.ps} 
%  \caption{Running-time averaged amplitude of the $m=2$ mode in the
%    outer disc, as a function of initial minimum Toomre $Q$. 
%    \label{m2_growth}}
%\end{figure}

\subsection{Development of edge modes for  $Q_o=1.5$}
%m=2 amp is 1\% of axisymmetric mode

We examine the  fiducial case  with $Q_o=1.5.$
 Fig. \ref{Qm1.5_nonlin1} shows the development of the
edge instability.
 The final dominance of $m=2$ is consistent with linear
calculations.
 The planet opens a well-defined gap by $t\sim 40P_0$, or 
$\sim 5P_0$ after the planet potential  $,\Phi_p,$ has been  fully 
ramped up. At  $t\sim 46P_0,$ two over-dense blobs, associated with the 
edge mode  can be  identified at the outer gap
edge. At this time the gap has $\Delta\Sigma/\Sigma \simeq -0.3$, implying
edge modes can develop \emph{during} gap
formation, since the steady state stable gap in $Q_o=2$ reaches
$\Delta\Sigma/\Sigma \simeq -0.6.$ 
Edge modes are global  and are associated with
long trailing spiral waves  with density perturbation  amplitudes
that are  not small compared to
that at the gap edge.
This is clearly seen at  $t\sim 50P_0$ when spiral
shocks have already developed.
We estimate that the edge modes have a growth rate 
consistent with predictions from linear theory and   become non-linear
within the time frame  $46P_0 < t < 50P_0.$


The edge perturbations  penetrate the 
outer gap edge and trail  an angle  similar to the planetary wake.
Notice the $m=3$ disturbance near $r=4$ in 
the snapshots taken at $t=50P_0$ and $t=56P_0.$  Two of the three
over-densities, seen as a function of azimuth,
correlate to the $m=2$ mode in the outer disc, while the third  over-density
adjacent to the planet correlates with the outer planetary wake. 
These features result from self-gravity and are unrelated to vortex modes.  

The presence of both planetary wakes (with pattern speed $\simeq
\Omega_k(5)$) and edge modes (with pattern speed $\simeq 
\Omega_k(5.5)$) of comparable amplitude enable direct interaction between them.% They have comparable amplitudes. 
Passage of edge mode
spirals through the planetary wake may disrupt the former, explaining some of the 
apparently split-spirals in the plots. 
% when 
%the edge disturbance passes through the planetary shock, it may become less effective
% in maintaining the disturbance in the smooth disc. increased pressure in edge disturbance
% making it more vortex type, less gravity? 
%When a spiral just passes through the planetary wake. 
%An example of this is the apparently disjointed spiral arm just upstream
%of the planetary wake at $t\sim 58P_0.$ 
%We typically find this feature when the other
%spiral has just passed through the planetary wake, so the disjointed part of the 
%upstream spiral may be due to disruption 
At 
$t\sim 64P_0$  Fig. \ref{Qm1.5_nonlin1} indicates  that a 
spiral density wave feature coincides with the
(outer) planetary wake. 
%for which over-density is enhanced relative to  
%to when the spiral does not coincide with the wake in the two
%subsequent snapshots.  
The enhanced outer planetary wake implies an  increased negative torque 
exerted on the planet at this time. 
%However, since the spiral and planet are differentially
%rotating, 
This effect occurs during the  overlap of positive
density perturbations. Assume that  at a fixed radius the
edge mode spiral has azimuthal thickness $nh$ where $n$ is a
dimensionless number. The time taken for this spiral to cross the
planetary wake is $  \Delta T = nh/|\Omega_k(5.5) -
  \Omega_k(5)| \simeq 0.06nP_0$. This is $\ll P_0$ for $n=O(1)$. We
expect such crossing spiral waves  to induce  associated  oscillations in the 
disc-planet torque. 


The non-linear evolution of edge modes in disc-planet systems can give
complicated surface density fields. The gap can  become  highly 
deformed.  Fig. \ref{Qm1.5_nonlin1} shows that  large voids develop to
compensate for the over-densities  in spiral 
arms, leading to  azimuthal gaps ($t=64P_0$). 
At $t=72P_0$, the gap width ahead of the planet is narrowed by the
spiral disturbance at the outer edge trying to connect  to that at the 
inner edge. 
%Because the edge modes are driven by self-gravity,
%they may try to close the gap in the radial direction because
%over-densities on either side of the gap attract gravitationally. 
However, this gap-closing effect is opposed by the planetary  torques
which tend to open it. %The edge mode disturbance 
%and planetary wake have comparable amplitudes. 


A quasi-steady state is reached by $t\geq 76P_0$  showing an eccentric
gap. For $t=99.5P_0$ additional contour lines are
plotted to indicate  two local surface density maxima along the edge mode
spiral adjacent to the planet. This spiral is disjointed around
$r\sim7.5$ where on traversing an arm,  there is a minimum in $\Delta\Sigma/\Sigma$.
 Taking co-rotation of the spiral at $r_c=5.5$ gives the
outer Lindblad resonance of an  $m=2$ disturbance at $r=7.2,$ assuming  a
Keplerian disc. This is within the disjointed region of the spiral
arm, which supports our interpretation that the disturbance at the
edge is driving activity in the outer disc by perturbing it
gravitationally and launching waves at outer Lindblad resonances. 

\begin{figure*}
  \centering
  \includegraphics[scale=0.47          ,clip=true,trim=0cm
  1.83cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens020b_ver2.ps}
  \includegraphics[scale=0.47                 ,clip=true,trim=2.34cm
  1.83cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens023b_ver2.ps}
  \includegraphics[ scale=0.47                  ,clip=true,trim=2.34cm
  1.83cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens025b_ver2.ps}
  \includegraphics[ scale=0.47                  ,clip=true,trim=2.34cm
  1.83cm 0cm 0cm]{figures/v3NRBCnu5_polarxy_dens029b_ver2.ps}
  \includegraphics[scale=0.47       ,clip=true,trim=0cm
  0cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens032b_ver2.ps}
  \includegraphics[scale=0.47                 ,clip=true,trim=2.34cm
  0cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens036b_ver2.ps}
  \includegraphics[ scale=0.47                  ,clip=true,trim=2.34cm
  0cm 1.645cm 0cm]{figures/v3NRBCnu5_polarxy_dens038b_ver2.ps}
  \includegraphics[ scale=0.47                  ,clip=true,trim=2.34cm
  0cm 0cm 0cm]{figures/v3NRBCnu5_polarxy_dens050b_ver2.ps}
  \caption{Evolution of  the surface density perturbation 
(relative to $t=0$ ) for the $Q_o=1.5$
    case from $t\sim 40P_0$ to $t\sim 100P_0$.   
    \label{Qm1.5_nonlin1}}
\end{figure*} %disc mass is $M_d=0.063M_*$. 


% Figure \ref{Qm1.5_nonlin} show several snapshots of the surface
% density perturbation in polar co-ordinates to show the global disc
% structure more easily. 
% After $t\gtrsim 70P_0$, the spiral mode has saturated. It is no
% longer two distinct spirals attached to the outer gap edge but exists
% as two azimuthally extended cresents, each with a trailing spiral. The
% spirals associated with the instability and that of the planet have
% similar magnitudes, so we expect their effect on the disc to be
% comparable to that by the planet.

% The snapshot at $t=80P_0$ demonstrates an eccentric gap with 
% apsidal line nearly $\pi$ radians relative to the planet's
% azimuth. This eccentricity results from non-constant gap width as a
% function of azimuth due to deformation of the outer gap edge (the
% inner edge remains circular). The over-density associated with spirals
% results in the gap adjacent to them being thinner. This 
% suggests that the presence of these spirals opposes the tendency of 
% the planet potential to push material away to open a gap. 
% %Conversely, the absence of spiral over-densities result in wider
% %gaps. 

% The final snapshot at $t=116P_0$ shows the apsidal line of the
% eccentric outer gap edge has precessed relative to the planet,
% otherwise the remaining features are indifferent to that in
% $t=80P_0$, the gap-spiral system has reached a quasi-steady state.  

\subsubsection{Eccentric gaps}
Several snapshots of the  $Q_o=1.5$ run  
taken during  the second half of the simulation are
shown in Fig. \ref{Qm1.5_ecc}, which  display  the precession of an
eccentric outer gap edge. Deformation of a  circular
gap into an eccentric one requires an $m=1$  disturbance.
{\bf By comparison with the stable case of $Q_o=1.5$
  (see Fig. \ref{qm_density}), we see that edge modes are 
 associated with the visibly eccentric gaps. However, the
 inner gap edge remain fairly circular. 
}
%The $m=2$ edge mode is present,  but sometimes obscured by the planetary
%wake.
%Defining the outer gap edge 
%as the locus of points where $\Delta\Sigma/\Sigma = 0$ and fitting an
%ellipse with eccentricity $e_\mathrm{edge}$ \footnote{This is a geometric
%measure rather than a specific  particle path.} we find for $Q_o=1.5$
%$e_\mathrm{edge}=0.3$---0.4 whereas for $Q_o=2$ it is
%$e_\mathrm{edge}=0.1$.
In their non-self-gravitating disc-planet simulations, \cite{kley06}
found  eccentric discs can result for planetary masses $M_p > 3M_J$
fixed on circular orbit. Our simulations show that edge modes in a
self-gravitating disc can provide an additional perturbation to deform
the gap into an eccentric shape for lower mass planets.  


 \begin{figure}
   \centering
   \includegraphics[width=0.25\textwidth,clip=true,trim=1cm 0cm 0cm 0cm]{figures/v3NRBCnu5_polar_dens072.ps}\includegraphics[width=0.25\textwidth,clip=true,trim=1cm 0cm 0cm 0cm]{figures/v3NRBCnu5_polar_dens088.ps} 
   \includegraphics[width=0.25\textwidth,clip=true,trim=1cm 0cm 0cm 0cm]{figures/v3NRBCnu5_polar_dens091.ps} 
 % \subfigure{\includegraphics[width=0.45\textwidth]{v3NRBCnu5_alpha_plot2.ps}} 
   % \subfigure{\includegraphics[width=0.45\textwidth]{ecc_plot_Qm1d2_to_2.ps}}
   \caption{Precession of an eccentric gap in the
     presence of an $m=2$ edge mode for a disc with  $Q_o=1.5.$ 
     \label{Qm1.5_ecc}}
 \end{figure}

\subsection{  Evolution of the gap structure  for  $Q_o=1.2$}
%m=2 amp is 1\% amplitude

With increasing disc mass,  evolution of the gap profile away from its original form
takes place. Fig. \ref{Qm1.2} illustrates  the emergence of the $m=3$ edge
mode, expected from linear calculations, and subsequent
evolution of the gap profile. 
By $t\sim 42P_0$ the $m=3$ edge mode has already become non-linear,
whereas for  $Q_o=1.5$ the $m=2$ mode only begins to emerge at
$t\sim 44P_0,$ being consistent with linear calculations that the former has
almost twice the growth rate of the latter. In Fig. \ref{Qm1.2} 
there is a  $m=3$ spiral at $r<r_p$ in phase with the
mode for  $r>r_p.$ The gap narrows where they almost touch. These are
part of a single mode.
By  $t=44P_0,$   shocks  have formed   and  
extend continuously across the gap.  The   self-gravity of the disc
 has overcome the planet's gravity which is responsible for
gap-opening. Edge mode spirals can be more prominent than planetary wakes. 


The evolution of the form  of the gap  is shown  in  the one-dimensional  averaged profiles
plotted in Fig. \ref{Qm1.2}. The quasi-steady  profile before the onset 
of the edge mode  instability is 
 manifest  at
$t\sim 40P_0.$ 
By $t=44P_0$, the original bump at $r=6$  has
diminished. This bump originates from the planet expelling
material as it opens a gap but is subsequently `undone' by the edge
mode as it grows and attempts to connect across the gap. This gap
filling effect is  possible as non axisymmetric 
perturbation  of the inner disc  may be induced via the outer  disc self-gravity.
Notice also in Fig. \ref{Qm1.2}
at $t=44P_0$ the increased surface density at $r\simeq7.5$ implying
radial re-distribution of material.
 By $t=120P_0$, the inner
bump ($r=4$) is similar to that produced by a  standard gap-opening planet. By
contrast, the outer bump cannot be maintained. The gap widens and
there is an overall increase in surface density for $r>6.5$. Note that
there is no additional  diminishing  of the outer edge bump from
$t=44P_0\to120P_0$.  %saturation

%Assuming a co-orbital region of $r_p\pm
%2.5r_H$ where $r_H$ is the Hill radius, we expect a gap in the region
%$r=[4.42,5.58]$. The edge mode has co-rotation at $r=5.5$ (vortensity
%maxima).  


Although  the $m=3$  mode emerges first and is predicted to be most unstable from
linear analysis, it does not persist. Linear theory can only predict the initially 
favoured mode. In the nonlinear regime, Fourier analysis shows that
$m=2$ becomes dominant for  $60P_0 \ga t \ga 145P_0$.  
We suspect this be due to  finite viscosity acting over this time-scale. 
Larger $m$ means  shorter  radial wavelengths, so
over given a time-scale, diffusion and hence stabilisation by viscosity is
more effective than smaller $m$. The evolution is  also 
complicated by the planetary wake which may gravitationally interact with edge modes. 
For $Q_o=1.2$ we found that $m=1$ becomes dominant at $t\ga145P_0$ when
there appears to be a coupling between the outer planetary wake and
the edge mode. 

%However, very long simulations may be significantly affected by boundary issues. 

% Hence, $m=2$ takes over, despite having smaller linear
%growth rates than $m>3$.  %well, these m>3 modes may not be edge modes anyway (weaker SG in response) 

%However, linear calculations
%showed the next most unstable mode after $m=3$ is $m=4$, which is not
%observed. We suspect the discrepency may  be due to the  finite viscosity acting
%over this time-scale. Increasing $m$ leads to  shorter  radial wavelengths, so
%over given a time-scale, diffusion and hence stabilisation by visocisty is
% more effective. 

%Linear theory is only able  to predict what mode should  first
%emerge.  The non-linear evolution is  complicated by the
%planetary wake which may gravitationally interact with edge modes. For
%$Q_o=1.2$ we found that $m=1$ becomes dominant at $t\geq145P_0$ when
%there appears to be a coupling between the outer planetary wake and
%the edge mode.

\begin{figure}
   \centering
   \includegraphics[scale=0.3,clip=true, trim=1cm 0cm 3.3cm
   0cm]{figures/v4NRBCnu5_polar_dens021.ps}\includegraphics[scale=0.3,clip=true, trim=1cm 0cm 0cm 
   0cm]{figures/v4NRBCnu5_polar_dens022.ps} 
   \includegraphics[width=0.45\textwidth]{figures/v4NRBCnu5_compare_profiles_dens020b.ps} 
   
   \caption{ The disc model with  $Q_o=1.2$: emergence of the $m=3$ edge mode (top) and
     evolution of the gap profile (bottom). 
     \label{Qm1.2}}
 \end{figure}
{\bf vortensity discussion

}
\begin{figure}
   \centering
   \includegraphics[width=0.45\textwidth,clip=true,trim=0cm 0cm 0cm 1cm]{figures/v4NRBCnu5_compare_profiles_dens020b_ver2_vortensity.ps}
   \caption{ The disc model with  $Q_o=1.2$: evolution of gap profile
     in terms of azimuthally averaged vortensity $\eta$. 
     \label{Qm1.2_vortensity}}
 \end{figure}


\subsection{Mass transport}
The similarity between the effects induced by an  edge mode and an external
perturber (planet) is further illustrated   by the induced  mass transport.
Just as when a  planet opens a gap, the development of an  edge disturbance   results
in a  radial re-distribution of  mass.  We 
express the angular momentum transport  in terms of an $\alpha$
viscosity parameter, defined through  $\alpha = \Delta u_r\Delta u_\varphi/c_s^2$, where
$\Delta$ here denotes deviation from the  azimuthal average.

Angular momentum is also transmitted  through  gravitational torques.
However, in practice we found  this to be a  small effect  compared to
transport  due to Reynolds stresses. The discs here are not gravito-turbulent. 
The azimuthally averaged $\alpha$ parameters $\langle\alpha\rangle$  are shown in
Fig. \ref{masstrans}. The stable disc with $Q_o=2$ is shown for
reference as in this case non-axisymmetric features
are entirely induced by the planetary perturbation and
$\langle\alpha\rangle$ is localised about the planet's
orbital radius giving a trough at $r_p$ and peaks either
side.

Increasing self-gravity  by adopting $Q_o=1.5$, we see that angular momentum  transport is
enhanced around $r_p$ and $r<4$, signifying the global nature of 
edge modes. Towards the inner boundary, $\alpha\simeq 10^{-3}$ for
$Q_o=1.5$ and is  twice as large as in the case  $Q_o=2.$  $Q_o=1.5$ also has enhanced
wave-like behaviour for  $r>7$ when compared to $Q_o=2.0.$ 

The $Q_o=1.2$ case is more dramatic, with $\langle\alpha\rangle$ reaching
$O(10^{-2})$, which is an order of magnitude larger than the value corresponding to the imposed
physical viscosity. This case also displays a trough at  about
$r=5.5$, i.e. edge mode co-rotation, as if another planet were
placed there. 
%In later snapshots we found the dip located  with  $r\in [6,7]$ to
%further develop, because the tips of the edge mode spirals are pushed
%outwards by gravitational torques due to the planet and the disc.
However, compared to $Q_o=1.5$,  there is
no enhanced transport away from the gap region. 


Fig. \ref{masstrans} also shows the  evolution of  the disc mass as a function of time, $M_d(t)$. 
Viscous
evolution leads to mass loss ($Q_o=2.0$) and there is clearly enhanced
mass loss if edge modes develop ($Q_o=1.2,\,1.5$). For $t\leq 50P_0$
the curves are identical, this interval includes gap formation and
the emergence of edge modes. When edge modes become non-linear,
mass loss is enhanced ($t\simeq 50P_0$), but there is no significant
difference between $Q_o=1.2,\,1.5$, which is consistent with the
previous $\langle \alpha\rangle $ plots near the inner boundary. The $Q_o=1.2$ curve
is non-monotonic, though still decreasing overall, possibly because
of boundary effects, and mass loss is enhanced once more around
$t=125P_0$. As $Q_o$ is lowered, mass loss becomes less smooth,
showing the dynamical nature of edge modes. 


\begin{figure}
   \centering
   \includegraphics[width=0.99\linewidth]{figures/alpha_plot2.ps}  
%   \includegraphics[width=0.32\linewidth]{figures/alpha_plot2_t80.ps} 
   \includegraphics[width=0.99\linewidth]{figures/masstrans_plot2_discmass.ps} 
   \caption{Top: azimuthally averaged Reynolds stresses associated with edge modes 
     when they become non-linear ($Q_o=1.2,\,1.5$), the $Q_o=2$ case
     is shown as a stable case with no edge modes for
     comparison. Bottom: evolution of the total disc mass for the three cases, scaled by initial mass.  
     \label{masstrans}}
 \end{figure}



\subsection{Additional effects}
We briefly discuss effects of softening and viscosity on edge modes. To analyse mode
amplitudes, the surface density field is Fourier transformed in azimuth giving
$a_m(r)$ as the (complex) amplitude of the $m^{\mathrm{th}}$ mode. 
We then integrate over the outer disc $r>5$ to get $C_m =\int a_m dr$ 
and consider $A = C_m/C_0$.  


\subsubsection{Softening}
In linear theory we found that edge modes cannot be constructed for
gravitational softening parameters that are too large. We have
simulated the $Q_o=1.5$ disc with
$\epsilon_{g0}=0.6,0.8,\,1.0$. \footnote{It should be remarked that increasing
$\epsilon_{g0}$ makes the Poisson kernel in simulations increasingly
non-symmetric, so the earlier analytical discussion is less applicable.}  

Fig. \ref{vsoft} shows the evolution of the running-time averaged $m=2$ amplitudes. 
The evolution for all cases is very similar for $t\leq
40P_0$. Unstable modes develop thereafter, with increasing growth rates
and saturation levels as $\epsilon_{g0}$ is lowered.
$\epsilon_{g0}=1$ displays either no growth or  a  much reduced growth rate. 
The gap for $Q_o=1.5,\,\epsilon_{g0}=1.0$ reaches a steady state
similar to the stable case with $Q_o=2.0,\,\epsilon_{g0}=0.3$.  This is
consistent with the fact that as softening weakens, edge disturbances
can no longer perturb the remainder of the disc via self-gravity, 
the residual non axisymmetric structure being due to the planetary perturbation. 
Interestingly, the decrease in
saturation level in going from $\epsilon_{g0}=0.3\to0.6$ is smaller than going from
$\epsilon_{g0}=0.6\to0.8$, which is in turn smaller than $\epsilon_{g0}=0.8\to1.0$,
despite a larger relative increase in softening in one pair than the next.  

%indicating a threshold value for edge modes

\begin{figure}
   \centering
   \includegraphics[width=0.45\textwidth]{figures/pattern_plot2_vsoft_outer.ps} 
   \caption{Running-time average of the surface density $m=2$ Fourier amplitude, integrated over
     $r\in[5,10]$ and scaled by the axisymmetric component, 
     for the $Q_o=1.5$ disc, as a function of the  gravitational softening
     length. 
%{\bf What was plotted here..if it was a Fourier amplitude it should depend 
%on radius}
     \label{vsoft}}
 \end{figure}



\subsubsection{Viscosity}
An important difference between edge dominated  modes and the already
well-studied vortex modes in planetary gaps is the effect of
viscosity on them. The standard viscosity $\nu=10^{-5}$ prevents vortex mode
development, but we have seen in \S\ref{motivation} that such
viscosity values still allow the $m=2$ edge modes to develop. Vortices are
localised disturbances and more easily smeared out than global spirals
in a given time interval. Hence, vortex growth is inhibited more
easily by viscosity than spirals. 

We repeated the $Q_o=1.5$ runs  with a range of viscosities. Results are
shown in Fig. \ref{vvisc}. Generally, lowering viscosity 
increases the amplitudes of the non-axisymmetric modes.
For $\nu\leq 10^{-6}$, the $m=3$  mode emerges first 
(note that this is not in conflict with our linear calculations 
which used $\nu=10^{-5}$ in its basic state), rather than $m=2$.  
This is because lowering viscosity allows a sharper vortensity peak to develop in the background model, 
and thus has the same effect as increasing the disc mass. 
%The latter
%increases the most unstable $m$. 
The latter can enable higher $m$ edge modes. 


Unlike vortex modes, even with twice the standard viscosity
($\nu=2\times10^{-5}$) the edge mode develops and grows. It is only
is suppressed when $\nu\geq5\times
10^{-5}$. However, this is because no vortensity maxima could be setup
at the gap edges due to vortensity diffusion in the co-orbital region
 making an almost uniform vortensity distribution in the gap. Since
the necessary condition for edge modes is not achieved, no linear
modes exist. This differs  from the nature of the suppression of vortex modes, because in
that case vortensity extrema that are stable can still be setup. 
\begin{figure}
   \centering
   \includegraphics[width=0.45\textwidth]{figures/pattern_plot2_vvisc.ps} 
   \caption{Non-axisymmetric disc modes 
%    {\bf *** What exatly has been plotted here?**}
     for the $Q_o=1.5$ disc as a function of applied
     viscosity $\nu$. The Fourier amplitude has been integrated over $r\in[5,10]$
	and scaled by the axisymmetric amplitude and its running-time average plotted. 
     Thick lines indicate the $m=2$ mode and is
     plotted for all $\nu$. Thin lines indicate the $m=3$ mode and is
     plotted for $\nu=10^{-7}$---$10^{-5}$ only. 
     \label{vvisc}}
 \end{figure}


\section{Applications to disc-planet systems}\label{disc-planet}
In order to focus on the issue of the stability of the dip/gap
in the surface density profile induced by a giant planet,
the planet was held on a fixed orbit.
However, torques exerted by the non axisymmetric disc
on the planet will induce migration that could occur
on a short time scale \citep[eg.][]{peplinski08b}.
Such torques  will be significantly affected by the presence
of edge modes.
Accordingly, we now discuss  the torques
exerted by a  disc, in which edge modes are excited,  on the planet.

\subsection{Disc-planet torques}
%The simulations described above show that effects due to 
%edge modes can be as prominent as
%wakes induced by the planet. 
The presence of large-scale edge mode spirals of comparable
amplitude as the planetary wake will significantly modify the torque 
on the planet, which in a stable disc is the origin of disc-planet 
torques. 
%Since  torques exerted on the planet
%by the disc  originate
%from these wakes, the presence of large-scale spirals of comparable
%amplitude will affect them.  
Here, we measure the disc-planet
torque but still keep the planet on fixed orbit.


Fig. \ref{Qm1.5_torques}(a) shows
the evolution of the 
torque per unit length  for the $Q_o=1.5$ fiducial case. 
The
torque profile at $t=40P_0,$ before the edge modes
have developed significantly,  shows the outer torque is larger in
magnitude than inner torque, implying inward  migration. This is a
typical result for disc-planet interactions and serves as a  reference. 
At $t=60P_0$ and $t=100P_0$, edge modes mostly modify the  torque contributions
exterior to the planet, though some disturbances are seen in the
interior disc ($r-r_p<-5r_h$, $r_h$ being the Hill radius). 
The original outer torque at $+r_h$, is reduced in magnitude as material
re-distributed to concentrate around the  co-rotation radius $r_c$ of the edge mode.
($r_c$ is $\sim2r_h$ away from the planet). 
%The voids between edge mode
%spirals means that, except when spirals are near the planet, the
%surface 

Edge modes can both enhance or reduce disc-planet
torques associated with planetary wakes. Consider 
$r-r_p\in [3,5]r_h$ in 
Fig. \ref{Qm1.5_torques}(a).
 Comparing the situation at $t=60P_0$ to that at 
$t=40P_0$, the torque contribution from this region is seen to be  more
negative. This is because  an edge mode spiral overlaps the
planetary wake and therefore contributes an  additional negative torque on
the planet.
 However, at $t=100P_0$, an edge mode spiral is just upstream of the
planet,  exerting  a positive torque on the planet, hence the torque
contribution from  $r-r_p\in [3,5]r_h$ becomes positive. 

Differential rotation between edge modes and the planet produces
oscillatory torques, shown in Fig. \ref{Qm1.5_torques}(b). Unlike typical
disc-planet interactions, which produce inward  migration, the total
instantaneous torques in the presence of edge modes can be of either
sign. For a disturbance with $m$ fold symmetry the time interval between
encounters with the planet is $\Delta T = (2\pi/m)/\dd\Omega$, where
$\dd\Omega$ is the difference in angular velocity of the planet and
the disturbance pattern.  Approximating $\delta \Omega =
|\Omega_k(r_p) - \Omega_k(r_c)|$ with $r_c=5.46$ obtained from linear theory, we
obtain $\Delta T = 4.04P_0$. Indeed, the oscillation period in
Fig. \ref{Qm1.5_torques} is $\simeq 4P_0$. %better match early on.
Both inner and outer torques oscillate, but since the edge mode is
more prominent in the outer disc, oscillations in the outer torque are
larger, particularly after mode saturation ($t>70P_0$).
%hence it modifies the outer torque more

\begin{figure*}
   \centering
\includegraphics[width=0.33\textwidth]{figures/v3NRBCnu5_torque_plot_text.ps}
\includegraphics[width=0.33\textwidth]{figures/v3NRBCnu5_torque2_notaper_text.ps}
\includegraphics[width=0.33\textwidth]{figures/torque2_begavg25_notaper_text.ps} 
   \caption{(a) Disc  torque per unit radius acting on the planet.
      The length scale
     $r_h=(M_p/3)^{1/3}r_p$ is the Hill radius.
     (b) Time dependent evolution of the disc planet torques, the  contribution
        from the inner disc (dotted curve), the
     outer disc (dashed curve) and the  total torque (solid curve).
     (c) The running  time average of the total
      torque acting on the planet  as a function of $Q_o.$  
     \label{Qm1.5_torques}}
 \end{figure*}

We compare time-averaged torques in Fig. \ref{Qm1.5_torques}(c). In
all three cases,  on average a negative torque acts on the planet and its magnitude
largest at $t=40P_0$. % or $5P_0$ after the planet potential is
%switched on and the gap is formed. 
Up to this point, the  torque becomes more negative as the disc mass increases, as expected.
%Although, the magnitude  increases slightly
%faster than linear (it increases by a factor $1.5$ as $Q_o$ decreases
%by a factor $1.3$). 
%In the stable disc with $Q_o=2.0$ the torque reaches a steady
%value. 
However, development of edge modes makes the averaged torques more
positive, and eventually reverses the trend with $Q_o$.  While the disc
with $Q_o=1.5$ also attains steady torque values as in $Q_o=2$, the disc with
$Q_o=1.2$ has significant  oscillations
even after time-averaging and is remains  non-steady at the end of the run. 

Before the
instability sets in, torques arise from wakes induced by the planet,
and the outer (negative) torque is dominant. Edge modes concentrate
material into spiral arms, leaving voids in between. Therefore, except
when spiral arms  cross the planet's azimuth, the surface density in 
the planetary wake is reduced because it resides in the void in between edge mode
spirals. Hence the torque magnitude is
reduced. If the reduction in surface density due to edge mode voids is
greater than the increase in surface density scale produced 
by decreasing $Q_o,$ the  presence of edge modes will, 
on average make the torque acting on the planet more positive.


%THERE MIGHT ALSO BE POSITIVE CO-ROTATIONAL TORQUE DUE TO EDGE MODE TIP MATERIAL CROSSING PLANET 
%(HORSESHOE EFFECT). THIS MAY ALSO CONTRIBUTE TO MAKING THE TORQUE MORE POSITIVE. BUT THESE ACT ON VERY SHORT
%TIME-SCALES. 


%\begin{figure}
%   \centering
%   \includegraphics[width=0.45\linewidth]{figures/torque2_begavg25_notaper.ps} 
%   \caption{Running-time average of disc-on-planet torques in the
%     $Q_m=1,2,\,1.5$ and 2.0 disc. The difference between these curves
%     are not significantly affectd by whether or not material inside
%     the planet's Hill radius is accounted. 
%     \label{torque_evol}}
% \end{figure}


\subsection{Outward scattering by spiral arms}
If edge modes develop, planetary migration may be affected by them.
 Their association with gap edges inevitably affects co-orbital
flows. While a detailed  numerical study of migration is
deferred to future work, we highlight an interesting effect found when
edge modes are present. This is \emph{outward} migration induced through scattering
by spiral arms. 

We restarted some of the simulations described  above
 at $t=50P_0$  allowing the planet
to move in response to the gravitational forces due to the disc.
 The  equation of motion of the planet  is
integrated using a fifth order Runge-Kutta
integrator\footnote{\cite{lin10} found the same integrator to be 
 adequate for studying migration induced through
 scattering by vortices}. Fig. \ref{orbit3_rp} shows the orbital radius of the
planet in discs with edge modes present. %\footnote{A plot of the 
% semi-major axis woukd be  similar
%because eccentricities $e$ are never  large, 
% reaching  almost $0.1$ during scattering, but typically being  a few per cent.}
 No obvious trend with
$Q_o$ is shown. This is because of oscillatory torques due to edge modes and
the partial gap associated with a Saturn mass planet, which is associated
with  type III migration \citep{masset03}. The initial direction of migration can
be inwards or outwards depending on the relative positioning  of the  edge mode
spirals with respect to the planet at the time
the planet was first allowed to move. 

Outward  migration is seen for $Q_o=1.3$ and $Q_o=1.5.$  
For $Q_o=1.5$, the planet migrates by $\Delta r = 2$, or 8.6 times its
initial Hill radius, within only $4P_0.$  This is essentially the result of  a
scattering event. %and is a form of type III migration. 
Repeating this run with  tapering applied to  contributions 
to disc torques from
within $0.6r_h$ of the planet, we found outward  scattering still
occurs, but limited to $\Delta r = 1$ and the planet remains at
$r_p\simeq 6$ until $t=128P_0$. Hence, while the subsequent inward
migration seen for  $Q_o=1.5$ may be associated with
 conditions close to the planet,
the initial outward scattering is due to an exterior edge mode spiral. 


For $Q_o=1.3$ the planet is scattered to $r_p\simeq 8$.  
It is interesting to note that the subsequent
inward migration for $Q_o=1.5$ and $Q_o=1.3$ stalls at $r\simeq6$, i.e. the
original outer gap edge. The planet remains there for sufficient time for
both gap and edge mode development and for $Q_o=1.3$ a second episode of
outward scattering occurs 
(it also occurs for $Q_o=1.5$ to a small extent around $t=70P_0$).   
%outwards-inwards migration disrupts outer disc 
Interaction with edge modes can affect
the disc well beyond the original co-orbital region of the planet. In the
case of outward  migration, it may promote gravitational activity in
the outer disc. However, boundary effects may be important after
significant outward scattering.  
%, where its
%co-orbital region will extend to $r_p+2.5r_h\simeq 9$, close to the
%outer boundary. 


\begin{figure}
   \centering
   \includegraphics[width=0.45\textwidth]{figures/orbit3_rp.ps} 
   \caption{Orbital radius evolution in discs with edge mode
     disturbances. The instantaneous orbital radius $r_p$ is shown as a
     function of time.
     \label{orbit3_rp}}
 \end{figure}


The spiral arm-planet interaction for $Q_o=1.5$ above is detailed in
Fig. \ref{Qm1.5_scatter}.
% As a spiral arm approaches the planet from
% upstream ($t=115.1P_0$), it exerts a positive torque on the planet,
% increasing $r_p$. The spiral itself loses angular momentum and reduces
% its orbital radius (gets closer to the planet). Notice the asymmetric
% gap about the planet's azimuth, this signifies type III migration. 
% %The spiral is more prominent than the planetary
% %wake.    
% As this edge spiral passes through the planetary wake ($t=116.3P_0$), an
% over-density builds up upstream, a pair of disturbances is identified.
% A new edge mode is being setup. The upstream disturbance grows but
% executes an horseshoe turn across $r_p$, imparting positive angular
% momentum to the planet, promoting it to larger orbital radius. By
% $t=118.5P_0$ the edge mode is reformed (with the edge disturbance at
% the original gap edge, $r=6$). In effect, the edge spiral scatters the
% planet outwards.  
A spiral arm approaches the planet from the
upstream direction ($t=50.9P_0$) and exerts  positive torque on the planet,
increasing $r_p$. The gap is asymmetric in the azimuthal direction
with the surface density upstream  of the planet being larger
than that downstream of the planet ($t=51.5P_0$).
 As the spiral arm  passes through the
planetary wake ($t=51.5P_0$---$52.1P_0$) the gap surface density just
ahead of the planet builds up as an edge mode is setup across the
gap. Notice the fluid blob at $r=5,\,\varphi-\varphi_p=0.3\pi$. This
signifies material executing horseshoe turns ahead of the planet. 
At the later time $t=53.1P_0$ the planet has exited the original gap, in
 which the
average surface density is now higher than before the scattering.
 Material that was originally outside
the gap loses angular momentum and moves into the original gap. This
material is not necessarily that composing the spiral. 


We remark that migration  through  scattering by spiral arms  differs from
 vortex
scattering \citep{lin10}. Vortices form about vortensity minima, which
lie further from the planet than vortensity maxima. We can assume
vortensity maxima are  stable in the case of vortex formation. This
means the ring of vortensity maxima must be disrupted in order for
vortices to flow across the planet's orbital radius for direct
interaction. Edge modes themselves correspond to a  disruption of
vortensity maxima, hence direct interaction is less hindered than in  the
vortex case. Furthermore, a vortex is a material volume of fluid. Vortex-planet 
scattering results in an  orbital radius change of both objects.
 A spiral pattern is generally not a material volume of fluid.  It can be seen
in Fig. \ref{Qm1.5_scatter} that the local $\mathrm{max}(\Sigma)$ in the spiral remains  at
approximately the same radius before and after the
interaction. The spiral as a whole does not move inwards. In this
case, the spiral first increases  the  planet's orbital radius, thereby
encouraging it to interact with the outer gap edge and scatter that
material inwards. %This material then reforms 
%into an edge mode. 


\begin{figure}
   \centering
   \includegraphics[scale=0.4, clip=true, trim=0cm 1.85cm 0cm
   0cm]{figures/M2nu5bHT_polarxy_dens034.ps}\includegraphics[scale=.4,clip=true,trim=2.2cm 1.85cm 0cm 0cm]{figures/M2nu5bHT_polarxy_dens039.ps}\\
   \includegraphics[scale=.4,clip=true,trim=0cm 0cm 0cm 0cm]{figures/M2nu5bHT_polarxy_dens045.ps}\includegraphics[scale=.4,clip=true,trim=2.2cm 0cm 0cm 0cm]{figures/M2nu5bHT_polarxy_dens054.ps} 
   \caption{Interaction between an edge mode spiral and the planet (green dot), 
	causing the latter to be scattered outwards. $\log\Sigma$ is shown. 
     \label{Qm1.5_scatter}}
 \end{figure}





\message{ !name(hydro2.tex) !offset(-865) }


==> Chapter3/analytic.tex <==
\section{Analytical discussion of edge modes}\label{analytic}
The fiducial disc is massive with
$M_d\sim 0.06M_*$ but it is still stable against gravitational
instabilities in the sense that $Q\geq 1.5$ everywhere.  The
intermediate-mass planet of Saturn is expected to only open a partial
gap, but even this is sufficient to trigger the $m=2$ spiral
instability. The fiducial case above thus suggest that spiral modes
may develop under not very extreme conditions, such as those
considered by \cite{meschiari08}.  We devote this section and the next
to a theortical discussion of spiral modes associated with planetary
gap edges. This  work is based on the governing equation for linear
perturbations of the Euler equations. Perturbations are assumed to
have a form $f(r)e^{i(\sigma t + m\phi)}$ where $\sigma$ is the
complex eigenfrequency and $m$ is the azimuthal wave-number taken to
be a positive integer. 

We first give an analytical description of the edge modes. For
analytical discussion it is convenient to assume a barotropic equation
of state, where the integrated pressure
$p=p(\Sigma)$ and the soundspeed $c_S^2\equiv dp/d\Sigma$). The
governing equations are
\begin{align}\label{barotropic}
  r\dd\Sigma = &\frac{d}{dr}\left[\frac{r
      \Sigma}{D}\left(\frac{dS}{dr}\right)\right]  
  + \left[\frac{2m}{\bar{\sigma}}\frac{d}{dr}
    \left(\frac{\Omega\Sigma}{D }\right)
    -\frac{m^2\Sigma}{rD}\right]S,\notag\\
  S = &c_s^2 W + \dd\Phi.
\end{align}
In the above expressions, $\Sigma, \, \Omega$ are
the surface density and angular speeds respectively,
$D\equiv \kappa^2 - \bar{\sigma}^2$ where $\kappa$ is the background
epicyclic frequency and $\bar{\sigma} = \sigma + m\Omega$ is the
shifted frequency. The perturbation variables are 
\begin{align*}
  W &= \dd\Sigma/\Sigma\\
  \dd\Phi & =  - G\int K_m(r,\xi)\xi\dd\Sigma(\xi)d\xi,
\end{align*}
with
\begin{align*}
  K_m(r,\xi) &= \int \frac{\cos(m\phi)d\phi}{\sqrt{r^2+\xi^2 -
      2r\xi\cos{(\phi)}+ \epsilon_g^2(\xi)}},
\end{align*}
where $\dd\Sigma, \, \dd\Phi$ is the Eulerian surface density and
gravitational potential perturbations respectively. The latter arises
from self-gravity. Integrations here are taken over the entire disc.
$\epsilon_g$ is a softening parameter. Hydrodynimal and linear
calculations specifically employ $\epsilon_g(r) = \epsilon_0 h r$ 
where $\epsilon_0$ is a dimensionless constant with fiducial value
0.3, and $h = H/r$ is the disc aspect-ratio. We have ignored indirect
potentials and viscosity.    

An alternative form of Eq. \ref{barotropic} given by
\cite{papaloizou91}:

\begin{align}\label{barotropic2}
r\dd\Sigma &= \frac{d}{dr}\left[\frac{r\Sigma}{D}\left(\frac{dS}{dr} +
    \frac{2m\Omega\bar{\sigma}S}{r\kappa^2}\right)\right]
-\frac{2m\Omega\bar{\sigma}\Sigma}{\kappa^2D}\left(\frac{dS}{dr} + 
  \frac{2m\Omega\bar{\sigma}S}{r\kappa^2}\right)  
+ \frac{mS}{\bar{\sigma}}\frac{d}{dr}\left(\frac{1}{\eta}\right) -
\frac{4m^2\Omega^2\Sigma S}{r\kappa^4},
\end{align}
where $\eta = \kappa^2/2\Omega\Sigma$ is the vortensity. This form
shows that co-rotation singularity $\bar{\sigma}$ can be avoided if
co-rotation corresponds to a vortensity extremum, making the ODE
regular. 


\subsection{Preliminaries}
We first derive expressions for angular momentum flux within the framework of
linear theory. We begin with the linearised equation of motion for the
Lagrangian displacement $\bm{\xi}$ in three dimensions given by
\cite{lin93b}, modified for a barotropic equation of state and
including self-gravity: 
\begin{align}\label{lagrangian}
  \frac{\p^2\bm{\xi}}{\p t^2} + 2\Omega\hat{\bm{z}}\wedge\frac{\p\bm{\xi}}{\p
    t} + 2im\Omega\frac{\p\bm{\xi}}{\p t} = -\nabla S -
  r\hat{\bm{r}}\left(\bm{\xi}\cdot\nabla\Omega^2\right) +
  m^2\Omega^2\bm{\xi} - 2im\Omega^2\hat{\bm{z}}\wedge\bm{\xi} - \nabla\Phi_\mathrm{ext},
\end{align}
where $\Phi_\mathrm{ext}$ is an external potential to assist the
identification of angular momentum flux later on. Taking the dot
product of $\rho\bm{\xi}^*$ and Equation \ref{lagrangian} and
subtracting off the complex conjugate of the same quanitity, we obtain:
\begin{align}
  \frac{\p}{\p t}\left\{\Im{\left[\rho\bm{\xi}^*\cdot\frac{\p\bm{\xi}}{\p t}
        +\rho\Omega\bm{\xi}\wedge\bm{\xi}^* +
        im\rho\Omega |\bm{\xi}|^2\right]}\right\} =&
    -\Im{\left(\rho\bm{\xi}^*\cdot\nabla S\right)} -
  \Im{\left(\rho\bm{\xi}^*\cdot\nabla \Phi_\mathrm{ext}\right)}\\\notag
  =& -\Im{\left[\nabla\cdot\left(\rho\bm{\xi}^* S\right)\right]} +
  \Im{\left[S\nabla\cdot\left(\rho\bm{\xi}^*\right)\right]} -
  \Im{\left(\rho\bm{\xi}^*\cdot\nabla \Phi_\mathrm{ext}\right)}.
\end{align}
Using the linearised continuity equation followed by the Poisson
equation on the second term on RHS, we obtain:
\begin{align}\label{angmomcons}
  &\frac{\p}{\p t}\left\{\Im{\left[\rho\bm{\xi}^*\cdot\frac{\p\bm{\xi}}{\p t}
        +\rho\Omega\bm{\xi}\wedge\bm{\xi}^* +
        im\rho\Omega |\bm{\xi}|^2\right]}\right\} +
  \Im{\left[\nabla\cdot\left(\rho\bm{\xi}^* S\right)\right]} 
  +\Im{\left[\nabla\cdot\left(\frac{1}{4\pi
          G}\dd\Phi\nabla\dd\Phi^*\right)\right]}\notag\\  
  &= - \Im{\left(\rho\bm{\xi}^*\cdot\nabla \Phi_\mathrm{ext}\right)}.
\end{align}
Eq. \ref{angmomcons} corresponds to angular momentum conservation. To 
see this, consider the external potential. The torque per unit volume
due to this potential is $-\rho\p_\phi\Phi_\mathrm{ext}$. Hence, the
(real) torque per unit volume associated with the perturbed density
field is:
\begin{align}
 T =
 -\Re{(\dd\rho)}\Re{\left(\frac{\p\Phi_\mathrm{ext}}{\p\phi}\right)}. 
\end{align}
We assume a $\exp{im\phi}$ dependence of perturbed variables and the
external potential. Then, defining the azimuthal average of some
quantity $q$ as
\begin{align*}
\langle q \rangle \equiv \frac{1}{2\pi}\int_0^{2\pi} q d\phi,
\end{align*}
we have:
\begin{align*}
\langle T \rangle &\equiv \frac{m}{2\pi}\int_0^{2\pi}
\Re{(\dd\rho)}\Im{\left(\Phi_\mathrm{ext}\right)}
d\phi\\\notag
& = \frac{m}{2}\Im{(\dd\rho^*\Phi_\mathrm{ext})}. 
\end{align*}
Performing azimuthal average on the RHS term of Eq. \ref{angmomcons}:
\begin{align}
  -\Im\left\langle \rho\bm{\xi}^*\cdot\nabla
        \Phi_\mathrm{ext} \right\rangle  = -
  \Im\left\langle \nabla\cdot\left(
        \rho\bm{\xi}^*\Phi_\mathrm{ext}\right)\right\rangle -
  \underbrace{\Im\left\langle\dd\rho^*\Phi_\mathrm{ext}\right\rangle}_{2\langle T \rangle/m}.    
\end{align}
Hence, the azimuthally averaged Eq. \ref{angmomcons} reads:
\begin{align}\label{angmomcons2}
  \frac{\p\rho_J}{\p t} + \nabla\cdot(\bm{F}_A + \bm{F}_G +
  \bm{F}_\mathrm{ext}) = \langle T\rangle,
\end{align}
where:
\begin{align}
  \rho_J &\equiv -\frac{m}{2} \rho
  \Im{\left[\bm{\xi}^*\cdot\frac{\p\bm{\xi}}{\p t} +
      \Omega\bm{\xi}\wedge\bm{\xi}^* + 
        im\Omega |\bm{\xi}|^2\right]} \\
\bm{F}_A &= -\frac{m\rho}{2}\Im{(\bm{\xi}^*S)} \\
\bm{F}_G &= -\frac{m}{2}\Im{\left(\frac{1}{4\pi
      G}\dd\Phi\nabla\dd\Phi^*\right)} \\
\bm{F}_\mathrm{ext} &=
-\frac{m\rho}{2}\Im{(\bm{\xi}^*\Phi_\mathrm{ext})}.
\end{align}
Since $\langle T\rangle$ is a torque density and Eq. \ref{angmomcons2}
has the standard form of a conservation law, we conclude that $\rho_J$
is the angular momentum density and the $\bm{F}$'s are angular
momentum flux. Specifically, $\bm{F}_A$ is the flux due to advection, 
$\bm{F}_G$ is the flux due to self-gravity and $\bm{F}_\mathrm{ext}$
is the flux associated with the external potential. Note that
self-gravity affects the angular momentum flux indirectly through
$\bm{F}_A$ via $S$ and it appears explicity in $\bm{F}_G$. In the
absence of external forcing, Eq. \ref{angmomcons2} says the rate of
change of angular momentum inside some volume is just due to the
angular momentum flux into or out of the volume.

To obtain the conservation law for razor-thin geometry, we set $\rho =
\Sigma \dd(z)$,  integrate vertically and and ignore external
potentials. This gives the
conservation law with radial fluxes:
\begin{align}
  F_A &= -\frac{m\Sigma}{2}\Im{(\xi_r^*S)}\\
  F_G &= -\frac{m}{2}\Im\int_{-\infty}^{\infty} \frac{1}{4\pi G}
  \dd\Phi\frac{\p\dd\Phi^*}{\p r} dz\label{gravflux}
\end{align}
It is neccessary to account for the three-dimensional nature of the
perturbed potential, even though we are aiming for razor-thin disc geomtry. 

We can obtain an explicit expression for $F_A$ in terms of the
fundamental perturbation $S$. The radial Lagrangian displacement is
\begin{align}
  \xi_r &= -\frac{1}{D}\left(S^\prime +
    \frac{2mS\Omega}{r\bar{\sigma}}\right)\\\notag
  &=-\frac{1}{D}\left(S^\prime + \frac{2m\Omega S
      \sbar}{r\kappa^2}\right) - \frac{2m\Omega S}{r\sbar\kappa^2}.
\end{align}
hence
\begin{align}\label{advflux}
  F_A &\equiv -\frac{m\Sigma}{2}\Im{(\xi_r^*S)}\\\notag
  &= \frac{m\Sigma}{2}\Im{\left(\frac{1}{D^*}SS^{\prime*} +
      \frac{2m|S|^2\Omega}{r\bar{\sigma}^*D^*}\right)}
  = \frac{m\Sigma}{2}\Im\left[\frac{1}{D^*}\left(SS^{\prime *} +
      \frac{2m\Omega|S|^2\sbar^*}{r\kappa^2}\right) +
    \frac{2m\Omega|S|^2}{r\kappa^2\sbar^*}\right]  
\\\notag
  &=\frac{m\Sigma}{2|D|^2}\left\{[\kappa^2 -
      (\bar{\sigma}_R^2-\gamma^2)]\left[\Im(SS^{\prime*}) +
      \frac{2m\Omega \gamma |S|^2}{r|\bar{\sigma}|^2}\right]  
- 2\gamma\bar{\sigma}_R\left[\Re (SS^{\prime*}) +
    \frac{2m|S|^2\Omega\bar{\sigma}_R}{r|\bar{\sigma}|^2}\right]\right\}.  
\end{align}
The second and third equalities will become useful later. 
In the limit $\gamma\to 0$ and hence $\bar{\sigma}$ being real, we
have
\begin{align}
  F_{A,\gamma\to 0} = \frac{m\Sigma}{2D}\Im{(SS^{\prime*})}.
\end{align}

It is useful to relate the gravity flux to $\dd\Sigma$. To see this, begin
with the linearised Poisson equation for razor-thin geometry:
\begin{align}
  \nabla^2\dd\Phi = 4\pi G \dd\Sigma\dd(z).
\end{align}
At this point the potential is regarded as three
dimensional. Multiplying the above by $\dd\Phi^*$ and taking imaginary
parts,
\begin{align}
\nabla\cdot\left[\Im\left(\frac{1}{4\pi
      G}\dd\Phi^*\nabla\Phi\right)\right] =
\Im[\dd\Sigma\dd\Phi^*\dd(z)],
\end{align}
or 
\begin{align*}
-\frac{m}{2}\nabla\cdot\left[\Im\left(\frac{1}{4\pi
      G}\dd\Phi \nabla\Phi^* \right)\right] = \nabla\cdot\bm{F}_G =
\frac{m}{2}\Im[\dd\Sigma\dd\Phi^*\dd(z)]. 
\end{align*}
Integrating the above vertically assuming $\dd\Phi\to0$ as $z\to\pm\infty$
\begin{align}
\frac{1}{r}\frac{\p}{\p r} r F_G = \frac{m}{2}\Im(\dd\Sigma\dd\Phi^*),
\end{align}
where $F_G$ is the vertically integrated radial gravity flux
(Eq. \ref{gravflux}). The potential is now evaluated at $z=0$. Hence, 
\begin{align}\label{gravflux2}
  \frac{2}{m}\left[rF_G\right]_{r_1}^{r_2} = \Im \int_{r_1}^{r_2}
  r\dd\Sigma \dd \Phi^* dr = \Im \int_{r_1}^{r_2} r\dd\Sigma S^* dr.
\end{align}
The last equality will be useful later. 

\subsubsection{Reynolds flux}
For completeness we also derive the Reynolds flux in terms of $S$. The
Reynolds flux (or stress) is
\begin{align}
  F_R \equiv r\Sigma \left\langle \Re{(\dd u_\phi)}\Re{(\dd u_r)}\right\rangle.
\end{align}
Note that this is simply a definition, unlike the advective or gravity
fluxes which were derived from first principles. From the
linearised momentum equations we have:
\begin{align}
\Re(\dd u_r) = & \Re\left\{\frac{1}{D}\left[-i\left(\bar{\sigma}S^\prime
      + \frac{2m\Omega S}{r}\right)\right]\right\}\\\notag
=& \Re\left(\frac{1}{D}\right)\left(\bar{\sigma}_R\Im{(S^\prime)} +
  \gamma\Re{(S^\prime)} + \frac{2m\Omega}{r}\Im{(S)}\right)\\\notag
+&\Im\left(\frac{1}{D}\right)\left(\bar{\sigma}_R\Re{(S^\prime)} -
  \gamma\Im{(S^\prime)} + \frac{2m\Omega}{r}\Re{(S)}\right).\\
\Re(\dd
u_\phi)= &\Re\left[\frac{1}{D}\left(\frac{\kappa^2}{2\Omega}S^\prime +
    \frac{m\bar{\sigma}}{r}S\right)\right]\\\notag
 = &
\Re\left(\frac{1}{D}\right)\left[\frac{\kappa^2}{2\Omega}\Re(S^\prime)
  + \frac{m}{r}\left(\bar{\sigma}_R\Re(S) -
    \gamma\Im(S)\right)\right]\\\notag
-& \Im\left(\frac{1}{D}\right)\left[\frac{\kappa^2}{2\Omega}\Im(S^\prime)
  + \frac{m}{r}\left(\bar{\sigma}_R\Im(S) +
    \gamma\Re(S)\right)\right].
\end{align}
Recall that peruturbed variables are assumed to have the form
\begin{align}
  S = [p(r) + iq(r)]\exp{im\phi},
\end{align}
where $p,\,q$ are real functions. Then we have the following
identities:
\begin{align*}
&\avg{\Re(S)\Im(S)} = \avg{\Re(S^\prime)\Im(S^\prime)} = 0,\\
&\avg{\Re(S)\Im(S^\prime)} =-\avg{\Re(S^\prime) \Im(S)} =-\frac{1}{2}\Im(SS^{\prime *}),\\
&\avg{\Im(S^\prime)\Im(S)} =\avg{\Re(S^\prime)\Re(S)} =\frac{1}{2}\Re(SS^{\prime *}),\\
&\avg{\Re(S^\prime)\Re(S^\prime)} = \avg{\Im(S^\prime)\Im(S^\prime)}=
\frac{1}{2}|S^\prime|^2,\\
&\avg{\Re(S)\Re(S)} = \avg{\Im(S)\Im(S)}=
\frac{1}{2}|S|^2.
\end{align*}
After some algebra, we find the Reynolds flux is
\begin{align}
  F_R = \frac{r\Sigma}{2|D|^2}\left[\frac{m}{r}\left(\kappa^2 -
      |\bar{\sigma}|^2\right)\Im(SS^{\prime *})
    +\frac{\gamma\kappa^2}{2\Omega}|S^\prime|^2 - \frac{2\gamma m^2\Omega}{r^2}|S|^2\right].
\end{align}
In the limit $\gamma\to 0$ and hence $\bar{\sigma}$ being real, we
have
\begin{align}
  F_{R,\gamma\to 0} = \frac{m\Sigma}{2D}\Im(SS^{\prime *}).
\end{align}
Coincidentally, this is the same expression as the advective flux in
the same limit. 

\subsection{Angular momentum flux balance}
The angular momentum flux associated with perturbations can be related
to the background vortensity profile. For this discussion we use
the governing equation in the form given by Eq.\ref{barotropic2}
\citep{papaloizou91}. Multiplying this equation by $S^*$ and
integrating, we get
\begin{align}\label{angmom_balance}
  \int_{r_1}^{r_2} r\dd\Sigma S^* dr &=
  \left[\frac{r\Sigma}{D}\left(S^*S^\prime +
    \frac{2m\Omega\bar{\sigma}}{r\kappa^2}|S|^2\right)\right]_{r_1}^{r_2} -
  \int_{r_1}^{r_2} \frac{r\Sigma}{D}|S^\prime|^2 dr - \int_{r_1}^{r_2}
  \frac{2m\Omega\bar{\sigma}\Sigma}{\kappa^2 D}\left(SS^{\prime *} +
    S^*S^\prime\right)dr \\\notag &-\int_{r_1}^{r_2}
  \frac{4m^2\Omega^2\Sigma|S|^2}{r\kappa^2D}dr + \int_{r_1}^{r_2}
  \frac{m|S|^2}{\bar{\sigma}}\left(\frac{1}{\eta}\right)^\prime dr. 
\end{align} 
% The imaginary part of the LHS is related to the gravity flux
% (Eq. \ref{gravflux2}). Taking the imaginary part of
% Eq. \ref{angmom_balance} gives: 
% \begin{align}\label{angmom_balance2}
%   \frac{2}{m}\left[rF_G\right]_{r_1}^{r_2} & =
%   \left[r\Sigma\Im\left(\frac{S^*S^\prime}{D}\right)\right]_{r_1}^{r_2}  
% + \left[\frac{2m\Omega\Sigma|S|^2}{\kappa^2}\Im\left(\frac{\bar{\sigma}}{D}\right)\right]_{r_1}^{r_2}  
% -  \Im \int_{r_1}^{r_2} r\Sigma |S^\prime|^2\left(\frac{1}{D}\right)
% dr \\\notag &
% - \Im \int_{r_1}^{r_2} \frac{2m\Omega\Sigma}{\kappa^2}\left(SS^{\prime *} +
%     S^*S^\prime\right) \left(\frac{\bar{\sigma}}{D}\right)dr \\\notag &-\Im\int_{r_1}^{r_2}
%   \frac{4m^2\Omega^2\Sigma|S|^2}{r\kappa^2}\left(\frac{1}{D}\right)
%   dr + \Im\int_{r_1}^{r_2} m|S|^2\left(\frac{1}{\eta}\right)^\prime \left(\frac{1}{\bar{\sigma}}\right) dr. 
% \end{align}
Using the Eq. \ref{advflux}, the imaginary part of the first term on
RHS can be expressed in terms of the advective flux: 
\begin{align}\label{advflux2}
  \Im\left[\frac{r\Sigma}{D}\left(S^*S^\prime +
      \frac{2m\Omega\bar{\sigma}}{r\kappa^2}|S|^2\right)\right] =
  -\frac{2}{m}rF_A - \Sigma\Im\left(\frac{2m\Omega|S|^2}{\sbar\kappa^2}\right).
\end{align}
Hence, taking the imaginary part of Eq. \ref{angmom_balance} and
noting the term on LHS results in the gravity flux(Eq. \ref{gravflux2}),
\begin{align}\label{angmom_balance2}
  \frac{2}{m}\left[rF_G\right]_{r_1}^{r_2}  = &
  -\frac{2}{m}\left[rF_A\right]_{r_1}^{r_2} -
    \left[\Sigma\Im\left(\frac{2m\Omega|S|^2}{\sbar\kappa^2}\right)\right]_{r_1}^{r_2} 
    -\Im\int_{r_1}^{r_2} r\Sigma |S^\prime|^2 \left(\frac{1}{D}\right) dr     
\\\notag &
- \Im \int_{r_1}^{r_2} \frac{2m\Omega\Sigma}{\kappa^2}\left(SS^{\prime *} +
    S^*S^\prime\right) \left(\frac{\bar{\sigma}}{D}\right)dr \\\notag &-\Im\int_{r_1}^{r_2}
  \frac{4m^2\Omega^2\Sigma|S|^2}{r\kappa^2}\left(\frac{1}{D}\right)
  dr + \Im\int_{r_1}^{r_2} m|S|^2\left(\frac{1}{\eta}\right)^\prime \left(\frac{1}{\bar{\sigma}}\right) dr. 
\end{align}
% We need explicit expressions for imaginary parts of complex
% quantities above. Recall that $D = \kappa^2  - \bar{\sigma}^2$ and
% that $\sbar = \sbar_R + i\gamma$, then
% \begin{align*}
% &\Im\left(\frac{1}{\bar{\sigma}^*D^*}\right) =
% \frac{\gamma}{|\sbar|^2|D|^2}\left(\kappa^2 - 3\sbar_R^2 +
%   \gamma^2\right) \\
% &\Im\left(\frac{\sbar}{D}\right) = \frac{\gamma}{|D|^2} \left(\kappa^2
%   + \sbar_R^2 + \gamma^2\right)\\
% &\Im\left(\frac{1}{D}\right) = \frac{2\gamma\sbar_R}{|D|^2}\\
% &\Im\left(\frac{1}{\sbar}\right) = -\frac{\gamma}{|\sbar|^2}.
% \end{align*}
A simple relation between the total angular momentum flux
($F_T = F_A + F_G$) and the vortensity profile can be obtained in the limit
$\gamma\to0$ {\bf and  no Lindblad resonances}. First consider the case with
co-rotation resonance such that $r_1<r_c<r_2$, where $r=r_c$ is such
that $\sbar_R = 0$ there. As we let $\gamma\to0$, terms in
Eq. \ref{angmom_balance2} that involve $\sbar/D$ and $1/D$
vanish in the limit $\sbar$ is real. Then at this stage, 
Eq. \ref{angmom_balance2} reduces to
\begin{align}
\frac{2}{m}\left[rF_T\right]_{r_1}^{r_2} & =  
-\left[\frac{ 2m\Omega \Sigma
    |S|^2}{\kappa^2}\Im\left(\frac{1}{\sbar}\right)\right]_{r_1}^{r_2} 
+ 
\Im \int_{r_1}^{r_2} m|S|^2\left(\frac{1}{\eta}\right)^\prime
\left(\frac{1}{\bar{\sigma}}\right) dr\\\notag
& = -\left[\frac{ m 
    |S|^2}{\eta}\Im\left(\frac{1}{\sbar}\right)\right]_{r_1}^{r_2} 
+ 
\Im \int_{r_1}^{r_2} m|S|^2\left(\frac{1}{\eta}\right)^\prime
\left(\frac{1}{\bar{\sigma}}\right) dr.
\end{align}
where we have combined the advective and gravity
fluxes. Now, if $r_1,\,r_2$ are away from $r_c$ so that at boundary
points, $|\sbar|\neq 0 $ in the limit $\gamma\to0$, the first term on
RHS vanishes. This is simply saying that $\sbar$ is real at the
boundary points. However, 
because the integration range includes co-rotation, the second term on 
RHS is non-vanishing in the limit $\gamma\to0$. We are
left with
\begin{align}\label{angmom_balance3}
\frac{2}{m}\left[rF_T\right]_{r_1}^{r_2} & = \Im
\int_{r_1}^{r_2} m|S|^2\left(\frac{1}{\eta}\right)^\prime
\left(\frac{1}{\bar{\sigma}}\right) dr\\\notag & =\Im \int_{r_1}^{r_2} 
\frac{m|S|^2}{|\sbar|^2}\left(\frac{1}{\eta}\right)^\prime (-i\gamma) dr. 
\end{align}
Assuming $\gamma$ is vanishingly small but negative (marginally
unstable mode), we can use the Landau prescription and set $1/\sbar =
P(1/\sbar) + i\pi\dd(\sbar),$ with $P$ denoting that the principal
value is to be taken when the expresion is inside integrals,  to find
\begin{align*}
\frac{2}{m}\left[r F_T\right]_{r_1}^{r_2} = \left.\frac{\pi
    |S|^2}{|\Omega^\prime|}\left(\frac{1}{\eta}\right)^\prime\right|_{r_c}\equiv -T_c
\end{align*}

%If we set $r_2$ such that $F(r_2)=0$ (e.g. vanishing surface density
%at the outer boundary) then 
%\begin{align*}
%- \frac{2}{m} r_1 F_T(r_1) = \left.\frac{\pi
%    |S|^2}{|\Omega^\prime|}\left(\frac{1}{\eta}\right)^\prime\right|_{r_c},
%\end{align*}

so we see that if co-rotation lies exactly at a vortensity extremum,
then there is no net angular momentum flux through $[r_1,r2]$, i.e. no
co-rotation torque. However, if
$(1/\eta)^\prime_{r_c} < 0$ then there is a positive torque. %flux through
%$r_1$ towards co-rotation. 

In the steps leading to the simple relation between angular momentum
flux and vortensity profile, we are effectively arguing that for small
$|\gamma|$, the largest contribution to the flux is from the
vortensity integral. This term contains $1/\sbar$, and near
co-rotation $|\sbar|\sim |\gamma|$ so $1/|\sbar|$ can be
large. Imaginary parts of other terms (boundary or integral) are
proportional to $\gamma$ so they have small contributions. 

We note that if the integration range excludes co-rotation,
i.e. $r_1,\,r_2 < r_c$ or vice versa, then $r_1 F_T(r_1) = r_2
F_T(r_2)$. In other words, the angular momentum flux is some constant
on either side of co-rotation. It is important to remember that the
above analysis is only valid in the limiting case $\gamma\to0_-$. 


{\bf ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK ASK} 

We now include Lindblad resonances. The co-rotation integral is
treated as before. In the limit of $\gamma\to0$, there is a singular
term due to $D\to 0$ at Lindblad resonances
($\kappa = \sbar_R$ at ILR and $\kappa = -\sbar_R$ at OLR). Again
considering $\gamma$ to be vanishinly small and negative, we use the
Landau prescription
\begin{align*}
  \frac{1}{D} = P\left(\frac{1}{D}\right) + 
  \frac{i\pi}{2\kappa}\left[\dd(\kappa+\sbar) -\dd(\kappa - \sbar)\right], 
\end{align*}
with $P$ here again denoting that a principal value is to be taken
\citep{papaloizou89}. Angular momentum flux balance now reads
\begin{align}
  &\frac{2}{m}[rF_T]_{r_1}^{r_2} = -T_L - T_c\\\notag
  &T_L = \Im\int_{r_1}^{r_2}\frac{\Sigma}{r}\left[r^2 |S^\prime|^2
    + \frac{2m\Omega r\sbar}{\kappa^2}(SS^{\prime *} + S^*S^\prime) +
    \frac{4m^2\Omega^2|S|^2}{\kappa^2}\right]\\\notag &\times\left\{P\left(\frac{1}{D}\right) 
  +\frac{i\pi}{2\kappa}\left[\dd(\kappa+\sbar) -\dd(\kappa -
    \sbar)\right]\right\}dr.
 \end{align}
We have neglected boundary terms by assuming $\sbar$ is real at
$r_1,\,r_2$. We regard $\sbar$ on the numerator to be real.
Picking up contributions to the integrals only from the
poles, we have
\begin{align}
  &T_L = T_{OLR} + T_{ILR},\\\notag
  &T_{OLR} = \left(\frac{\pi\Sigma}{2\kappa r |m\Omega^\prime +
    \kappa^\prime|}\left|rS^\prime - \frac{2m\Omega
      S}{\kappa}\right|^2\right)_{OLR},\\\notag
&T_{ILR} = \left(\frac{-\pi\Sigma}{2\kappa r |m\Omega^\prime -
    \kappa^\prime|}\left|rS^\prime + \frac{2m\Omega
      S}{\kappa}\right|^2\right)_{ILR}.
\end{align}
In the case where there is zero net flux across the entire system and
co-rotation is exactly at vortensity extremum, angular momentum is
lost from the ILR and gained at OLR, this shows outwards transport of
angular momentum without solving the governing equation.  

\subsection{Analogy with disc-planet system}
Our goal here is to demonstrate the resemblence of self-excited modes
associated with edges in a self-gravitating disc to disturbances
excited by an external potential. This is possible in a
self-gravitating disc because the disturbance associated with edges
can be communicated gravitationally to other parts of the disc, much
like an external potential (e.g. a planet) excites density waves in a
disc. We shall consider an interior edge located at $r=r_e$ and its
effect on the disc at the outer Lindblad resonance
($r=r_\mathrm{OLR}>r_e$) or inner Lindblad resonance
($r=r_\mathrm{ILR}<r_e$). Let us begin with new notation. Define $F$
such that 
\begin{align}
  \frac{dS}{dr} + \frac{2m\Omega\sbar S}{r\kappa^2} = DF.
\end{align}
Our governing equation is then 
\begin{align}\label{goveq_with_F}
 \dd\Sigma = \frac{1}{r}\frac{d}{dr}\left(r\Sigma F\right) - \frac{2m\Omega\sbar
   \Sigma}{r\kappa^2}F +
 \frac{mS}{r\sbar}\left(\frac{1}{\eta}\right)^\prime -
 \frac{4m^2\Omega^2\Sigma S}{r^2\kappa^4}. 
\end{align}
We split the perturbed potential $\dd\Phi$ into an interior and edge
part, so that $\dd\Phi = \dd \Phi_\mathrm{in} + \dd\Phi_0$. Then the
perturbation variable $S$ is written
\begin{align}
  S = S_\mathrm{in} + \dd\Phi_0,
\end{align}
where $S_\mathrm{in} = c_s^2\dd\Sigma/\Sigma +
\dd\Phi_\mathrm{in}$. The defining equation of $F$ becomes
\begin{align}\label{define_f}
  \frac{dS_\mathrm{in}}{dr} + \frac{2m\Omega\sbar
    S_\mathrm{in}}{r\kappa^2} +\frac{d\dd\Phi_0}{dr} + \frac{2m\Omega\sbar
    \dd\Phi_0}{r\kappa^2}  = DF. 
\end{align}

\subsubsection{Local equations}
We consider the solution near Lindblad resonances. Denote 
\begin{align}
r - r_\mathrm{LR} = x,
\end{align}
where $r_\mathrm{LR}$ are radii of Lindblad resonances, the
coefficient $D$ can be written to first order in its Taylor expansion
\begin{align}
 & D \equiv \kappa^2 - \sbar^2 \simeq \beta x \\\notag
 & \beta = 2\kappa(\kappa^\prime \pm m\Omega^\prime)x, 
\end{align}
where the upper sign is for OLR and lower sign for ILR. Near Lindblad
resonances, the defining equation for $F$ is approximated as
\begin{align}
  &\frac{dS_\mathrm{in}}{dx} +
  S_\mathrm{in}\left(\frac{2m\Omega\sbar}{r\kappa^2}\right)_\mathrm{LR}  
  + R = \beta x F, \\\notag
& R = \left(\frac{d\dd\Phi_0}{dr} + \frac{2m\Omega\sbar 
    \dd\Phi_0}{r\kappa^2}\right)_\mathrm{LR}.
\end{align}
In local theory, the background is considered as constant so we have
ignored variations in the coefficient of $S_\mathrm{in}$. We have also evaluated
the edge terms at LR, assuming that this potential from the edge is
slowly varying in the region of interest. This is the key assumption
in our analogy.   

We also need the local approximation of the governing equation:
\begin{align}
  \dd\Sigma = \Sigma \frac{dF}{dx} - \frac{2m\Omega\sbar
   \Sigma}{r\kappa^2}F.
\end{align}
Coefficients of $F$ and $dF/dx$ are now  evaluated at LR. In going
from the full governing equation to the local
version above, we have retained only $dF/dr$ from the first term on
RHS of Eq. \ref{goveq_with_F} and neglected the last two terms in that
equation. {\bf ASK ASK ASK ASK ASK ASK ASK ASK}. The vortensity term
is small because we are away from the edge (where vortensity gradients
are largest). When solving the problem in local theory we will set
$d/dx = d/dr = ik$ where $k$ is a large wavenumber. This means that
terms that do not involve spatial derivatives of the perturbed
variables are small compared to those with $d/dx$. This justifies
neglecting the last two terms in Eq. \ref{goveq_with_F}. 


Finally, the local approximation to the Poisson equation is simply
\begin{align}
  \nabla^2 \dd\Phi_\mathrm{in} = 4\pi G \dd\Sigma\dd(z),
\end{align}
which just means we have again neglected variations of the edge
potential in the region of interest. 

\subsubsection{Local solutions}
We solve the local equations using Fourier transforms. Perturbed
variables are written as 
\begin{align}
  F(x) = \int_{-\infty}^{\infty}F_k \exp{ikx}dk,
\end{align}
and similarity for other variables, where $k$ is real and it is
assumed that most of the contribution comes from large $k$. In Fouier
space, our local equations become
\begin{align}
&  i\beta\frac{dF_k}{dk} = ikS_{in,k} +
  \left(\frac{2m\Omega\sbar}{r\kappa^2}\right)S_{in,k} + R_k \\ 
& \dd\Sigma_k = ik\Sigma F_k - \left(\frac{2m\Omega\sbar
    \Sigma}{r\kappa^2}\right)F_k. \\
& R_k = \left(\frac{d\dd\Phi_0}{dr} + \frac{2m\Omega\sbar 
    \dd\Phi_0}{r\kappa^2}\right)\dd(k) \equiv A\dd(k).
\end{align}
The last equation comes from the treatment of the edge potential as a
constant. The local solution to our Poisson in the region of interest is
\begin{align}
\dd\Phi_{in} = -\frac{2\pi G \dd\Sigma_k}{|k|}.
\end{align}
Finally, in Fourier space the definition of  $S_{in}$ is
\begin{align}
  S_{in,k} = c_s^2\frac{\dd\Sigma_k}{\Sigma} + \dd\Phi_{in}.
\end{align}
Equations above can be combined to give
\begin{align}
i\beta \frac{dF_k}{dk} &= \left(-k^2 -
  \frac{4m^2\Omega^2\sbar^2}{r^2\kappa^4}\right)\left(c_s^2 - \frac{2\pi
  G \Sigma}{|k|}\right)F_k + A\dd(k)\\\notag  
&\simeq (-c_s^2 k^2 + 2\pi G \Sigma |k|)F_k + A\dd(k). 
\end{align}
The last approximation follows from large $k$. The solution for $F_k$
is 
\begin{align}
  F_k = \left\{ \begin{array}{ll}
      \frac{A}{i\beta}\exp{\frac{i}{\beta}(c_s^2k^3/3 - \pi G \Sigma
        k^2)} & \quad k > 0\\
        0 & \quad k <0.\\\end{array}\right.
\end{align}
 We also have, for $k>0$
\begin{align}
S_{in,k} &= \left(c_s^2 - \frac{2\pi G \Sigma}{|k|}\right)\left(ik -
  \frac{2m\Omega\sbar}{r\kappa^2}\right)F_k \\\notag
&\simeq ik\left(c_s^2 - \frac{2\pi G \Sigma}{|k|}\right)F_k\\\notag
&= \frac{A}{\beta}\left(c_s^2k - 2\pi G \Sigma\right)\exp{\frac{i}{\beta}(c_s^2k^3/3 - \pi G \Sigma
        k^2)}. 
\end{align}
We have real-space solutions
\begin{align}
  & F(x) = \frac{A}{i\beta}\int_0^\infty \exp{if(k)} dk\\
  & S_{in,k} = \frac{A}{\beta}\int_0^\infty (c_s^2k - 2\pi G
  \Sigma )\exp{if(k)} dk\\\notag
& f(k)\equiv \frac{1}{\beta}(c_s^2k^3/3 - \pi G \Sigma k^2 + k\beta x). 
\end{align}
We now evaluate these integrals explicitly using the method of
stationary phase. In this approximation, integrals of the form
\begin{align}
  I = \int_0^\infty g(k)\exp{if(k)} dk,
\end{align}
where $f(k)$ is a real function, is approximated as
\begin{align}
  I \simeq g(k_0)\exp{if(k_0)}\int_0^\infty\exp{i
    \left[f^{\prime\prime}(k_0)(k-k_0)^2/2\right]} dk,
\end{align}
where $k_0$ is such that $f^\prime{k_0} = 0$.
The integral term is approximately
\begin{align}
  \sqrt{\frac{2}{f^{\prime\prime}(k_0)}}\int_{-\infty}^\infty \exp iz^2 dz.
\end{align}
We have assumed that $k_0$ is large so that the lower integral limit
in $z$ space is replaced by $-\infty$. Then, using results
for Fresnel integrals, we find
\begin{align}  
  I\simeq g(k_0) \exp{if(k_0)} \sqrt{\frac{2\pi i}{f^{\prime\prime}(k_0)}}.
\end{align}
We therefore have
\begin{align}
&F = \frac{A}{i\beta} \exp{if(k_0)} \sqrt{\frac{2\pi
    i}{f^{\prime\prime}(k_0)}} \\
&S_{in} = \frac{A}{\beta}(c_s^2 k_0 - 2\pi G\Sigma) \exp{if(k_0)} \sqrt{\frac{2\pi
    i}{f^{\prime\prime}(k_0)}}\\\notag
& f^{\prime\prime}(k_0) = \frac{1}{\beta}(2c_s^2 k_0 - 2\pi G\Sigma)
\end{align}
We can insert these solutions into the definition of the advective
angular momentum flux (in the limit $\sbar$ being real)
\begin{align}
  F_A &= \frac{m\Sigma}{2}\Im(F^* S_{in}). \\\notag
  & = \frac{\pi m \Sigma |A|^2}{2\beta} \frac{(c_s^2 k_0 - 2\pi G\Sigma
    )}{(c_s^2k_0 -
    \pi G \Sigma)}. 
\end{align}
Note that we are using $S_{in}$ instead of $S$ because we are
attempting to isolate the edge effect as an external source. 

We also need the gravity flux. This is obvious since  the edge needs
to gravitationally disturb the interior disc for us to interpret it as
an external source for the interior. In the local limit, the gravity flux
associated with $\dd\Phi_{in}$ is
\begin{align}
F_G & = -\frac{m}{2}\Im\int_{-\infty}^{\infty} 
\frac{\dd\Phi_{in}}{4\pi G}\frac{\p\dd\Phi_{in}^*}{\p r} dz \\\notag
&=\frac{m}{2}\frac{k}{4\pi G} \int_{-\infty}^{\infty} |\dd\Phi_{in}|^2 dz.
\end{align}
The solution for $\dd\Phi_{in}$ in real space is, with the appropriate $z$ dependence:
\begin{align}
\dd\Phi_{in} = -2\pi G \int_{-\infty}^{\infty}\frac{\exp{-|kz|}}{|k|}\dd\Sigma_k \exp{ikx} dk.
\end{align}
Now, using $\dd\Sigma_k\simeq ik \Sigma F_k$ as a first approximation from the local equations, we find
\begin{align}
\dd\Phi_{in} = -\frac{2\pi G \Sigma A}{\beta} \exp{-|k_0z|}\exp{if(k_0)}
\sqrt{\frac{2\pi i}{f^{\prime\prime}(k_0)}},
\end{align}
and
\begin{align}
F_G = \frac{\pi m\Sigma|A|^2}{2\beta}\frac{\pi G\Sigma}{c_s^2k_0 - \pi G\Sigma}.
\end{align}
The total flux is then
\begin{align}
F_T = \frac{\pi m\Sigma }{2\beta}\left|\frac{d\dd\Phi_0}{dr} + \frac{2m\Omega\sbar 
    \dd\Phi_0}{r\kappa^2}\right|^2.
\end{align}


{\bf ASK ABOUT SIGN OF FLUX (OPPOSITE SIGNS AT LR'S?). ASK ASK ASK ASK ASK ASK ASK. }

\subsection{Description of the edge disturbance}
We now focus on the self-gravitating disturbance associated with an
edge, which we interpret as driving activitin elsewhere in the
disc. We consider the region around the edge, defined by steep
vortensity gradient, and co-rotation lies within the region of
interest. 

From the governing equation, we assume the balance
\begin{align} 
  \dd\Sigma = \frac{mS}{r\sbar}\frac{d}{dr}\left(\frac{1}{\eta}\right),
\end{align}
motivated by the fact the in the region considered, the vortensity
gradient is large. We insert the approximation above into the
defintion of $S$ to obtain
\begin{align}
S =
\frac{mc_s^2S}{r\Sigma\sbar}\frac{d}{dr}\left(\frac{1}{\eta}\right) -
G\int_{r_1}^{r_2} \xi
K_m(r,\xi)\frac{mS(\xi)}{\sbar(\xi)\xi}\frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]
d\xi,  
\end{align}
or
\begin{align}
S\left[ 1-
  \frac{mc_s^2}{r\Sigma\sbar}\frac{d}{dr}\left(\frac{1}{\eta}\right)\right] = 
- G\int_{r_1}^{r_2}\xi
K_m(r,\xi)\frac{mS(\xi)}{\sbar(\xi)\xi}\frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]d\xi.      
\end{align}
The integration range $[r_1,r_2]$ corresond to the entire disc, but
contribution outside the vortensity edge is negligible where vortensity
gradient is assumed small. 
Introducing the function $\mathcal{H}$ such that
\begin{align}
  S =
  \left\{-\left[\frac{d}{dr}\left(\frac{1}{\eta}\right)\frac{m}{\sbar}\right]^{-1}\right\}^{1/2}
    \left[
      1-\frac{mc_s^2}{r\Sigma\sbar}\frac{d}{dr}\left(\frac{1}{\eta}\right)\right]^{-1/2} \mathcal{H},
\end{align}
the integral equation above can be simplified to 
\begin{align}
  &\left[-\frac{d}{dr}\left(\frac{1}{\eta}\right)\frac{m}{\sbar}\right]^{-1/2}\left[1 -\frac{mc_s^2}{r\Sigma\sbar}\frac{d}{dr}\left(\frac{1}{\eta}\right)\right]^{1/2}\mathcal{H}
  \\\notag =
  &G\int_{r_1}^{r_2}K_m(r,\xi)\left\{-\frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]\frac{m}{\sbar(\xi)}\right\}^{1/2}
  \left\{ 1
      -\frac{mc_s^2}{\xi\Sigma(\xi)\sbar(\xi)}\frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]\right\}^{-1/2} \mathcal{H}(\xi)d\xi.
\end{align}
Defining the new kernel $\mathcal{R}(r,\xi)$ as
\begin{align}
\mathcal{R}_m(r,\xi) \equiv  &  GK_m(r,\xi)\left\{\frac{m}{\sbar(r)}
    \frac{d}{dr}\left[\frac{1}{\eta(r)}\right]\frac{m}{\sbar(\xi)}
    \frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]\right\}^{1/2} \notag\\
&\left/ \left\{1 -
    \frac{mc_s^2}{r\sbar(r)\Sigma{r}}\frac{d}{dr}\left[\frac{1}{\eta(r)}\right]\right\}^{1/2}\notag
\left\{ 1 -
    \frac{mc_s^2}{\xi\sbar(\xi)\Sigma{\xi}}\frac{d}{d\xi}\left[\frac{1}{\eta(\xi)}\right]\right\}^{1/2}\right.,
\end{align}
we obtain
\begin{align}
  \mathcal{H} = \int_{r_1}^{r_2}\mathcal{R}_m(r,\xi)\mathcal{H}(\xi)d\xi.
\end{align}
In other words, $\mathcal{H}$ is required to be
the solution to
\begin{align}\label{fredholm}
  \lambda \mathcal{H} = \int_{r_1}^{r_2}\mathcal{R}_m(r,\xi)\mathcal{H}(\xi)d\xi,
\end{align}
with $\lambda=1$. However, Eq. \ref{fredholm} is just the standard
homogenous Fredholm equation of the second type. Thus mode
existence ($\mathcal{H}\neq 0$) imply $\mathcal{H}$ is an
eigenfunction of the kernel $\mathcal{R}_m$ with unit eigenvalue.

For symmetric kernels, the Fredholm
equation above has the property that the maximum eigenvalue $\lambda$
is the maximum of the quantity $\Lambda$
\begin{align}
  \Lambda = \frac{\int_{r_1}^{r_2}\int_{r_1}^{r_2}\mathcal{R}_m(r,\xi)
    \mathcal{H}(\xi)\mathcal{H}^*(r)drd\xi}{\int_{r_1}^{r_2}|\mathcal{H}(r)|^2 dr}
\end{align}
among all $\mathcal{H}$. Thus, if $\mathrm{max}(\Lambda) < 1$ then it
is not possible to have a non-trivial mode. Upon application of the
Cauchy-Schwarz inequality (twice), one can deduce
\begin{align}
  \Lambda^2 \leq
  \int_{r_1}^{r_2}\int_{r_1}^{r_2}[\mathcal{R}(r,\xi)]^2drd\xi\equiv\Lambda_\mathrm{max}. 
\end{align}
Thus mode existence is not possible if the RHS is less than unity. 

To relate the neccessary condition for mode existence to physical
quantities, we can estimate $\Lambda_\mathrm{max}$.
The Poisson kernel $K_m(r,\xi)$ is largest at $r = \xi$. Other factors in
the numerator of  $\mathcal{R}_m$ involves the factor $1/\sbar$. We assume
these factors have largest contribution from co-rotation where
$\sbar(r_c) = 0$, but we also need $(1/\eta)^{\prime\prime} = 0$ at
co-rotation to remain regular. Hence, roughly speaking, $
\Lambda_\mathrm{max}^2 \sim
\int_{r_1}^{r_2}\int_{r_1}^{r_2}[\mathcal{R}(r_c,r_c)]^2drd\xi
$. Assuming the edge region has width of order the local scale-height,
we estimate
\begin{align}  
\Lambda_\mathrm{max} \sim &\mathcal{R}(r_c, r_c) H(r_c)\notag\\
& =
GK_m(r_c,r_c)\left|\frac{1}{\Omega^\prime}\left(\frac{1}{\eta}\right)^{\prime\prime}\right|
\left/ \left| 1 - \frac{c_s^2}{r_c \Sigma
      \Omega^\prime}\left(\frac{1}{\eta}\right)^{\prime\prime}\right|\right..  
\end{align}
All quantities are evaluated at co-rotation. Because the edge is thin
by assumption, we can further approximate the Poisson kernel by
\begin{align}
K_m(r,\xi) \sim \frac{2}{\bar{r}}K_{B0}\left(\frac{m}{\bar{r}}\sqrt{|r
    - \xi|^2 + \epsilon_g^2} \right),
\end{align}
where $K_{B0}$ is the zeroth modified Bessel function of the second
kind, $\bar{r}$ is the average radius of the region and recall that
$\epsilon_g$ is the softening length. If we further assume negligible
pressure effects ($c_s^2$ being small), we obtain
\begin{align}
  \Lambda_\mathrm{max} \sim
  \frac{2GK_{B0}(m\epsilon_g/\bar{r})}{\bar{r}}
  \left|\frac{1}{\Omega^\prime}\left(\frac{1}{\eta}\right)^{\prime\prime}\right|_{r_c}H(r_c).   
\end{align}
Since $\eta = \kappa^2/2\Omega\Sigma$, we expect such
modes can exist for sufficiently large surface density scales. This is
expected for a gravitationally-related disturbance. However, the
fundamental quantity is the vortensity extremum, if it is not
sufficiently large then there can be no mode. 
Similarly, mode existence becomes difficult for increasing
softening and/or increasing $m$. We expect self-gravitating modes where
density perturbation at the edge can balanced by the vortensity term
is only possible for low $m$. 


==> Chapter3/hydro1.tex <==
\section{Existence of edge modes in massive discs}\label{hydro1}
{\bf Show that edge modes develop in simulations, as motivation for
  remaining work.}
%To remove
%complications from vortex-forming edge  instabilities, we the
%standard viscosity $\nu=10^{-5}$ in code 
%units is adopted for most simulations. However, for the $Q\leq 2$
%cases considered here, we note from the previous Chapter that such
%modes are in fact surppressed by self-gravity. 

We first demonstrate the existence of global instabilities associated
with a gap self-consistently opened by a giant planet. 
Numerical details are deferred to \S\ref{hydro2} where hydrodynamic
simulations are investigated more fully. Here, we describe results for
a gap opened by a Saturn-mass planet $M_p=3\times10^{-4}M_*$. The
planet is introduced at radius $r_p=5$ at $t=25P(r_p)\equiv25
P_0$ and is held on fixed cicular orbit. Its potential is switched on
over $10P_0$.  We compare a disc with $Q_m=1.5$ ($M_d = 0.063M_*$) to 
that with $Q_m=4.0$ ($M_d = 0.024$). It is already known that 
non-self-gravitating or weakly self-gravitating discs support local
instabilities that lead to vortex formation \citep{li09,
lin10}. However, this instability require low viscosity. For
comparison purposes we use a kinematic viscosity of $\nu = 10^{-6}$
(code units) in this section. This value of viscosity is an order of
magnitude smaller than what is typically adopted for protoplanetary
disc models.    

The gap profile for $Q_m=1.5$ is shown in
Fig. \ref{basic} in terms of azimuthally averaged surface
density and Toomre $Q$. The profile for $Q_m=4$ is essentially the 
same apart from a scale factor. The Toomre parameter is calculated
properly from one-dimensional profiles of epicycle frequency. This is
important because the Toomre parameter is related to the vortensity
$\eta \equiv  \kappa^2/2\Omega\Sigma$ through the epicycle frequency,
and it is the extremum in vortensity that is associated with
instability. For typical gap profiles that result from disc-planet
interactions, such as Fig. \ref{basic}, extrema in $Q$ and
$\eta$ coincide, so vortensity and Toomre $Q$ extrema may be used
interchangeably.  

At the outer gap edge, maximum $Q$ 
occurs at $r=5.5$ ($Q=4.2$) and minimum at $r=5.7$(
$Q=1.45$); at the inner gap edge $Q$ maximises at $r=4.55$ ($Q=5.5$)
and minimum at $r=4.3$ ($Q=2.35$). The extrema are seperated by
$\simeq 1.1H,\,0.7H$ for the inner and outer gap edges respectively,
so the characterstic width of the gap edge is the local scale-height.   

In the $Q_m=1.5$ disc, $Q(r>6)$ is approximately
1.8. Since $Q>1$ everywhere, the disc is stable against axisymmetric
perturbations. Based on $Q$ values alone, we may naively expect the
outer $Q$ minimum to be most susceptible to gravitational
instability. We do not expect gravitational-driven instabilities to
operate in the $Q_m=4$ disc because it is $2.7$ times less massive
than $Q_m=1.5$. 

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/v3_basic_Q_nu6.ps}
\caption{Gap profile opened by a Saturn-mass planet in a disc with
  $Q_m=1.5$, in terms of the Toomre $Q$ parameter (solid) and surface
  density (dotted). The planet is located at $r=5$. 
\label{basic}}
\end{figure}

Fig. \ref{vortex_edge} show two types of instabilities depending on
disc mass. In the $Q_m=4$ disc, 6 vortices develop at the
outer gap edge. They are localised and aligned with the edge. Vortex
formation at gap edges is a standard result for giant planets in low
viscosity non-self-gravitating discs \citep{valborro07,lin10}. The
more massive $Q_m=1.5$ disc develop a different instability: global
$m=3$ spiral arms. It is associated with the outer gap edge but not 
localised. Consider a spiral arm extending 
inwards from the outer disc ($r>r_p$): it protrudes the original gap 
edge where its surface density perturbation is largest (the `tip').
The edge modes make the gap less identifyable than vortex modes.

% actually the first edge mode to emergy is m=2
%
%

In Fig. \ref{vortex_edge}, the $Q_m=1.5$ disc show spiral disturbances 
on both sides of the gap, unlike $Q_m=4$ where the inner edge remain stable.
The edge mode spirals do not extend continously across the gap because the 
planet potential favour gap opening. Nevertheless, surface density
perturbations on either side of the gap can communicate via
self-gravity, and the plot shows clear correlation between
disturbances on either side of the gap. However, the outer spiral 
is more prominent. This may because the outer disc has low 
Toomre $Q$. 

The amplitudes in Fig. \ref{vortex_edge} means the modes are already 
in their non-linear evolution. While the edge mode only takes a few 
$P_0$ to become non-linear, the vortex mode takes a longer time. 
(the figure is for $Q_m=4$ is $30P_0$ after gap formation). The spiral
shocks of the edge modes have comparable amplitudes to the planetary
wakes. 

The edge modes seen above has been suggested to occur in 
self-gravitating discs with a surface density depression 
\citep[][, where it is called `groove modes']{meschiari08}. 
\citeauthor{meschiari08} used analytic surface density
profiles to mimic a deep gap opened by a Jovian-mass planet
($90\%$ surface densit deficit relative to the smooth background). 
%They considered disc masses of at least $M_d/M_*=0.08$ and more 
%typically $M_d/M_* > 0.1$. 

Simulations here confirm the existence of spiral instabilities associated 
with a  partial gap self-consistently opened by a Saturn-mass planet. The 
disc masses we consider are $M_d < 0.1 M_*$ whereas those considered by 
\cite{meschiari08} were typically $M_d > 0.1M_*$. For a disc mass of 
$M_d \simeq 0.06M_*$ (our $Q_m=1.5$ case), \citeauthor{meschiari08}'s 
profile do not show the spiral instability. We also found that the 
co-rotation radii for the $m=3$ edge mode in $Q_m=1.5$ to be $r_c \simeq 5.5$ 
(Fig. \ref{v0_pattern}) This coincides with local maxima in Toomre $Q$ / vortensity 
at the outer gap edge. However, co-rotation in \citeauthor{meschiari08} where located
at the gap centre. 

\begin{figure}
  \centering
  \subfigure[$Q_m=1.5$]{\includegraphics[width=0.33\textwidth]{figures/v0_polar_dens023_nu6.ps}} 
  \subfigure[$Q_m=4.0$]{\includegraphics[width=0.33\textwidth]{figures/v2_polar_dens070_nu6.ps}} 
  \caption{Relative surface density perturbation for the $Q_m=1.5$
    disc (a) and the $Q_m=4.0$ disc. These plots show that the gap
    opened by a Saturn-mass planet support vortex instabilities in low
    mass discs and spiral instabilities with sufficient disc mass. 
    \label{vortex_edge}}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.33\textwidth]{figures/v0_pattern_nu6}
  \caption{Local pattern speed for the $m=3$ edge mode in the $Q_m=1.5$ disc (solid). 
	Intersection between dashed lines and the solid line denote inner Lindblad resonance
	($\Omega - \kappa/3$), co-rotation resonance ($\Omega$, the co-rotation point) and outer
        Lindblad resonance ($\Omega + \kappa/3$). 
    \label{v0_pattern}}
\end{figure}










% Direct simulation show that both gap edges become unstable. The
% relative surface density perturbation is shown in
% Fig. \ref{Qm1.5_t50} at $t=50P_0$. We identify a
% $m=3$ mode with $\Delta\Sigma/\Sigma\simeq 0.4$ associated with the
% inner edge $r=4$; and a $m=2$ mode with $\Delta\Sigma/\Sigma\simeq
% 0.9$ with the outer edge.   

% These amplitudes means the system is already
% non-linear, with the development of shocks by the outer spiral
% mode. The instability becomes non-linear within $<10P_0$, i.e. it
% grows on dynamical time-scales. In contrast to vortex-forming
% instabilities, these are global spiral modes, but neither spiral
% pattern extend across the gap. This is probably because the planet is
% trying to open a gap and the self-gravity is not strong enough to
% connect the two spiral modes on either side of $r_p$.  


% We focus on the outer gap edge because  the $m=2$ spiral mode has more
% than twice the amplitude than the inner spiral
% mode. Fig. \ref{Qm1.5_t50} shows the pattern speed 
% $\Omega_\mathrm{pat}$ of the $m=2$ Fourier component of the surface
% density. % including features due to planetary wakes and
% inner disc spiral modes. 
% There is a co-rotation point at $r=5.5$ where
% $\Omega=\Omega_\mathrm{pat}\sim 0.078 $, i.e. the local vortensity
% (surface density) maximum (minimum) of the basic state, which is just
% inside the gap (see Figure \ref{Qm1.5_basic}.   It is
% also consistent with pattern speeds from linear calculations presented
% later. 

% The figure suggests a another co-rotation point at $r\simeq 4.7$ but
% this is due to calculation of the pattern speed, which includes
% features from the planetary wakes. Typically $\Omega_\mathrm{pat}\sim
% 0.08$ across the disc. We have explicitly checked
% that this is the pattern speed by measuring the angle through which
% the spiral pattern rotates through in a given time interval.

% The unstable mode here differs to the vortex-forming modes found
% in weakly self-gravitating or non-self-gravitating discs, which have
% co-rotation radius at vortensity minimum ($r=5.7$). The
% vortex modes are localised with high $m$ being dominant ($m>5$),
% whereas spiral modes found here are global with low $m$. 


% The spiral pattern speed is that
% of local vortensity maximum just inside the gap edge.
% This is different to `groove modes' studied by
% \cite{meschiari08,sellwood91} which have co-rotation near the centre
% of the density depression, which corresponds to the planetary gap in
% our context. If co-rotation lies at the gap centre, the spiral pattern
% co-rotates with the planet, then there would be no change in the
% orientation of the spirals relative to the planet.

%The two spirals have angular separation of nearly $\pi$, but perfect
%symmetry is not expected because of the planet. 


















































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%BELOW: ORIGINAL DISCUSSION WITH VISCOSITY = 1D-5, Q_M=1.5 CASE TO            %
%DEMONSTRATE EXISTENCE OF EDGE MODE. NOW REPLACED WITH ABOVE, BY              %
%COMAPING EDGE MODE AND VORTEX MODE, BUT NEEDED TO DO VISCOSITY = 1D-6        %
%TO GET THE VORTEX MODE, SO HAD TO REPLACE EDGE MODE EXAMPLE WITH             %
%SIM. WITH NU=1D-6                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We first demonstrate the existence of global instabilities associated
% with a gap self-consistently opened by a giant planet. We
% defer numerical details to \S\ref{hydro2} where hydrodynamic
% simulations are investigated more fully. Here, we describe results for
% a disc with $Q_m=1.5,\, M_d/M_* = 0.063$ 
% and a Saturn-mass planet
% $M_p=3\times10^{-4}M_*$. 
% The planet is introduced
% at radius $r_p=5$ at $t=25P(r_p)\equiv25 P_0$. Its
% potential is switched on over $10P_0$.  It is held on fixed cicular
% orbit. 
% The gap profile opened by the planet is shown in
% Fig. \ref{Qm1.5_basic} in terms of azimuthally averaged surface
% density and Toomre $Q$. The Toomre parameter is calculated properly
% from one-dimensional profiles of epicycle frequency. This is important
% because the Toomre parameter is related to the vortensity $\eta \equiv 
% \kappa^2/2\Omega\Sigma$ through the epicycle frequency, and it is the
% extremum in vortensity that is associated with instability. For
% typical gap profiles that result from disc-planet interactions, such
% as Fig. \ref{Qm1.5_basic}, extrema in $Q$ and $\eta$ coincide, so
% vortensity and Toomre $Q$ extrema may be used interchangeably. 

% %The main feature that gives rise to instability are vortensity
% %extrema. As argued in
% %the previous Chapter, self-gravity can destabilise neutral modes
% %associated with vortensity maxima. Thus, in the present regime of
% %strong self-gravity we can expect modes with co-rotation radius at
% %$\mathrm{max}(\eta)$. 

% At the outer gap edge, $Q$ maximum
% occurs at $r=5.5$ ($Q=4.2$) and minimum at $r=5.7$---5.8 (
% $Q=1.75$); at the inner gap edge $Q$ maximises at $r=4.55$ ($Q=4.75$)
% and minimum at $r=4.3$ ($Q=2.55$). For $r>6$, $Q$ is approximately
% two. Since $Q>1$ everywhere, the disc is stable against axisymmetric
% perturbations. Based on $Q$ values alone, we may naively expect the
% outer $Q$ minimum to be most susceptible to gravitational
% instability. The extrema are seperated by $\simeq 1.1H,\,0.89H$ for
% the inner and outer gap edges respectively, so the characterstic width
% of the gap edge is the local scale-height.  

% %Vortensity maximum coincides with local surface
% %density minimum just inside the gap, whereas vortensity minimum
% %approximately coincides with local surface density maximum just
% %outside the gap edge. 
    
% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/v3NRBCnu5_basic_Q.ps}
% \caption{Gap profile opened by a Saturn-mass planet in a disc with
%   $Q_m=1.5$, in terms of the Toomre $Q$ parameter (solid) and surface
%   density (dotted). The planet is located at $r=5$. 
% \label{Qm1.5_basic}}
% \end{figure}

% Direct simulation show that both gap edges become unstable. The
% relative surface density perturbation is shown in
% Fig. \ref{Qm1.5_t50} at $t=50P_0$. We identify a
% $m=3$ mode with $\Delta\Sigma/\Sigma\simeq 0.4$ associated with the
% inner edge $r=4$; and a $m=2$ mode with $\Delta\Sigma/\Sigma\simeq
% 0.9$ with the outer edge.   

% These amplitudes means the system is already
% non-linear, with the development of shocks by the outer spiral
% mode. The instability becomes non-linear within $<10P_0$, i.e. it
% grows on dynamical time-scales. In contrast to vortex-forming
% instabilities, these are global spiral modes, but neither spiral
% pattern extend across the gap. This is probably because the planet is
% trying to open a gap and the self-gravity is not strong enough to
% connect the two spiral modes on either side of $r_p$.  


% We focus on the outer gap edge because  the $m=2$ spiral mode has more
% than twice the amplitude than the inner spiral
% mode. Fig. \ref{Qm1.5_t50} shows the pattern speed 
% $\Omega_\mathrm{pat}$ of the $m=2$ Fourier component of the surface
% density. % including features due to planetary wakes and
% inner disc spiral modes. 
% There is a co-rotation point at $r=5.5$ where
% $\Omega=\Omega_\mathrm{pat}\sim 0.078 $, i.e. the local vortensity
% (surface density) maximum (minimum) of the basic state, which is just
% inside the gap (see Figure \ref{Qm1.5_basic}.   It is
% also consistent with pattern speeds from linear calculations presented
% later. 

% The figure suggests a another co-rotation point at $r\simeq 4.7$ but
% this is due to calculation of the pattern speed, which includes
% features from the planetary wakes. Typically $\Omega_\mathrm{pat}\sim
% 0.08$ across the disc. We have explicitly checked
% that this is the pattern speed by measuring the angle through which
% the spiral pattern rotates through in a given time interval.

% The unstable mode here differs to the vortex-forming modes found
% in weakly self-gravitating or non-self-gravitating discs, which have
% co-rotation radius at vortensity minimum ($r=5.7$). The
% vortex modes are localised with high $m$ being dominant ($m>5$),
% whereas spiral modes found here are global with low $m$. 


% The spiral pattern speed is that
% of local vortensity maximum just inside the gap edge.
% This is different to `groove modes' studied by
% \cite{meschiari08,sellwood91} which have co-rotation near the centre
% of the density depression, which corresponds to the planetary gap in
% our context. If co-rotation lies at the gap centre, the spiral pattern
% co-rotates with the planet, then there would be no change in the
% orientation of the spirals relative to the planet.

% %The two spirals have angular separation of nearly $\pi$, but perfect
% %symmetry is not expected because of the planet. 


% %{\bf TO ADD:
% %\begin{itemize}
% %  \item CALCULATION OF MODE AMPLITUDES.
% %  \item CALCULATION OF PATTERN SPEED, WHICH REQUIRE TIME DERIVATIVES
% %    OF SURFACE DENSITY FIELD FROM DATA. CONVERT TIME DERIVATIVE TO
% %    SPATIAL DERIVATIVE VIA CONTINUITY EQUATION.
% %  \end{itemize}
% %}

% \begin{figure}[!h]
% \centering
% \subfigure[Surface density
% perturbation]{\includegraphics[width=0.33\textwidth]{figures/v3NRBCnu5_polar_dens025.ps}} 
% \subfigure[Pattern
% speed]{\includegraphics[width=0.45\textwidth]{figures/v3NRBCnu5_pattern_m2.ps}} 
% \caption{Surface density distribution for $Q_m=1.5$ at $t=50P_0$
%   (left) and the corresponding pattern speed for the $m=2$ mode
%   (right, solid). $\Omega$ and $\Omega\pm\kappa/2$ are also shown
%   (right, dashed).
% \label{Qm1.5_t50}}
% \end{figure}


==> Chapter3/hydro1NEW.tex <==
\section{Existence of edge modes in massive discs}\label{hydro1}
{\bf Show that edge modes develop in simulations, as motivation for
  remaining work.}
%To remove
%complications from vortex-forming edge  instabilities, we the
%standard viscosity $\nu=10^{-5}$ in code 
%units is adopted for most simulations. However, for the $Q\leq 2$
%cases considered here, we note from the previous Chapter that such
%modes are in fact surppressed by self-gravity. 

We first demonstrate the existence of global instabilities associated
with a gap self-consistently opened by a giant planet. 
Numerical details are deferred to \S\ref{hydro2} where hydrodynamic
simulations are investigated more fully. Here, we describe results for
a gap opened by a Saturn-mass planet $M_p=3\times10^{-4}M_*$. The
planet is introduced at radius $r_p=5$ at $t=25P(r_p)\equiv25
P_0$ and is held on fixed cicular orbit. Its potential is switched on
over $10P_0$.  We compare a disc with $Q_m=1.5$ ($M_d = 0.063M_*$) to 
that with $Q_m=4.0$ ($M_d = 0.024$). It is already known that 
non-self-gravitating or weakly self-gravitating discs support local
instabilities that lead to vortex formation \citep{li09,
lin10}. However, this instability require low viscosity. For
comparison purposes we use a kinematic viscosity of $\nu = 10^{-6}$
(code units) in this section. This value of viscosity is an order of
magnitude smaller than what is typically adopted for protoplanetary
disc models.    

The gap profile for $Q_m=1.5$ is shown in
Fig. \ref{basic} in terms of azimuthally averaged surface
density and Toomre $Q$. The profile for $Q_m=4$ is essentially the 
same apart from a scale factor. The Toomre parameter is calculated
properly from one-dimensional profiles of epicycle frequency. This is
important because the Toomre parameter is related to the vortensity
$\eta \equiv  \kappa^2/2\Omega\Sigma$ through the epicycle frequency,
and it is the extremum in vortensity that is associated with
instability. For typical gap profiles that result from disc-planet
interactions, such as Fig. \ref{basic}, extrema in $Q$ and
$\eta$ coincide, so vortensity and Toomre $Q$ extrema may be used
interchangeably.  

At the outer gap edge, maximum $Q$ 
occurs at $r=5.5$ ($Q=4.2$) and minimum at $r=5.7$(
$Q=1.45$); at the inner gap edge $Q$ maximises at $r=4.55$ ($Q=5.5$)
and minimum at $r=4.3$ ($Q=2.35$). The extrema are seperated by
$\simeq 1.1H,\,0.7H$ for the inner and outer gap edges respectively,
so the characterstic width of the gap edge is the local scale-height.   

In the $Q_m=1.5$ disc, $Q(r>6)$ is approximately
1.8. Since $Q>1$ everywhere, the disc is stable against axisymmetric
perturbations. Based on $Q$ values alone, we may naively expect the
outer $Q$ minimum to be most susceptible to gravitational
instability. We do not expect gravitational-driven instabilities to
operate in the $Q_m=4$ disc because it is $2.7$ times less massive
than $Q_m=1.5$. 

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/v3_basic_Q_nu6.ps}
\caption{Gap profile opened by a Saturn-mass planet in a disc with
  $Q_m=1.5$, in terms of the Toomre $Q$ parameter (solid) and surface
  density (dotted). The planet is located at $r=5$. 
\label{basic}}
\end{figure}

Fig. \ref{vortex_edge} show two types of instabilities depending on
disc mass. In the $Q_m=4$ disc, 6 vortices develop at the
outer gap edge. They are localised and aligned with the edge. Vortex
formation at gap edges is a standard result for giant planets in low
viscosity non-self-gravitating discs \citep{valborro07,lin10}. The
more massive $Q_m=1.5$ disc develop a different instability: global
$m=3$ spiral arms. It is associated with the outer gap edge but not 
localised. Consider a spiral arm extending 
inwards from the outer disc ($r>r_p$): it protrudes the original gap 
edge where its surface density perturbation is largest (the `tip').
The edge modes make the gap less identifyable than vortex modes.

% actually the first edge mode to emergy is m=2
%
%

In Fig. \ref{vortex_edge}, the $Q_m=1.5$ disc show spiral disturbances 
on both sides of the gap, unlike $Q_m=4$ where the inner edge remain stable.
The edge mode spirals do not extend continously across the gap because the 
planet potential favour gap opening. Nevertheless, surface density
perturbations on either side of the gap can communicate via
self-gravity, and the plot shows clear correlation between
disturbances on either side of the gap. However, the outer spiral 
is more prominent. This may because the outer disc has low 
Toomre $Q$. 

The amplitudes in Fig. \ref{vortex_edge} means the modes are already 
in their non-linear evolution. While the edge mode only takes a few 
$P_0$ to become non-linear, the vortex mode takes a longer time. 
(the figure is for $Q_m=4$ is $30P_0$ after gap formation). The spiral
shocks of the edge modes have comparable amplitudes to the planetary
wakes. 

The edge modes seen above has been suggested to occur in 
self-gravitating discs with a surface density depression 
\citep[][, where it is called `groove modes']{meschiari08}. 
\citeauthor{meschiari08} used analytic surface density
profiles to mimic a deep gap opened by a Jovian-mass planet
($90\%$ surface densit deficit relative to the smooth background). 
%They considered disc masses of at least $M_d/M_*=0.08$ and more 
%typically $M_d/M_* > 0.1$. 

Simulations here confirm the existence of spiral instabilities associated 
with a  partial gap self-consistently opened by a Saturn-mass planet. The 
disc masses we consider are $M_d < 0.1 M_*$ whereas those considered by 
\cite{meschiari08} were typically $M_d > 0.1M_*$. For a disc mass of 
$M_d \simeq 0.06M_*$ (our $Q_m=1.5$ case), \citeauthor{meschiari08}'s 
profile do not show the spiral instability. We also found that the 
co-rotation radii for the $m=3$ edge mode in $Q_m=1.5$ to be $r_c \simeq 5.5$ 
(Fig. \ref{v0_pattern}) This coincides with local maxima in Toomre $Q$ / vortensity 
at the outer gap edge. However, co-rotation in \citeauthor{meschiari08} where located
at the gap centre. 

\begin{figure}
  \centering
  \subfigure[$Q_m=1.5$]{\includegraphics[width=0.33\textwidth]{figures/v0_polar_dens023_nu6.ps}} 
  \subfigure[$Q_m=4.0$]{\includegraphics[width=0.33\textwidth]{figures/v2_polar_dens070_nu6.ps}} 
  \caption{Relative surface density perturbation for the $Q_m=1.5$
    disc (a) and the $Q_m=4.0$ disc. These plots show that the gap
    opened by a Saturn-mass planet support vortex instabilities in low
    mass discs and spiral instabilities with sufficient disc mass. 
    \label{vortex_edge}}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.33\textwidth]{figures/v0_pattern_nu6}
  \caption{Local pattern speed for the $m=3$ edge mode in the $Q_m=1.5$ disc (solid). 
	Intersection between dashed lines and the solid line denote inner Lindblad resonance
	($\Omega - \kappa/3$), co-rotation resonance ($\Omega$, the co-rotation point) and outer
        Lindblad resonance ($\Omega + \kappa/3$). 
    \label{v0_pattern}}
\end{figure}










% Direct simulation show that both gap edges become unstable. The
% relative surface density perturbation is shown in
% Fig. \ref{Qm1.5_t50} at $t=50P_0$. We identify a
% $m=3$ mode with $\Delta\Sigma/\Sigma\simeq 0.4$ associated with the
% inner edge $r=4$; and a $m=2$ mode with $\Delta\Sigma/\Sigma\simeq
% 0.9$ with the outer edge.   

% These amplitudes means the system is already
% non-linear, with the development of shocks by the outer spiral
% mode. The instability becomes non-linear within $<10P_0$, i.e. it
% grows on dynamical time-scales. In contrast to vortex-forming
% instabilities, these are global spiral modes, but neither spiral
% pattern extend across the gap. This is probably because the planet is
% trying to open a gap and the self-gravity is not strong enough to
% connect the two spiral modes on either side of $r_p$.  


% We focus on the outer gap edge because  the $m=2$ spiral mode has more
% than twice the amplitude than the inner spiral
% mode. Fig. \ref{Qm1.5_t50} shows the pattern speed 
% $\Omega_\mathrm{pat}$ of the $m=2$ Fourier component of the surface
% density. % including features due to planetary wakes and
% inner disc spiral modes. 
% There is a co-rotation point at $r=5.5$ where
% $\Omega=\Omega_\mathrm{pat}\sim 0.078 $, i.e. the local vortensity
% (surface density) maximum (minimum) of the basic state, which is just
% inside the gap (see Figure \ref{Qm1.5_basic}.   It is
% also consistent with pattern speeds from linear calculations presented
% later. 

% The figure suggests a another co-rotation point at $r\simeq 4.7$ but
% this is due to calculation of the pattern speed, which includes
% features from the planetary wakes. Typically $\Omega_\mathrm{pat}\sim
% 0.08$ across the disc. We have explicitly checked
% that this is the pattern speed by measuring the angle through which
% the spiral pattern rotates through in a given time interval.

% The unstable mode here differs to the vortex-forming modes found
% in weakly self-gravitating or non-self-gravitating discs, which have
% co-rotation radius at vortensity minimum ($r=5.7$). The
% vortex modes are localised with high $m$ being dominant ($m>5$),
% whereas spiral modes found here are global with low $m$. 


% The spiral pattern speed is that
% of local vortensity maximum just inside the gap edge.
% This is different to `groove modes' studied by
% \cite{meschiari08,sellwood91} which have co-rotation near the centre
% of the density depression, which corresponds to the planetary gap in
% our context. If co-rotation lies at the gap centre, the spiral pattern
% co-rotates with the planet, then there would be no change in the
% orientation of the spirals relative to the planet.

%The two spirals have angular separation of nearly $\pi$, but perfect
%symmetry is not expected because of the planet. 


















































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%BELOW: ORIGINAL DISCUSSION WITH VISCOSITY = 1D-5, Q_M=1.5 CASE TO            %
%DEMONSTRATE EXISTENCE OF EDGE MODE. NOW REPLACED WITH ABOVE, BY              %
%COMAPING EDGE MODE AND VORTEX MODE, BUT NEEDED TO DO VISCOSITY = 1D-6        %
%TO GET THE VORTEX MODE, SO HAD TO REPLACE EDGE MODE EXAMPLE WITH             %
%SIM. WITH NU=1D-6                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We first demonstrate the existence of global instabilities associated
% with a gap self-consistently opened by a giant planet. We
% defer numerical details to \S\ref{hydro2} where hydrodynamic
% simulations are investigated more fully. Here, we describe results for
% a disc with $Q_m=1.5,\, M_d/M_* = 0.063$ 
% and a Saturn-mass planet
% $M_p=3\times10^{-4}M_*$. 
% The planet is introduced
% at radius $r_p=5$ at $t=25P(r_p)\equiv25 P_0$. Its
% potential is switched on over $10P_0$.  It is held on fixed cicular
% orbit. 
% The gap profile opened by the planet is shown in
% Fig. \ref{Qm1.5_basic} in terms of azimuthally averaged surface
% density and Toomre $Q$. The Toomre parameter is calculated properly
% from one-dimensional profiles of epicycle frequency. This is important
% because the Toomre parameter is related to the vortensity $\eta \equiv 
% \kappa^2/2\Omega\Sigma$ through the epicycle frequency, and it is the
% extremum in vortensity that is associated with instability. For
% typical gap profiles that result from disc-planet interactions, such
% as Fig. \ref{Qm1.5_basic}, extrema in $Q$ and $\eta$ coincide, so
% vortensity and Toomre $Q$ extrema may be used interchangeably. 

% %The main feature that gives rise to instability are vortensity
% %extrema. As argued in
% %the previous Chapter, self-gravity can destabilise neutral modes
% %associated with vortensity maxima. Thus, in the present regime of
% %strong self-gravity we can expect modes with co-rotation radius at
% %$\mathrm{max}(\eta)$. 

% At the outer gap edge, $Q$ maximum
% occurs at $r=5.5$ ($Q=4.2$) and minimum at $r=5.7$---5.8 (
% $Q=1.75$); at the inner gap edge $Q$ maximises at $r=4.55$ ($Q=4.75$)
% and minimum at $r=4.3$ ($Q=2.55$). For $r>6$, $Q$ is approximately
% two. Since $Q>1$ everywhere, the disc is stable against axisymmetric
% perturbations. Based on $Q$ values alone, we may naively expect the
% outer $Q$ minimum to be most susceptible to gravitational
% instability. The extrema are seperated by $\simeq 1.1H,\,0.89H$ for
% the inner and outer gap edges respectively, so the characterstic width
% of the gap edge is the local scale-height.  

% %Vortensity maximum coincides with local surface
% %density minimum just inside the gap, whereas vortensity minimum
% %approximately coincides with local surface density maximum just
% %outside the gap edge. 
    
% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/v3NRBCnu5_basic_Q.ps}
% \caption{Gap profile opened by a Saturn-mass planet in a disc with
%   $Q_m=1.5$, in terms of the Toomre $Q$ parameter (solid) and surface
%   density (dotted). The planet is located at $r=5$. 
% \label{Qm1.5_basic}}
% \end{figure}

% Direct simulation show that both gap edges become unstable. The
% relative surface density perturbation is shown in
% Fig. \ref{Qm1.5_t50} at $t=50P_0$. We identify a
% $m=3$ mode with $\Delta\Sigma/\Sigma\simeq 0.4$ associated with the
% inner edge $r=4$; and a $m=2$ mode with $\Delta\Sigma/\Sigma\simeq
% 0.9$ with the outer edge.   

% These amplitudes means the system is already
% non-linear, with the development of shocks by the outer spiral
% mode. The instability becomes non-linear within $<10P_0$, i.e. it
% grows on dynamical time-scales. In contrast to vortex-forming
% instabilities, these are global spiral modes, but neither spiral
% pattern extend across the gap. This is probably because the planet is
% trying to open a gap and the self-gravity is not strong enough to
% connect the two spiral modes on either side of $r_p$.  


% We focus on the outer gap edge because  the $m=2$ spiral mode has more
% than twice the amplitude than the inner spiral
% mode. Fig. \ref{Qm1.5_t50} shows the pattern speed 
% $\Omega_\mathrm{pat}$ of the $m=2$ Fourier component of the surface
% density. % including features due to planetary wakes and
% inner disc spiral modes. 
% There is a co-rotation point at $r=5.5$ where
% $\Omega=\Omega_\mathrm{pat}\sim 0.078 $, i.e. the local vortensity
% (surface density) maximum (minimum) of the basic state, which is just
% inside the gap (see Figure \ref{Qm1.5_basic}.   It is
% also consistent with pattern speeds from linear calculations presented
% later. 

% The figure suggests a another co-rotation point at $r\simeq 4.7$ but
% this is due to calculation of the pattern speed, which includes
% features from the planetary wakes. Typically $\Omega_\mathrm{pat}\sim
% 0.08$ across the disc. We have explicitly checked
% that this is the pattern speed by measuring the angle through which
% the spiral pattern rotates through in a given time interval.

% The unstable mode here differs to the vortex-forming modes found
% in weakly self-gravitating or non-self-gravitating discs, which have
% co-rotation radius at vortensity minimum ($r=5.7$). The
% vortex modes are localised with high $m$ being dominant ($m>5$),
% whereas spiral modes found here are global with low $m$. 


% The spiral pattern speed is that
% of local vortensity maximum just inside the gap edge.
% This is different to `groove modes' studied by
% \cite{meschiari08,sellwood91} which have co-rotation near the centre
% of the density depression, which corresponds to the planetary gap in
% our context. If co-rotation lies at the gap centre, the spiral pattern
% co-rotates with the planet, then there would be no change in the
% orientation of the spirals relative to the planet.

% %The two spirals have angular separation of nearly $\pi$, but perfect
% %symmetry is not expected because of the planet. 


% %{\bf TO ADD:
% %\begin{itemize}
% %  \item CALCULATION OF MODE AMPLITUDES.
% %  \item CALCULATION OF PATTERN SPEED, WHICH REQUIRE TIME DERIVATIVES
% %    OF SURFACE DENSITY FIELD FROM DATA. CONVERT TIME DERIVATIVE TO
% %    SPATIAL DERIVATIVE VIA CONTINUITY EQUATION.
% %  \end{itemize}
% %}

% \begin{figure}[!h]
% \centering
% \subfigure[Surface density
% perturbation]{\includegraphics[width=0.33\textwidth]{figures/v3NRBCnu5_polar_dens025.ps}} 
% \subfigure[Pattern
% speed]{\includegraphics[width=0.45\textwidth]{figures/v3NRBCnu5_pattern_m2.ps}} 
% \caption{Surface density distribution for $Q_m=1.5$ at $t=50P_0$
%   (left) and the corresponding pattern speed for the $m=2$ mode
%   (right, solid). $\Omega$ and $\Omega\pm\kappa/2$ are also shown
%   (right, dashed).
% \label{Qm1.5_t50}}
% \end{figure}


==> Chapter3/introduction.tex <==
\section{Introduction}
{\bf Introduce subject}





\section{Basic equations and model}\label{basic_equations}
{\bf Present full governing equations (including indirect potentials,
  viscosity). This is used for numerical simulations. Describe these
  here because simulations are used to prepare the gap profile to
  serve as basic state for analysis. Simpler
  equations used for analytical discussion and linear calculation, but
  mention these where appropriate.}

We describe here the full governing equations and models for the
disc-planet system as solved in hydrodynamic simulations. Simpler sets
of equations are used in analytical discussions and linear
calculations.   

The system is a gaseous disc of mass $M_d$ orbiting a central star 
of mass $M_*.$  We adopt a cylindrical, non-rotating, co-ordinate
system $(r,\phi,z)$ centred on the star where $z$ is the vertical
co-ordinate increasing in the direction normal to the disc plane. 
We integrate vertically to obtain a two-dimensional flat disc model,
for which the governing hydrodynamic equations are the continuity equation

\begin{align}\label{continuity}
\frac{\p\Sigma}{\p t}+\nabla\cdot(\mathbf{u}\Sigma)=0,
\end{align}
and the equation of motion
\begin{align}\label{momentum}
\frac{\p\bm{u}}{\p t}+\bm{u}\cdot\nabla\bm{u} =
-\frac{1}{\Sigma}\nabla P - \nabla\Phi + \frac{\bm{f}}{\Sigma}. 
\end{align}
Here $\Sigma$ is the surface density, $\bm{u}$ is the velocity field and
$P$ is the vertically  integrated pressure. We adopt a locally
isothermal equation of state, $P=c_s^2\Sigma$ where 
$c_s = H\Omega_k$ is the local sound speed, $\Omega_k=\sqrt{GM_*/r^3}$ 
being the Keplerian rotation speed and $H=hr$ is the disc
semi-thickness with $h=0.05$ being a constant aspect-ratio. 

In the momentum equation (Eq. \ref{momentum}), $\bm{f}$ is the viscous force characterised
by a uniform kinematic viscosity $\nu$ (details in \cite{masset02})
and the potential $\Phi$ is given by 
\begin{align}
\Phi = &-\frac{GM_*}{r} -
\frac{GM_p}{\sqrt{r^2+r_p^2-2rr_p\cos{(\phi-\phi_p)+\epsilon_p^2}}} + \Phi_d
  \\\notag 
&+\frac{GM_p}{r_p^2}r\cos{(\phi-\phi_p)} + r\int \frac{G\Sigma(r^\prime,\phi^\prime)}{r^{\prime2}}\cos{(\phi-\phi^\prime)}r^\prime dr^\prime d\phi^\prime\\
\Phi_d = &-\int
\frac{G\Sigma(r^\prime,\phi^\prime)}{\sqrt{r^2+r^{\prime 2} -
    2rr^\prime\cos{(\phi-\phi^\prime)}+ \epsilon_g^2}}r^\prime dr^\prime d\phi^\prime,
\end{align}
where the second term for $\Phi$ represents the planet potential 
centred at $(r_p,\phi_p,0)$ and softened by 
$\epsilon_p=\epsilon_{p0}H(r_p)$. $\Phi_d$ is the disc potential 
(the self-gravity), softened by
$\epsilon_g=\epsilon_{g0}H(r^\prime)$. Fiducial softening values are
$\epsilon_{p0} = 0.6$ and $\epsilon_{g0}=0.3$. The last two terms for 
$\Phi$ is the indirect potential which arises from the  non-inertial 
frame of reference.  

\subsection{Disc-planet model}
We adopt units such that $G=M_*=1$. The Keplerian orbital period at
$r=1$ is then $P(1)=2\pi$. The disc occupies $r=[r_0,r_m]=[1,10]$.  
A modified surface density profile of \cite{armitage99}   
is set initially:
\begin{align} 
 \Sigma(r) = \Sigma_0 r^{-3/2}\left(1-\sqrt{\frac{r_o}{r+H_0}}\right),
\end{align}
where $H_0=H(r_0)$ and is introduced here to prevent a singular
pressure gradient at the inner boundary. The constant surface density
scale $\Sigma_0$ is chosen via the parameter $Q_m\equiv Q(r_m)$ where  
\begin{align}\label{myQ} 
  Q(r) = \frac{hM_*}{\pi r^2\Sigma(r)}
\end{align}
is the Toomre $Q$ parameter for thin Keplerian discs. Note that we quote
$Q_m$ for ease of parametrisation. The actual Toomre $Q$ is
$c_s\kappa/\pi G\Sigma$ where $\kappa$ is the epicycle frequency. The
expression above assumes  $\kappa=\Omega_k$ which is 
only true in strict Keplerian orbit. Our discs, however, are
initialised with centrifugal balance between  
stellar gravity, self-gravity and pressure. 

The initial azimuthal velocity satisfies
 \begin{align}
 u_{\phi,i}^2 = \frac{r}{\Sigma}\frac{d P}{dr} + \frac{GM_*}{r} - rg_r,
 \end{align}
where $g_r=-\p\Phi_d/\p r$. For a local isothermal equation of state,
the contribution to $u^2_{\phi,i}$ due to the pressure 
gradient is given by 
\begin{align}
  \frac{r}{\Sigma}\frac{d P}{dr} = c_s^2 \left\{-\frac{5}{2} + \frac{r\sqrt{r_0}(r+H_0)^{-3/2}}{2\left[1-\sqrt{r_o/(r+H_0)}\right]}\right\}
\end{align}
At $r=r_0$ this is $\sim 20c_s^2$ with $h=0.05$, which is
approximately $5\%$ of the square of the local Keplerian speed. 
The initial radial velocity  
is set to $u_r = 3\nu/r$, which would correspond to  the radial
velocity  of a Keplerian accretion disc with $\Sigma\propto
r^{-3/2}$. 

Hence, our disc is not initialised in a steady state, so we
evolve the disc typically for $\sim 280P(r_0)$, before introducing the
planet.  

When a planet of mass $M_p$ is introduced, we denote its distance to
the primary as $r_p(t)$. It is introduced on a circular orbit, with  
azimuthal velocity including contribution from the disc gravity.
We also define $Q_p\equiv Q(r_p)$,using Eq. \ref{myQ}, to represent
the stability at the planet's initial orbital radius.
We will quote time in units  of the Keplerian orbital period at the
planet's initial radius, $P_0=2\pi/Omega_k(r_p)$. If the planet
is held on fixed circular orbit then $r_p(t)=r_p(t=0)$.  


==> Chapter3/scratch <==
% The energy densities are shown in Fig. \ref{energy_den}.
% ${\mathrm{Re}}(\rho)$ is negative around co-rotation (the internal edge, 
% $r=[5,6]$), which must be attributed to the gravitational energy since
% the pressure contribution is positive definite. This supports the
% interpretation of the disturbace as an edge mode. If it were the
% vortex mode, the total energy near co-rotation would be positive
% because in that case, self-gravity is unimportant compared to
% pressure.  


% Beyond $r\simeq 6.4$, ${\mathrm{Re}}(\rho)$ becomes positive due to pressure and
% oscillates towards the outer boundary as the perturbation becomes
% wave-like. Similarly, pressure perturbation dominates interior to the
% ILR in $r< 3.2$ (not shown). This signifies gravitational energy
% becomes unimportant relative to pressure in these regions. This is
% consistent with the gravitational potential perturbations, which is
% largest near co-rotation. We checked explicitly that the gravitational
% energy is largely focused around the gap edge ($r=[5,6]$), even more
% so than potential perturbation. 

% %because
% %$|W|=|\dd\Sigma|/\Sigma$ becomes large as $\Sigma\to 0$ at the inner
% %boundary). 

% ${\mathrm{Re}}(\rho_\mathrm{wave})$ and ${\mathrm{Re}}(\rho_\mathrm{corot})$ have a
% spurious bump around $r=7.2$ (OLR) that is numerical.
% The eigenfunctions $W,\, \dd\Phi$ are well-defined
% without singularities, but evaluation of
% $\rho_\mathrm{corot}$  and $\rho_\mathrm{wave}$ involve division by
% $D$, which can amplify numerical errors at Lindblad
% resonances ($D\to 0$). We reconcile this issue later. 

% Fig. \ref{energy_den} show that ${\mathrm{Re}}(\rho_\mathrm{corot})$ and 
% ${\mathrm{Re}}(\rho_\mathrm{wave})$ have largest variations within $r=[5,6]$. 
% In this region, ${\mathrm{Re}}(\rho_\mathrm{corot})$ has two negative and one 
% positive peak whereas ${\mathrm{Re}}(\rho_\mathrm{wave})$ has the
% opposite variation. The largest peak at $r\simeq 5.6$ coincide with the
% background vortensity edge (Fig. \ref{linear_basic}); the negative
% co-rotation term is larger in magnitude than the positive wave term,
% resulting in ${\mathrm{Re}}(\rho)<0$. The co-rotation radius $r_c < 5.6$ 
% makes the shifted frequency $\sbar_R(5.6) = m[\Omega(5.6) -
% \Omega(r_c)]<0$. Also at $r=5.6$, $d(\eta^{-1})/dr > 0$, resulting in 
% ${\mathrm{Re}}(\rho_\mathrm{corot}) <0$ at this point.       
% The co-rotation term
% contributes to the gravitational energy of the mode. Because
% vortensity gradients are largest near the gap edge, gravitational
% energy is most negative here and overtakes pressure, resulting in
% negative total energy. Away from the gap edge and towards the outer
% boundary, ${\mathrm{Re}}(\rho_\mathrm{corot})$ is  negligible because vortensity
% gradients are small so gravitational energy becomes negligible and the
% positive total energy density is balanced by
% ${\mathrm{Re}}(\rho_\mathrm{wave})$.    


% Integrating ${\mathrm{Re}}(\rho)$ between $r=[5,10]$, we find
% \begin{align*}
%   U\simeq -5.447
% \end{align*}
% in scaled units. The total energy is negative, which means
% gravitational energy dominates over pressure in $r\geq 5$. 
% %The total energy is negative, which
% %indicate dominant contribution from $\rho_\mathrm{corot}$ (the
% %vortensity term), because the $\rho_\mathrm{wave}$ contributes
% %positively to $U$ beyond $r=8.4$.
% Integrating the co-rotation and wave energy densities, we find
% \begin{align*}
%   & U_\mathrm{corot}\simeq -5.117,\\
%  & U_\mathrm{wave}\simeq -0.4218,
% \end{align*}
% in the same units.  The slight mismatch (by $\sim 2\%$) between $U$
% and $ U_\mathrm{corot} + U_\mathrm{wave}$ is probably numerical
% . The integration range includes OLR, for which
% there is a spurious bump in $\rho_\mathrm{wave}$ and
% $\rho_\mathrm{corot}$ due to numerics. However, we found that when
% integrated over a region around OLR, using the numerically evaluated
% densities, that $U$ approximately equals $ U_\mathrm{corot} +
% U_\mathrm{wave}$. Energy balance is still satisfied in this region
% despite it being subject to numerical error due to the diverging
% factor $1/D$. 


%The region numerically affected by the divering
%factor $1/D$ nearly cancels.
%Suppose we have exact, error-free energy
%densities, then we can write  
%\begin{align*}
%  \int_a^b\rho dr -  \int_\mathrm{OLR}\rho dr
%  =  \int_a^b( \rho_\mathrm{corot} + \rho_\mathrm{wave})dr -
%  \int_\mathrm{OLR} ( \rho_\mathrm{corot} + \rho_\mathrm{wave}) dr.
%\end{align*}
%$\int_\mathrm{OLR}$ denotes integration over a region near the outer
%Lindblad resonance. Now choose this region to be where we believe
%the \emph{numerically} derived values of $\rho_\mathrm{corot}$ and
%$\rho_\mathrm{wave}$ have been affected by the diverging factor $1/D$. 
%The above expression is now applicable to numerical densities  because
%we have excluded the problematic region. Choosing the affect region to
%be $r=[6.4,8.4]$ and using numerical densities, we find
%\begin{align*}
%  &{\mathrm{Re}} \int_\mathrm{OLR}\rho dr \simeq -1.888,\\
%  &{\mathrm{Re}} \int_\mathrm{OLR} ( \rho_\mathrm{corot} + \rho_\mathrm{wave})
%  dr \simeq -1.776,
%\end{align*}
%so in fact, the affected region roughly balances out and the
%$\int_\mathrm{OLR}$ terms nearly cancel. 
%This means we can use the
%numerically energy densities in the equation $U =
%U_\mathrm{corot} + U_\mathrm{wave}$. 

% This means the energy values for $r=[5,10]$ may still be used in
% interpreting energy balance. Then $|U_\mathrm{corot}/ U|\sim 0.9$, so
% the total energy is predominantly due to the vortensity term. 


%We have argued above that the spurious bump in co-rotation and wave
%energy densities do not affact overall energy balance. 



%The arguement can also be applied to a single vortensity edge bounded
%by two extrema. Consider the case of the outer gap edge shown in
%Fig. \ref{linear_basic}. The vortensity edge has $d(\eta^{-1})/dr >
%0$. Labeling the edge radius $r_e$, $\mathrm{min}(\eta^{-1})$ is located
%at $r_\mathrm{min}<r_e$ while $\mathrm{max}(\eta^{-1})$ is at
%$r_\mathrm{max}>r_e$. If co-rotation occurs at $r_c = r_\mathrm{min}$
%then $\sbar(r_e) = m[\Omega(r_e) - \Omega(r_c)] < 0 $
%(ignoring the small growth rates) and  $\rho_\mathrm{corot,1} < 0$
%near the edge. The vortensity edge contributes negatively to total
%energy, leading to the edge mode, driven by self-gravity.   On the
%other hand,  if co-rotation occurs at $r_c = r_\mathrm{max}$
%then $\sbar(r_e) = m[\Omega(r_e) - \Omega(r_c)] > 0 $
%and  $\rho_\mathrm{corot,1} > 0$ near the edge. The vortensity edge
%contributes positively to total energy, leading to the vortex mode,
%driven by pressure.  


%\subsection{Reference case: angular momentum}
%{\bf TO DO}

% For our non-barotropic equation of state, the expression for advective
% angular momentum flux (Eq. \ref{advflux}) becomes:

% \begin{align}\label{advflux3}
%   F_A   &= \frac{m\Sigma}{2}\Im\left[\frac{S}{D^*}(c_s^2 W^\prime +
%       \dd\dd\Phi)^* +
%       \frac{2m\Omega|S|^2\sbar^*}{r\kappa^2 D^*} +
%     \frac{2m\Omega|S|^2}{r\kappa^2\sbar^*}\right] \\\notag
%   & = F_{A,1} + F_{A,2} + F_{A,3},
% \end{align}
% where the $F_{A,i}$'s correspond to terms in square brackets,
% respectively. If the growth rate $\gamma$ is arbitarily small but
% non-zero, then $F_{A,3}$ diverges near co-rotation, as well as the
% angular momentum density $\rho_J$. The equation for angular momentum
% conservation is not very useful in this region. However, the
% definition for Reynolds flux does not involve the factor $1/\sigma$
% and is therefore well-behaved at co-rotation. In
% Fig. \ref{Qm1.5_advflux_reyflux} we compare advective and Reynolds
% fluxes. Using the full expression for $F_A$
% (Fig. \ref{Qm1.5_advflux_reyflux1}) results in large differences
% between the two fluxes near co-rotation. This is due to the singular
% co-rotation term. If we artifically set
% $F_{A,3}$ to zero, then Fig. \ref{Qm1.5_advflux_reyflux2} show the two
% fluxes are similar (even beyond co-rotation, not shown). From earlier
% analysis, similarity between the two is expected for modes with
% $\sigma$ that has a small imaginary part.  

% \begin{figure}[!h]
%   \centering
%   \subfigure[Advective flux using full
%   expression\label{Qm1.5_advflux_reyflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_full.ps}}    
% %  \subfigure[Advective flux using full
% %  expression\label{Qm1.5_advflux_reyflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_full_global.ps}} 
%   \subfigure[Advective flux without
%   $F_{A,3}$\label{Qm1.5_advflux_reyflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_nof3.ps}}  
% % \subfigure[Advective flux without
% %  $F_{A,3}$\label{Qm1.5_advflux_reyflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_nof3_global.ps}}  

%   \caption{A comparison between advective angular momentum flux with
%     using the full expression (a) and that without the $F_{A,3}$
%     term. Dotted curve in each figure shows the Reynolds flux,
%     vertical line is co-rotation and horizontal line indicate zero
%     flux. 
% \label{Qm1.5_advflux_reyflux}}
% \end{figure}


% The linear results typically give growth rates $|\gamma|$ that is a few
% per cent of $\sigma_R$. These are slowly growing modes where the
% eigenfrequency is almost real. In the case $\sigma$ is real, advective
% and Reynold fluxes are identical and equal to $F_A = F_{A,1}
% m\Sigma\Im[S(c_s^2 W^\prime + \dd\dd\Phi)^*]/2D$.

% \begin{figure}[!h]
%   \centering
%   \subfigure[$F_A$ and
%   $F_R$\label{Qm1.5_linear_advflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_reyflux.ps}}  
%   \subfigure[$F_{A,1}$\label{Qm1.5_linear_advflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_realsigma.ps}}    
%   \caption{Advective and Reynolds angular momentum fluxes (a) and the
%     advective flux when $\sigma$ is regarded as real (b).
%     Vertical lines indicated co-rotation and horizontal
%     lines indicate zero flux.  
% \label{Qm1.5_linear_advflux}}
% \end{figure}

% Fig. \ref{Qm1.5_linear_advflux1} compares the advective flux
% $F_A$ to the Reynolds flux $F_R = r\Sigma{\mathrm{Re}}(\dd u_r \dd
% u_\phi^*)/2$. Near co-rotation, $F_R$ is well behaved because  it does
% not involve the factor $1/\sbar$. $F_A$ is very similar to $F_R$
% around co-rotation, despite the fact that we have artifically
% neglected $F_{A,3}$ in the full expression for $F_A$. Both curves
% indicate outwards transport of angular momentum by fluid flow
% (advection or Reynolds stresses) across co-rotation. Away from
% co-rotation, the two curves are still similar, as expected
% from earlier analysis for modes with small $|\gamma|$. The
% formula for $F_A$ and $F_R$ involve factors $1/D$ and $1/D^2$,
% respectively. The peaks at $r\simeq 3.4,\,7.3$ correspond to inner and
% outer Lindblad resonances, respectively, where ${\mathrm{Re}}(D)\to 0$. 
% %Applying L'H\^{o}pital's rule at the ILR gives a flux value
% %between those on either side of the resonance, whereas application at
% %OLR does not give an intermediate value. This suggests that the inner 
% %$|D|$ is non-zero
% %because $\gamma\neq 0$, although there could be contribution from
% %finite resolution.
% Although $F_R$ involves an additional factor
% of $1/D$ compared to $F_A$, this does not affect the sharpness of
% these peaks. These peaks are likely to have significant numerical
% contribution. 

% In Fig. \ref{Qm1.5_linear_advflux2} we show the angular momentum flux
% when $\sigma$ is real. This is just $F_{A,1}$ with $\gamma$
% artifically set to zero. In this case, advective and
% Reynolds fluxes are identical. $|D|$ now vanishes at Lindblad
% resonances, and although there is no true singularity there is one
% due to finite resolution. We have smoothed out the
% region around Lindblad resonances by applying L'H\^{o}pital's rule. Of course,
% this does not affect the flux near co-rotation. The peaks at Lindblad
% resonances are removed, resulting in negative fluxes. This suggests
% the peaks in the previous figure is numerical. 
 
% If we regard the region $r>r_c\simeq 5.5$ as an isolated system, there
% there is a positive angular momentum flux into its inner boundary,
% this is associated with the gap edge.  

% The definition of the gravity flux require 3D solution to the
% perturbed potential, whereas the linearised equations only give
% $\dd\Phi$ evaluated in the disc plane. However, the gravity flux is
% related to the perturbation variables by $\p_r(rF_G) =
% rm\Im(\dd\Sigma\dd\Phi^*)/2$. If we neglect the gravity flux at the
% innermost boundary, then we have
% \begin{align}
%   F_G = \frac{m}{2r}\int_{r_1}^{r} r \Im(\dd\Sigma\dd\Phi^*) dr^\prime.
% \end{align}
%  The gravity flux is shown in Fig. \ref{Qm1.5_linear_gravflux}.

% \begin{figure}[!h]
%   \centering
%   \subfigure[$F_G$]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_gravflux.ps}}   
%   \subfigure[Torque]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_gravtorque.ps}}
%   \caption{Gravity flux and corresponding gravity torque for the reference case.
% \label{Qm1.5_linear_gravflux}}
% \end{figure}


%The least self-gravitating disc, $Q_m=1.6$, displays an interesting
%double-peak in growth rates. This could be because as $Q_m$ is
%increased and edge modes are stabilised, and the preferred $m$ for
%edge modes to exist is reduced. 

%Preliminary
%simulations in \S\ref{hydro1} show that  increasing $Q_m$ eventually
%favour vortex modes. We therefore expect some intermediate disc mass
%where vortex modes and edge modes have similar growth rates and both
%can develop.   

%Recall also that perturbation theory predicts the
%destabilisation of modes with co-rotation at vortensity
%maximum (applicable to low $m$ solutions). 

%Spiral modes considered here have maximum growth rates for
%low $m$. For the reference disc $Q_m=1.5$, the most unstable mode is
%$m=2$ consistent with simulation. Although linear calculations give
%similar growth rates for $m=3$---5, these higher $m$ modes are not
%seen in simulations where a standard viscosity $\nu=10^{-5}$ was
%used. In a non-self-gravitating disc, this viscosity surpress the
%vortex modes which typically have $m=3$---4. 

%The $m=8$ mode for
%$Q_m=1.5$ is shown in Fig. \ref{Qm1.5_linear_m8}.  These 
%high $m$ modes in massive discs do not look like the
%non-self-gravitating vortex modes or edge modes describe above,
%because there is no concentration of disturbance around co-rotation.  

%Using Fig. \ref{linear_basic}, its
%co-rotation point $r_c=5.7$ is in fact just inside
%$\mathrm{min}(\eta^{-1})$, whereas the non-self-gravitating mode has
%$r_c=5.8$ which is just outside $\mathrm{min}(\eta^{-1})$. 

%Increasing $Q_m$ further one expects the emergence of vortex modes. In
%Fig. \ref{compare_gamma_and_corot}, the
%multiply-peaked growth rate for the $Q_m=1.6$ solution is comparable to
%the $Q_m=2$ curve in Fig. \ref{compare_v} from Chapter
%\ref{vortex}. These intermediate $Q_m$'s permit both vortex and spiral
%modes.  


% \begin{figure}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figures/varQ_basic.ps}
%   \includegraphics[width=0.45\textwidth]{figures/varQ_basic_sigma.ps}
%   \caption{Comparison of gap profile basic states opened by a
%     Saturn-mass planet in a range of discs, in terms of the Toomre $Q$
%     parameter. 
% \label{varQ_basic}}
% \end{figure}



%The high-$m$ modes are absent in the simulations. These disturbances
%have short wave-lengths and more easily stabilised by viscosity, which
%was used in the simulations but not in linear theory. The standard
%viscosity $\nu=10^{-5}$ surpress vortex modes, which typically have
%$m\geq 4$.  


% \begin{table}
%   \centering
%   \caption{table}{Result for various azimuthal mode numbers
%     $m$, for the standard disc with $Q_m=1.5$. \label{Qm1.5_varm}}   
%   \begin{tabular}{cccccccccc}
%     \hline\hline
%     $m$ & $-\sigma_R$ & $-\gamma\times10^{2}$ &  $r_c$ &$-U$ & $-U_\mathrm{corot}$
%     & $-U_\mathrm{wave}$ &  $-U_D$ & $-U_\mathrm{corot,D}$ &
%     $-U_\mathrm{wave,D}$\\ 
%     \hline
%     1 & 0.0794 & 0.2701 & 5.4538 & 42.13 & 21.77 & 15.46 & 16.98 &
%     11.00 & 5.90 \\

%     2 & 0.1587 & 0.4515 & 5.4626 & 5.447 & 5.117 & 0.4281 & 3.133 &
%     2.576 & 0.5596 \\

%     3 & 0.2366 & 0.4042 & 5.4977 & -0.8773 & 2.250 & -3.086 & -3.696 & 
%     1.258 & -4.9304 \\

%     4 & 0.3131 & 0.4117 & 5.5327 & -2.914 & 0.5548 & -3.431 & -13.27 & 
%     0.3488 & -13.61 \\

%     5 & 0.3863 & 0.3662 & 5.5854 & -5.998 & 0.3282 & -6.221 & -55.72 & 
%     0.2660 & -55.91 \\

%     6 & 0.4620 & 0.0501 & 5.6029 & -4.811 & 0.2030 & -4.991 & -94.78 & 
%     0.1385 & -94.55 \\

%     7 & 0.5243 & 0.2226 & 5.6994 & -12.42 & -1.031 & -11.24 & -342.4 & 
%     0.3475 & -341.3 \\

%     8 & 0.5993 & 0.1894 & 5.6994 & -5.733 & -0.382 & -5.302 & -271.5 & 
%     0.2658 & -270.2 \\
%    \hline
%   \end{tabular}
% \end{table}



%   \begin{tabular}{ccccccc}
%     \hline\hline
%     $m$ & $-\sigma_R$ & $\gamma\times10^{2}$ & $r_c$ & $-\tilde{U}$ &
%     $-\tilde{U}_\mathrm{corot}$ & $-\tilde{U}_\mathrm{wave}$\\ 
%     \hline
%  %   1 & 0.0794 & 0.2701 & 5.4538  & 16.98 &
%  %   11.00 & 5.90 \\
%     1 & 0.079 & 0.270 & 5.454  & 17.0 &
%    11.0 & 5.90 \\
  
% %    2 & 0.1587 & 0.4515 & 5.4626  & 3.133 &
% %    2.576 & 0.5596 \\

%     2 & 0.159 & 0.452 & 5.463  & 3.13 &
%     2.58 & 0.560 \\

% %    3 & 0.2366 & 0.4042 & 5.4977  &-3.696 & 
% %    1.258 & -4.9304 \\

%     3 & 0.237 & 0.404 & 5.498  &-3.70 & 
%     1.26 & -4.93 \\

% %    4 & 0.3131 & 0.4117 & 5.5327  &-13.27 & 
% %    0.3488 & -13.61 \\

%     4 & 0.313 & 0.412 & 5.533  &-13.3 & 
%     0.349 & -13.6 \\

% %    5 & 0.3863 & 0.3662 & 5.5854  & -55.72 & 
% %    0.2660 & -55.91 \\

%     5 & 0.386 & 0.366 & 5.585  & -55.7 & 
%     0.266 & -55.9 \\

% %    6 & 0.4620 & 0.2415 & 5.6029  & -94.78 & 
% %    0.1385 & -94.55 \\

%     6 & 0.462 & 0.242 & 5.603  & -94.8 & 
%     0.139 & -94.6 \\

% %    7 & 0.5243 & 0.2226 & 5.6994  & -342.4 & 
% %    0.3475 & -341.3 \\

%     7 & 0.524 & 0.223 & 5.699  & -342.4 & 
%     0.348 & -341.3 \\

% %    8 & 0.5993 & 0.1894 & 5.6994  & -271.5 & 
% %    0.2658 & -270.2 \\

%     8 & 0.599 & 0.189 & 5.699  & -271.5 & 
%     0.269 & -270.2 \\



% We performed further calculations with different softening parameters
% $\epsilon_0$, such that $0.05\epsilon_0r$ is the softening
% length. Ideally $\epsilon_0$ for basic state,
% denoted $\epsilon_{0,\mathrm{eqm}}$ should be the same as that used in
% liner calculations, denoted $\epsilon_{0,\mathrm{lin}}$. However,
% because the equilibrium disc was setup through hydrodynamic simulations,
% requring self-consistent softening lengths means a new run must be
% performed for each new softening parameter condsidered. To avoid
% additional computation cost, only two $\epsilon_{0,\mathrm{eqm}}$
% values are considered, we then vary $\epsilon_{0,\mathrm{lin}}$ in the
% linear code. 

% Results for various $\epsilon_{0,\mathrm{eqm}}$ and
% $\epsilon_{0,\mathrm{lin}}$ are summarised in Table \ref{soft_expts}. The
% eigenvalues, energies and modified energies are listed. Modified
% energies are less prone to numerical errors. The co-rotation
% (vortensity) contributions have \emph{not} been further decomposed as
% described in \S\ref{furtherdecomp}. 




% \begin{table}
%   \centering
%   \caption{table}{Linear calculations for different softening
%     parameters, for the $Q_m=1.5$ reference disc and azimuthal mode
%     $m=2$. \label{soft_expts}}   
%   \begin{tabular}{cccccccccc}
%     \hline\hline
%     $\epsilon_{g0},\, \mathrm{lin.}$ & $\epsilon_{g0},\, mathrm{eqm.}$ &
%     $-\sigma_R$ & $-\gamma\times10^{2}$  & $-U$ & $-U_\mathrm{corot}
%     $ $-U_\mathrm{wave}$ & $-\tilde{U}$ &
%     $-\tilde{U}_\mathrm{corot}$ &  $-\tilde{U}_\mathrm{wave}$\\ 
%     \hline
%     0.1 & 0.3 & 0.159 & 0.508 & 11.4 & 7.80 & 3.61 & 5.33 & 3.65 &
%     1.58 \\
%     0.2 & 0.3 & 0.159 & 0.461 & 6.88 & 5.39 & 1.47 & 3.57 & 2.66 &
%     0.84 \\    
%     0.3 & 0.3 & 0.159 & 0.452 & 5.45 & 5.12 & 0.42 & 3.13 & 2.58 &
%     0.56 \\
%     0.4 & 0.3 & 0.159 & 0.454 & 6.00 & 5.76 & 0.36 & 3.39 & 2.89 &
%     0.57 \\
%     0.5 & 0.3 & 0.158 & 0.435 & 6.47 & 6.31 & 0.27 & 3.61 & 3.13 &
%     0.52 \\

%     0.2 & 0.6 & 0.159 & 0.426 & 6.05 & 5.28 & 0.75 & 3.23 & 2.62 &
%     0.54 \\
%     0.3 & 0.6 & 0.159 & 0.420 & 4.57 & 5.07 & -0.40 & 2.79 & 2.55 &
%     0.25 \\
%     0.4 & 0.6 & 0.158 & 0.428 & 5.36 & 5.96 & -0.47 & 3.13 & 2.92 &
%     0.26 \\
%     0.5 & 0.6 & 0.158 & 0.410 & 6.01 & 6.70 & -0.58 & 3.44 & 3.28 &
%     0.21 \\
%     0.6 & 0.6 & 0.158 & 0.375 & 6.09 & 7.09 & -0.92 & 3.54 & 3.52 &
%     0.061 \\
%     0.7 & 0.6 & 0.158 & 0.329 & 5.62 & 7.15 & -1.48 & 3.44 & 3.65 &
%     -0.17 \\
%     0.8 & 0.6 & 0.158 & 0.276 & 4.71 & 6.93 & -2.19 & 3.18 & 3.67 &
%     -0.46 \\
%    \hline
%   \end{tabular}
% \end{table}



%   \begin{tabular}{ccccccc}
%     \hline\hline
%     $\epsilon_{g0,l}$ & $\epsilon_{g0,e}$ &
%     $-\sigma_R$ & $\gamma\times10^{2}$  &  $-\tilde{U}$ &
%     $-\tilde{U}_\mathrm{corot}$ &  $-\tilde{U}_\mathrm{wave}$\\ 
%     \hline
%     0.1 & 0.3 & 0.159 & 0.508  & 5.33 & 3.65 &
%     1.58 \\
% %    0.2 & 0.3 & 0.159 & 0.461  & 3.57 & 2.66 &
% %    0.84 \\    
%     0.3 & 0.3 & 0.159 & 0.452  & 3.13 & 2.58 &
%     0.56 \\
% %    0.4 & 0.3 & 0.159 & 0.454  & 3.39 & 2.89 &
% %    0.57 \\
%     0.5 & 0.3 & 0.158 & 0.435  & 3.61 & 3.13 &
%     0.52 \\

% %    0.2 & 0.6 & 0.159 & 0.426  & 3.23 & 2.62 &
% %    0.54 \\
%     0.3 & 0.6 & 0.159 & 0.420  & 2.79 & 2.55 &
%     0.25 \\
% %    0.4 & 0.6 & 0.158 & 0.428  & 3.13 & 2.92 &
% %    0.26 \\
%     0.5 & 0.6 & 0.158 & 0.410  & 3.44 & 3.28 &
%     0.21 \\
%     0.6 & 0.6 & 0.158 & 0.375  & 3.54 & 3.52 &
%     0.061 \\
% %    0.7 & 0.6 & 0.158 & 0.329  & 3.44 & 3.65 &
% %    -0.17 \\
%     0.8 & 0.6 & 0.158 & 0.276  & 3.18 & 3.67 &
%     -0.46 \\


%************
%
%{\bf This desn't seem like a big change..were other kinds
%of boundary condition tried?}
%
%*************

==> Chapter3/scratch_ <==
% The energy densities are shown in Fig. \ref{energy_den}.
% ${\mathrm{Re}}(\rho)$ is negative around co-rotation (the internal edge, 
% $r=[5,6]$), which must be attributed to the gravitational energy since
% the pressure contribution is positive definite. This supports the
% interpretation of the disturbace as an edge mode. If it were the
% vortex mode, the total energy near co-rotation would be positive
% because in that case, self-gravity is unimportant compared to
% pressure.  


% Beyond $r\simeq 6.4$, ${\mathrm{Re}}(\rho)$ becomes positive due to pressure and
% oscillates towards the outer boundary as the perturbation becomes
% wave-like. Similarly, pressure perturbation dominates interior to the
% ILR in $r< 3.2$ (not shown). This signifies gravitational energy
% becomes unimportant relative to pressure in these regions. This is
% consistent with the gravitational potential perturbations, which is
% largest near co-rotation. We checked explicitly that the gravitational
% energy is largely focused around the gap edge ($r=[5,6]$), even more
% so than potential perturbation. 

% %because
% %$|W|=|\dd\Sigma|/\Sigma$ becomes large as $\Sigma\to 0$ at the inner
% %boundary). 

% ${\mathrm{Re}}(\rho_\mathrm{wave})$ and ${\mathrm{Re}}(\rho_\mathrm{corot})$ have a
% spurious bump around $r=7.2$ (OLR) that is numerical.
% The eigenfunctions $W,\, \dd\Phi$ are well-defined
% without singularities, but evaluation of
% $\rho_\mathrm{corot}$  and $\rho_\mathrm{wave}$ involve division by
% $D$, which can amplify numerical errors at Lindblad
% resonances ($D\to 0$). We reconcile this issue later. 

% Fig. \ref{energy_den} show that ${\mathrm{Re}}(\rho_\mathrm{corot})$ and 
% ${\mathrm{Re}}(\rho_\mathrm{wave})$ have largest variations within $r=[5,6]$. 
% In this region, ${\mathrm{Re}}(\rho_\mathrm{corot})$ has two negative and one 
% positive peak whereas ${\mathrm{Re}}(\rho_\mathrm{wave})$ has the
% opposite variation. The largest peak at $r\simeq 5.6$ coincide with the
% background vortensity edge (Fig. \ref{linear_basic}); the negative
% co-rotation term is larger in magnitude than the positive wave term,
% resulting in ${\mathrm{Re}}(\rho)<0$. The co-rotation radius $r_c < 5.6$ 
% makes the shifted frequency $\sbar_R(5.6) = m[\Omega(5.6) -
% \Omega(r_c)]<0$. Also at $r=5.6$, $d(\eta^{-1})/dr > 0$, resulting in 
% ${\mathrm{Re}}(\rho_\mathrm{corot}) <0$ at this point.       
% The co-rotation term
% contributes to the gravitational energy of the mode. Because
% vortensity gradients are largest near the gap edge, gravitational
% energy is most negative here and overtakes pressure, resulting in
% negative total energy. Away from the gap edge and towards the outer
% boundary, ${\mathrm{Re}}(\rho_\mathrm{corot})$ is  negligible because vortensity
% gradients are small so gravitational energy becomes negligible and the
% positive total energy density is balanced by
% ${\mathrm{Re}}(\rho_\mathrm{wave})$.    


% Integrating ${\mathrm{Re}}(\rho)$ between $r=[5,10]$, we find
% \begin{align*}
%   U\simeq -5.447
% \end{align*}
% in scaled units. The total energy is negative, which means
% gravitational energy dominates over pressure in $r\geq 5$. 
% %The total energy is negative, which
% %indicate dominant contribution from $\rho_\mathrm{corot}$ (the
% %vortensity term), because the $\rho_\mathrm{wave}$ contributes
% %positively to $U$ beyond $r=8.4$.
% Integrating the co-rotation and wave energy densities, we find
% \begin{align*}
%   & U_\mathrm{corot}\simeq -5.117,\\
%  & U_\mathrm{wave}\simeq -0.4218,
% \end{align*}
% in the same units.  The slight mismatch (by $\sim 2\%$) between $U$
% and $ U_\mathrm{corot} + U_\mathrm{wave}$ is probably numerical
% . The integration range includes OLR, for which
% there is a spurious bump in $\rho_\mathrm{wave}$ and
% $\rho_\mathrm{corot}$ due to numerics. However, we found that when
% integrated over a region around OLR, using the numerically evaluated
% densities, that $U$ approximately equals $ U_\mathrm{corot} +
% U_\mathrm{wave}$. Energy balance is still satisfied in this region
% despite it being subject to numerical error due to the diverging
% factor $1/D$. 


%The region numerically affected by the divering
%factor $1/D$ nearly cancels.
%Suppose we have exact, error-free energy
%densities, then we can write  
%\begin{align*}
%  \int_a^b\rho dr -  \int_\mathrm{OLR}\rho dr
%  =  \int_a^b( \rho_\mathrm{corot} + \rho_\mathrm{wave})dr -
%  \int_\mathrm{OLR} ( \rho_\mathrm{corot} + \rho_\mathrm{wave}) dr.
%\end{align*}
%$\int_\mathrm{OLR}$ denotes integration over a region near the outer
%Lindblad resonance. Now choose this region to be where we believe
%the \emph{numerically} derived values of $\rho_\mathrm{corot}$ and
%$\rho_\mathrm{wave}$ have been affected by the diverging factor $1/D$. 
%The above expression is now applicable to numerical densities  because
%we have excluded the problematic region. Choosing the affect region to
%be $r=[6.4,8.4]$ and using numerical densities, we find
%\begin{align*}
%  &{\mathrm{Re}} \int_\mathrm{OLR}\rho dr \simeq -1.888,\\
%  &{\mathrm{Re}} \int_\mathrm{OLR} ( \rho_\mathrm{corot} + \rho_\mathrm{wave})
%  dr \simeq -1.776,
%\end{align*}
%so in fact, the affected region roughly balances out and the
%$\int_\mathrm{OLR}$ terms nearly cancel. 
%This means we can use the
%numerically energy densities in the equation $U =
%U_\mathrm{corot} + U_\mathrm{wave}$. 

% This means the energy values for $r=[5,10]$ may still be used in
% interpreting energy balance. Then $|U_\mathrm{corot}/ U|\sim 0.9$, so
% the total energy is predominantly due to the vortensity term. 


%We have argued above that the spurious bump in co-rotation and wave
%energy densities do not affact overall energy balance. 



%The arguement can also be applied to a single vortensity edge bounded
%by two extrema. Consider the case of the outer gap edge shown in
%Fig. \ref{linear_basic}. The vortensity edge has $d(\eta^{-1})/dr >
%0$. Labeling the edge radius $r_e$, $\mathrm{min}(\eta^{-1})$ is located
%at $r_\mathrm{min}<r_e$ while $\mathrm{max}(\eta^{-1})$ is at
%$r_\mathrm{max}>r_e$. If co-rotation occurs at $r_c = r_\mathrm{min}$
%then $\sbar(r_e) = m[\Omega(r_e) - \Omega(r_c)] < 0 $
%(ignoring the small growth rates) and  $\rho_\mathrm{corot,1} < 0$
%near the edge. The vortensity edge contributes negatively to total
%energy, leading to the edge mode, driven by self-gravity.   On the
%other hand,  if co-rotation occurs at $r_c = r_\mathrm{max}$
%then $\sbar(r_e) = m[\Omega(r_e) - \Omega(r_c)] > 0 $
%and  $\rho_\mathrm{corot,1} > 0$ near the edge. The vortensity edge
%contributes positively to total energy, leading to the vortex mode,
%driven by pressure.  


%\subsection{Reference case: angular momentum}
%{\bf TO DO}

% For our non-barotropic equation of state, the expression for advective
% angular momentum flux (Eq. \ref{advflux}) becomes:

% \begin{align}\label{advflux3}
%   F_A   &= \frac{m\Sigma}{2}\Im\left[\frac{S}{D^*}(c_s^2 W^\prime +
%       \dd\dd\Phi)^* +
%       \frac{2m\Omega|S|^2\sbar^*}{r\kappa^2 D^*} +
%     \frac{2m\Omega|S|^2}{r\kappa^2\sbar^*}\right] \\\notag
%   & = F_{A,1} + F_{A,2} + F_{A,3},
% \end{align}
% where the $F_{A,i}$'s correspond to terms in square brackets,
% respectively. If the growth rate $\gamma$ is arbitarily small but
% non-zero, then $F_{A,3}$ diverges near co-rotation, as well as the
% angular momentum density $\rho_J$. The equation for angular momentum
% conservation is not very useful in this region. However, the
% definition for Reynolds flux does not involve the factor $1/\sigma$
% and is therefore well-behaved at co-rotation. In
% Fig. \ref{Qm1.5_advflux_reyflux} we compare advective and Reynolds
% fluxes. Using the full expression for $F_A$
% (Fig. \ref{Qm1.5_advflux_reyflux1}) results in large differences
% between the two fluxes near co-rotation. This is due to the singular
% co-rotation term. If we artifically set
% $F_{A,3}$ to zero, then Fig. \ref{Qm1.5_advflux_reyflux2} show the two
% fluxes are similar (even beyond co-rotation, not shown). From earlier
% analysis, similarity between the two is expected for modes with
% $\sigma$ that has a small imaginary part.  

% \begin{figure}[!h]
%   \centering
%   \subfigure[Advective flux using full
%   expression\label{Qm1.5_advflux_reyflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_full.ps}}    
% %  \subfigure[Advective flux using full
% %  expression\label{Qm1.5_advflux_reyflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_full_global.ps}} 
%   \subfigure[Advective flux without
%   $F_{A,3}$\label{Qm1.5_advflux_reyflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_nof3.ps}}  
% % \subfigure[Advective flux without
% %  $F_{A,3}$\label{Qm1.5_advflux_reyflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_advflux_reyflux_nof3_global.ps}}  

%   \caption{A comparison between advective angular momentum flux with
%     using the full expression (a) and that without the $F_{A,3}$
%     term. Dotted curve in each figure shows the Reynolds flux,
%     vertical line is co-rotation and horizontal line indicate zero
%     flux. 
% \label{Qm1.5_advflux_reyflux}}
% \end{figure}


% The linear results typically give growth rates $|\gamma|$ that is a few
% per cent of $\sigma_R$. These are slowly growing modes where the
% eigenfrequency is almost real. In the case $\sigma$ is real, advective
% and Reynold fluxes are identical and equal to $F_A = F_{A,1}
% m\Sigma\Im[S(c_s^2 W^\prime + \dd\dd\Phi)^*]/2D$.

% \begin{figure}[!h]
%   \centering
%   \subfigure[$F_A$ and
%   $F_R$\label{Qm1.5_linear_advflux1}]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_reyflux.ps}}  
%   \subfigure[$F_{A,1}$\label{Qm1.5_linear_advflux2}]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_realsigma.ps}}    
%   \caption{Advective and Reynolds angular momentum fluxes (a) and the
%     advective flux when $\sigma$ is regarded as real (b).
%     Vertical lines indicated co-rotation and horizontal
%     lines indicate zero flux.  
% \label{Qm1.5_linear_advflux}}
% \end{figure}

% Fig. \ref{Qm1.5_linear_advflux1} compares the advective flux
% $F_A$ to the Reynolds flux $F_R = r\Sigma{\mathrm{Re}}(\dd u_r \dd
% u_\phi^*)/2$. Near co-rotation, $F_R$ is well behaved because  it does
% not involve the factor $1/\sbar$. $F_A$ is very similar to $F_R$
% around co-rotation, despite the fact that we have artifically
% neglected $F_{A,3}$ in the full expression for $F_A$. Both curves
% indicate outwards transport of angular momentum by fluid flow
% (advection or Reynolds stresses) across co-rotation. Away from
% co-rotation, the two curves are still similar, as expected
% from earlier analysis for modes with small $|\gamma|$. The
% formula for $F_A$ and $F_R$ involve factors $1/D$ and $1/D^2$,
% respectively. The peaks at $r\simeq 3.4,\,7.3$ correspond to inner and
% outer Lindblad resonances, respectively, where ${\mathrm{Re}}(D)\to 0$. 
% %Applying L'H\^{o}pital's rule at the ILR gives a flux value
% %between those on either side of the resonance, whereas application at
% %OLR does not give an intermediate value. This suggests that the inner 
% %$|D|$ is non-zero
% %because $\gamma\neq 0$, although there could be contribution from
% %finite resolution.
% Although $F_R$ involves an additional factor
% of $1/D$ compared to $F_A$, this does not affect the sharpness of
% these peaks. These peaks are likely to have significant numerical
% contribution. 

% In Fig. \ref{Qm1.5_linear_advflux2} we show the angular momentum flux
% when $\sigma$ is real. This is just $F_{A,1}$ with $\gamma$
% artifically set to zero. In this case, advective and
% Reynolds fluxes are identical. $|D|$ now vanishes at Lindblad
% resonances, and although there is no true singularity there is one
% due to finite resolution. We have smoothed out the
% region around Lindblad resonances by applying L'H\^{o}pital's rule. Of course,
% this does not affect the flux near co-rotation. The peaks at Lindblad
% resonances are removed, resulting in negative fluxes. This suggests
% the peaks in the previous figure is numerical. 
 
% If we regard the region $r>r_c\simeq 5.5$ as an isolated system, there
% there is a positive angular momentum flux into its inner boundary,
% this is associated with the gap edge.  

% The definition of the gravity flux require 3D solution to the
% perturbed potential, whereas the linearised equations only give
% $\dd\Phi$ evaluated in the disc plane. However, the gravity flux is
% related to the perturbation variables by $\p_r(rF_G) =
% rm\Im(\dd\Sigma\dd\Phi^*)/2$. If we neglect the gravity flux at the
% innermost boundary, then we have
% \begin{align}
%   F_G = \frac{m}{2r}\int_{r_1}^{r} r \Im(\dd\Sigma\dd\Phi^*) dr^\prime.
% \end{align}
%  The gravity flux is shown in Fig. \ref{Qm1.5_linear_gravflux}.

% \begin{figure}[!h]
%   \centering
%   \subfigure[$F_G$]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_gravflux.ps}}   
%   \subfigure[Torque]{\includegraphics[width=0.45\textwidth]{Qm1.5_linear_advflux_gravtorque.ps}}
%   \caption{Gravity flux and corresponding gravity torque for the reference case.
% \label{Qm1.5_linear_gravflux}}
% \end{figure}


%The least self-gravitating disc, $Q_m=1.6$, displays an interesting
%double-peak in growth rates. This could be because as $Q_m$ is
%increased and edge modes are stabilised, and the preferred $m$ for
%edge modes to exist is reduced. 

%Preliminary
%simulations in \S\ref{hydro1} show that  increasing $Q_m$ eventually
%favour vortex modes. We therefore expect some intermediate disc mass
%where vortex modes and edge modes have similar growth rates and both
%can develop.   

%Recall also that perturbation theory predicts the
%destabilisation of modes with co-rotation at vortensity
%maximum (applicable to low $m$ solutions). 

%Spiral modes considered here have maximum growth rates for
%low $m$. For the reference disc $Q_m=1.5$, the most unstable mode is
%$m=2$ consistent with simulation. Although linear calculations give
%similar growth rates for $m=3$---5, these higher $m$ modes are not
%seen in simulations where a standard viscosity $\nu=10^{-5}$ was
%used. In a non-self-gravitating disc, this viscosity surpress the
%vortex modes which typically have $m=3$---4. 

%The $m=8$ mode for
%$Q_m=1.5$ is shown in Fig. \ref{Qm1.5_linear_m8}.  These 
%high $m$ modes in massive discs do not look like the
%non-self-gravitating vortex modes or edge modes describe above,
%because there is no concentration of disturbance around co-rotation.  

%Using Fig. \ref{linear_basic}, its
%co-rotation point $r_c=5.7$ is in fact just inside
%$\mathrm{min}(\eta^{-1})$, whereas the non-self-gravitating mode has
%$r_c=5.8$ which is just outside $\mathrm{min}(\eta^{-1})$. 

%Increasing $Q_m$ further one expects the emergence of vortex modes. In
%Fig. \ref{compare_gamma_and_corot}, the
%multiply-peaked growth rate for the $Q_m=1.6$ solution is comparable to
%the $Q_m=2$ curve in Fig. \ref{compare_v} from Chapter
%\ref{vortex}. These intermediate $Q_m$'s permit both vortex and spiral
%modes.  


% \begin{figure}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figures/varQ_basic.ps}
%   \includegraphics[width=0.45\textwidth]{figures/varQ_basic_sigma.ps}
%   \caption{Comparison of gap profile basic states opened by a
%     Saturn-mass planet in a range of discs, in terms of the Toomre $Q$
%     parameter. 
% \label{varQ_basic}}
% \end{figure}

==> Makefile <==
VERSION=
LATEXTARGET=thesis$(VERSION)

#
# LaTeX Makefile
# --------------
#
# Author : s.m.vandenoord@student.utwente.nl (Stefan van den Oord)
# Date   : March 18, 1999, second version of today.
# 
# This Makefile is a generic makefile for LaTeX documents. Distribute it
# as you wish, but please don't edit or remove this initial comment.
#
# The Makefile can be used by setting the environment variable "MAKEFILES",
# e.g. export MAKEFILES=~/data/TeX/Makefile.
# It requires GNU Make and bash or better, like zsh. Simply sh is not
# sufficient, I believe. The first few lines of the Makefile contains
# the executables that are used, edit them to point to the executables
# on your system.
#
# DISCLAIMER: Using this Makefile is fully at your own risk. I am not
#             responsible for anything! So if crucial files are removed
#             by the Makefile, it is your own problem. But you should
#             have backups anyway. :-)
#
# Usage
# -----
# The Makefile can do the following things for you:
# - generate PostScript equivalents of XFig figures;
# - run makeindex and BibTeX, but only if necessary;
# - compile the .dvi file, running LaTeX as many times as needed;
# - run XDvi with the compiled .dvi file;
# - create a PostScript equivalent of the .dvi file;
# - generate a HTML equivalent of the .dvi file (if Latex2HTML is
#   installed);
# - remove all generated output.
# The Makefile is in some points even RCS aware.
#
# In many cases, you don't even have to tell the Makefile which LaTeX
# file it has to compile. The Makefile uses the following strategy:
# 1. Check if the environment variable LATEXTARGET is set; if it is,
#    generate $LATEXTARGET.dvi.
# 2. If there is only one .tex file, use that one.
# 3. Check if there is a LaTeX file that has the same basename as the
#    directory. For example, if the directory is named "Thesis" and
#    there is a file "Thesis.tex", "Thesis.dvi" is generated.
#
# Invocation
# ----------
# When the MAKEFILES environment variable is set, you can use the
# following commands:
# - make latexhelp
#   Prints an overview of the available commands.
# - make latexfigures
#   Only generate the PostScript equivalents of XFig figures.
# - make file.dvi
#   Generates the specified DVI file.
# - make file.ps
#   Generates the DVI file and then runs dvips.
# - make latex
#   Use the above explained strategy to find out what has to be
#   generated, and generate it.
# - make view
#   Do a make latex and then run XDvi.
# - make latexps
#   Do a make latex and then run dvips.
# - make html
#   Do a make latex and then use LaTeX2HTML to create the HTML equivalent.
#   To do this, the following environment variables are used:
#   * HTMLDIR : the base dir in which the output is written. For example,
#               if HTMLDIR=~/public_html/LaTeX, and the file that is
#               generated is "Thesis", the output will be written in the
#               directory ~/public_html/LaTeX/Thesis.
#   * LATEX2HTML_OPTS : if you want to pass options to LaTeX2HTML, put
#                       them in this variable.
# - make latexclean
#   This command removes all generated output. CAUTION: the files that are
#   removed are thought out pretty well, but it is possible that files are
#   removed that you wanted to keep! Check below what files are removed if
#   you want to be certain!
#   Note that a file figure.eps is only removed if a file figure.fig exists.
#   (Even if the file figure.fig exists, but is checked in using RCS, the
#   file figure.eps will be removed.)
#
# Tip
# ---
# For some projects it is useful to have a separate Makefile in the project's
# directory. For example, when you use RCS, you could add functionality for
# automatic checkouts of the right files (adding dependencies is sufficient;
# GNU Make rocks :-).
# The command "latexclean" is declared so that you can add your own
# functionality in the project's Makefile; instead of one colon, declare it
# with two colons if you want to do that.
# For example:
# latexclean::
#     rm -f foo.bar
# This way both the origional definition in this Makefile and your own are
# used.

#.SILENT:

# SHELL=/usr/local/bin/bash

LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIPS=dvips
MAKEINDEX=makeindex
DVIVIEWER=xdvi -geometry 710x950-0+10
LATEX2HTML=latex2html

FIGURES=$(wildcard *.fig)
FIGUREOBJS=$(FIGURES:.fig=.eps)

TEXFILES=$(wildcard *.tex)

# Disable standard pattern rule:
%.dvi: %.tex

# Do not delete the following targets:
.PRECIOUS: %.aux %.bbl %.eps %.ind

%.aux: %.tex $(FIGUREOBJS) $(TEXFILES)
	@$(LATEX) $*
# Look for citations. Make sure grep never returns an error code.
	@grep "^\\\\citation" *.aux > .btmp.new || true

# If the citations are not changed, don't do anything. Otherwise replace
# the .btmp file to make sure Bibtex will be run.
	@if ( diff .btmp.new .btmp >& /dev/null ); then \
		rm .btmp.new; \
	else \
		mv .btmp.new .btmp; \
	fi

	@if [ -f $*.idx ]; then cp $*.idx .itmp.new; else touch .itmp.new; fi
	@if ( diff .itmp.new .itmp >& /dev/null ); then \
		rm .itmp.new; \
	else \
		mv .itmp.new .itmp; \
	fi

.btmp:

%.bbl: $(BIBFILES) .btmp
# Only use BibTeX if \bibliography occurs in the document. In that case,
# run BibTeX and recompile. .btmp is touched to prevent useless making
# next time.
	@if ( grep "^\\\\bibliography{" $*.tex > /dev/null ); then \
		$(BIBTEX) $*; \
		touch .rerun; \
	fi
	@touch .btmp

.itmp:

%.ind: .itmp
	@if [ -f $*.idx ]; then \
		$(MAKEINDEX) $*; \
		touch .rerun; \
		touch .itmp; \
	fi

%.eps:%.fig
	@echo Generating figure $@...
	@fig2dev -L ps $< $@

%.dvi: %.aux %.ind %.bbl
# Make sure the dvi-file exists; if not: recompile.
	@if [ ! -f $*.dvi ]; then \
		touch .rerun; \
	fi

	@if [ -f .rerun ]; then \
		rm .rerun; \
		$(LATEX) $*; \
	else \
		$(MAKE) $*.aux; \
	fi

# While references et al. are changed: recompile.
	@while ( grep Rerun $*.log > /dev/null ); do \
		$(LATEX) $*; \
	done

# Touch the figureobjects to prevent making next time
	@if [ -n "$(FIGUREOBJS)" ]; then \
		touch $(FIGUREOBJS); \
		touch $*.aux; \
	fi

	@if [ -f $*.ind ]; then \
		touch $*.ind; \
	fi
	@$(MAKEINDEX) -s nomencl.ist -o $*.gls $*.glo

latex:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

latexfigures:
	@for i in $(FIGUREOBJS); do \
		$(MAKE) $$i; \
	done

view:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi && \
		$(DVIVIEWER) ${LATEXTARGET}.dvi ; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi && \
			$(DVIVIEWER) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi && \
			$(DVIVIEWER) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

%.ps: %.dvi
	$(DVIPS) -o $*.ps $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(DVIPS) -o $*.ps $<

%.pdf: %.tex
	$(PDFLATEX) $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(PDFLATEX) $<
	$(PDFLATEX) $<

latexps:
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.ps && \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.ps && \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.ps && \
			true; \
		fi; \
	fi

html: .html

.html:
	@if [ -n "${LATEXTARGET}" ]; then \
		if [ -n "${HTMLDIR}" ]; then \
			$(MAKE) ${LATEXTARGET}.dvi; \
			$(LATEX2HTML) $(LATEX2HTML_OPTS) -dir $(HTMLDIR)/$(LATEXTARGET) $(LATEXTARGET) && \
			chmod a+rx $(HTMLDIR)/$(LATEXTARGET) && \
			chmod a+r $(HTMLDIR)/$(LATEXTARGET)/* &&  \
			touch .html; \
		else \
			echo Set variable HTMLDIR\!; \
		fi; \
	else \
		echo Set variable LATEXTARGET\!; \
	fi

latexhelp:
	@echo "LaTeX Makefile Options"
	@echo "----------------------"
	@echo ""
	@echo "Environment variables:"
	@echo "  LATEXTARGET   Filename to make (without extension)"
	@echo "  HTMLDIR       Directory for HTML-output"
	@echo "  FIGURES       Figures that have to be compiled"
	@echo ""
	@echo "Targets:"
	@echo "  all           Make the LATEXTARGET or <dirname>.dvi"
	@echo "  <name>.dvi    Make the given dvi file"
	@echo "  latex         Make the LATEXTARGET or <dirname>.dvi"
	@echo "  view          Make and view the LATEXTARGET or <dirname>.dvi"
	@echo "  html          Make the LATEXTARGET  or <dirname>.dvi and generate HTML output"
	@echo "  latexhelp     This overview"
	@echo "  latexclean    Remove all generated files"

clean latexclean::
	@rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.out *.brf *.html *.btmp *.itmp *.rerun *.glo *.gls
	@epsfiles=`find * -name "*.eps" -maxdepth 0`; \
	if [ -n "$$epsfiles" ]; then \
		for i in *.eps; do \
			if [ -f `basename $$i .eps`.fig ]; then \
				rm -f $$i; \
			elif ( rcs `basename $$i .eps`.fig >& /dev/null ); then \
				rm -f $$i; \
			fi \
		done \
	fi

cleanpspdf : clean
	@rm -f *.ps *.pdf

clobber : cleanpspdf
	@rm -f *~


==> _ <==
\section{Gap stability in 3D}\label{3d_stability}
The substantial cost of a 3D numerical calculation prevent extensive
parameter studies. Instead, described below are specific simulations
on gap stability. The general numerical setup is as follows. 

The disc is divided into $N_r\times
N_\theta \times N_\phi$ zones in the $(r,\theta,\phi)$ directions,
uniformly spaced in $(\theta,\phi)$
and logarithmically spaced in $r$. During $t\leq t_0 \equiv 10P_0$ the
disc is evolved without the planet. 
Between $t_0 \leq t \leq 2t_0$, the planet mass is switched on.
If the disc is self-gravitating then for $0 \leq t \leq t_0$, 
$(\lmax, \mmax)=(48,0)$ is set for the boundary potential and $g_\theta$ is smoothly switched on. 
For $t>t_0$, $(\lmax, \mmax)=(16,10)$ is set for the boundary potential. 
Hydrodynamic boundary conditions are
outflow in radius, reflecting in $\theta$ and periodic in $\phi$.  


\subsection{Vortex instability in a non-self-gravitating
  disc}\label{3dvortex} 
In this simulation the disc model is $Q_o=4$. The domain is 
$r\in[1,10]$ and $n_H=2$ scale-heights above and below the
midplane.  The resolution is
$(N_r, N_\theta, N_\phi) = (256,64,696)$, corresponding to $16$ cells
per $H$ in $\theta$, but only $\simeq 5.6$ cells per $H$ in $r$ and
$\phi$. The planet mass is $M_p = 3\times10^{-4} M_*$ and is fixed
in the midplane at radius $r_{p}=5$ after its introduction. The EOS parameter is
$h_p=0.7$. 

Fig. \ref{ch5_vortex2} show density perturbations
relative to the azimuthally-averaged density field at $t=10P_0$. Two
cuts in $\theta$ are shown, corresponding to the midplane and at
$z=2H$. The vortex instability clearly persists for planetary gaps in 
a three-dimensional disc. The relative density pertubation has no
vertical dependence (except near the planet since it is
embedded). This is also seen in the three-dimensional plot in
Fig. \ref{ch5_vortex2_3d}. Since the background density is essentially
Gaussian in $z$, the vortex density field will also be Gaussian
vertically. 



%\begin{landscape}
  \begin{figure}
    \centering
    \includegraphics[scale=.31,clip=true,trim=0.74cm 0.64cm 2.08cm 
    0cm]{figures/vortex2_polar_dens010_z0}\includegraphics[scale=.31,clip=true,trim=0.74cm
    0.64cm 2.08cm 
    0cm]{figures/vortex2_polar_dens012_z0}\includegraphics[scale=.31,clip=true,trim=0.74cm   
    0.64cm 2.08cm
    0cm]{figures/vortex2_polar_dens016_z0}\includegraphics[scale=.31,clip=true,trim=0.74cm  
    0.64cm 0cm 0cm]{figures/vortex2_polar_dens020_z0}\\
    \includegraphics[scale=.31,clip=true,trim=0.74cm 0.64cm 2.08cm 
    0cm]{figures/vortex2_polar_dens010_2h}\includegraphics[scale=.31,clip=true,trim=0.74cm
    0.64cm 2.08cm 
    0cm]{figures/vortex2_polar_dens012_2h}\includegraphics[scale=.31,clip=true,trim=0.74cm   
    0.64cm 2.08cm
    0cm]{figures/vortex2_polar_dens016_2h}\includegraphics[scale=.31,clip=true,trim=0.74cm  
    0.64cm 0cm 0cm]{figures/vortex2_polar_dens020_2h}
    \caption{Relative density perturbation near the midplane (top) and 
      near $z=2H$ (bottom).    
    \label{ch5_vortex2}}
\end{figure}
%\end{landscape}


\begin{figure}
    \centering
    \includegraphics[scale=.33]{figures/vortex2_polar_dens016_3d}
    \caption{Three-dimensional visualisation of the vortex
      instability at $t=80P_0$. The colourbar is relative density
      perturbation. 
    \label{ch5_vortex2_3d}}
\end{figure}

The evolution is very similar to 2D discs simulated in Chapter
\ref{paper1}---\ref{paper2}. The only noticeable difference is that in 2D without
self-gravity, 3 vortices develop initially then merge
(Fig. \ref{vortices_sg_nsg}). In the 3D run,  one vortex develops from
the beginning (although a weak, second vortex can be identified
in Fig. \ref{ch5_vortex2} at $t=60P_0$). A similar observation was
made by \cite{meheut10}. However, in quasi-steady state the vortex in
3D and 2D are essentially identical.  
%A snapshot of the 2D run in quasi-steady
%state is shown in Fig. \ref{ch5_vortex2_v1NSG_2d}, and is essentially
%identical to the 3D run. 
These results show that the vortex instability is a 2D instability and
. Thus, the condition for
instability can be largely determined by vertically integrated
properties of the disc. 

%a snapshot
%of which is shown in . 

% \begin{figure}
%     \centering
%     \includegraphics[scale=.5,clip=true,trim=0.74cm  
%     0.64cm 0cm 0cm]{figures/v1NSG_polar_dens041_2d}
%     \caption{Relative surface density perturbation of a 2D
%       non-self-gravitating simulation, showing the quasi-steady state
%       of the vortex instability at a planetary gap. 
%     \label{ch5_vortex2_v1NSG_2d}}
% \end{figure}

%some plots of vertical cuts

The vortex vertical structure is shown in Fig. \ref{ch5_vert_cut}. 
The vortex lies just outside the outer gap edge at $R\simeq 5.6$. Its
associated relative density and vortensity perturbations have very
weak vertical dependence, despite the background being
Gaussian. Stratification has no effect on the instability. 

%The relative
%density perturbation has little vertical dependence, and although the
%vortensity perturbation is 

%slightly larger near $\pm 2H$,
%its vertical variation is still weak.  

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    1.0cm 0cm 0cm]{figures/vortex2_polarRZ_dens016}\\
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    0.0cm 0cm 0.99cm]{figures/vortex2_vortRZ_016} 
    \caption{Relative perturbation of density (top) and
      vertical vortensity $\eta/\rho$ (bottom) in a meridional plane
      through the vortex at $R\in[5.6,6.7]$ (white contour lines).  
    \label{ch5_vert_cut}}
\end{figure}

The mass flux $\rho\bm{u}$ of the main vortex at
$t=80P_0$ is drawn in Fig. \ref{ch5_stream} for several meridional
planes. 
As expected for an anticyclonic vortex, the radial flow
transits from inwards to outwards as one traverses 
anti-clockwise (increasing $\phi $) through the vortex. The transition
point is the vortex centroid. The
$\phi/2\pi=0.45$ slice shows that the transition involves
vertical flux, but its magnitude is small even near the midplane,
where the mass density is largest. This means the vortex
centroid has very little motion. There is no evidence for strong
convection rolls found by \cite{meheut10}, but the flow towards the
midplane highlighted in Fig. \ref{ch5_stream} suggest vertical motion
near the vortex centroid, 
%may correspond to the
%vertical flow 
which was also seen in \citeauthor{meheut10}. Note that symmetry about
$z=0$ is broken, so mass flux can overshoot across the
midplane.       

%non symmetric about z=0
%possible downwelling? but no convection rolls

%\begin{landscape}
\begin{figure}[!ht]
  \centering
  \includegraphics[scale=.55,clip=true,trim=0.0cm 1.0cm 1.68cm
  0cm]{figures/vortex2_stream_016_d33}\includegraphics[scale=.55,clip=true,trim=1.7cm 1.0cm 1.68cm 0cm]{figures/vortex2_stream_016_d41}\\
  \includegraphics[scale=.55,clip=true,trim=0.0cm 1.0cm 1.68cm
  0cm]{figures/vortex2_stream_016_d44}\includegraphics[scale=.55,clip=true,trim=3.6cm
  13.7cm 5.33cm 6.5cm]{figures/vortex2_stream_016_d45_circ}\\
  \includegraphics[scale=.55,clip=true,trim=0.0cm 0.0cm 1.68cm 0cm]{figures/vortex2_stream_016_d47}\includegraphics[scale=.55,clip=true,trim=1.7cm 0.0cm 1.68cm 0cm]{figures/vortex2_stream_016_d50}
  \caption{Meridional flow in vertical planes through the
    vortex. Velocity vectors have been scaled by the local
    density.  The vertical velocity has also been
    divided by $H$. The circled region highlights flux towards the
    midplane near the vortex centroid. 
    \label{ch5_stream}}
\end{figure}
% \end{landscape}

%Three simulations were run. In all cases the disc has $Q_0=4$ and occupy
%$r\in[1,10]$.Two cases include the full
%vertical extent of $n_H=2$ scale-heights above and below the midplane,
%one where the planet is allowed to migrate from $t=50P_0$ and the
%other from $t=100P_0$. The third case only simulates the upper $n_H=2$
%scale-heights, and the planet is released at $t=50P_0$ but confined in   
%the midplane. 

\subsection{Vortex-planet interaction}
  
Fig. \ref{ch5_orbit3_nsg} shows the planet orbital radius after
it is released at $t=100P_0$ for the simulation in
\S\ref{3d_stability}. Also shown is a second simulation where only
$z>0$ was simulated and the planet released at $t=50P_0$, before vortices fully
develop . Results are very similar to 2D, the migration 
composing of slow and rapid phases, the latter induced by the vortex
associated with the inner gap edge. Since the interaction is gravitational,
and the perturbed density field associated with the vortex 
has no vertical structure, one expects the same interaction in
3D as in 2D. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/orbit3_rp_nsg}
    \caption{Vortex-induced migration of a Saturn-mass planet in 3D
      discs. The run `full z' simulates the entire disc and
      `half z' only simulates the upper plane ($z>0$). 
    \label{ch5_orbit3_nsg}}
\end{figure}

%weaker interaction because disc density is diluted vertically
%
%

\subsection{Vortex modes with self-gravity}
For 3D self-gravitating simulations, the computational domain is 
$r\in[1,25]$ and $0 \leq z \leq 2H$. For simulations in this
subsection, the resolution is $(N_r,
N_\theta, N_\phi)=(256, 32, 512)$.  Jovian planets
are used to open the gap because the steeper
edges imply higher growth rates than gaps opened by a Saturn-mass
planet, shortening the simulation time. The planet is fixed at
$r_{p0}=10$ and simulated upto $t=50P_0$. The EOS parameter is
$h_p=0.5$. 

Fig. \ref{ch5_vortex5_vortex6} compares vortex formation in the
$Q_o=3,\,4,\,8$ disc models, with $M_p=0.001M_*$. 
It confirms the effect of
self-gravity on the vortex instability discussed in Chapter
\ref{paper2}, persists in 3D. Comparing the outer gap edge at
$t=30P_0$ shows self-gravity is stabilising, because in $Q_o=8$
vortices can already be identified and not so readily seen in
$Q_o=4$. At $t=40P_0$, more vortices develop with lowering $Q_o$
because stabilisation is more effective for low $m$, thus higher $m$
vortex modes are favoured, just as in 2D. 
The 6-vortex and 5-vortex configuration remains
in $Q_o=3,\,4$, respectively, at $t=50P_0$ whereas only 3 remain in
$Q_o=8$ (reduced from 4). This is due to resisted merging as vortices
behave like co-orbital planets with increasing self-gravity. Again,
this was seen in 2D. 


%stabilisation
%more vortices 
%merging

%vertical cuts

The vortex vertical structure for $Q_o=4$ is shown in
Fig. \ref{ch5_vortex5_vert_cut}. Because the initial disc is not in
self-gravitating equilibrium, density perturbations relative to $t=0$
and to $t=10P_0$ (just after $g_\theta$ is fully switched on) are both
shown. The increasing perturbation towards the midplane is partly due
to the background vertical self-gravity. 
%Without starting with exact
%equilbrium, it is unclear how much of the vertical vortex structure is
%due to relaxation towards equilibrium, or due to the linear
%instability. 
Stratification is reduced if the perturbation is 
taken relative to $t=10P_0$, so the instability tends to involve
the entire column of fluid. 
Between $t=10P_0$ and $t=50P_0$ there may also be additional
stratification due to vertical self-gravity of the vortex, since the
midplane density is largest.% and
%its central over-density is $\sim 3$ times larger than the
%non-self-gravitating vortex. 
%even if vortex instablity gives no vertical dependece in terms of
%relative perturbations, eventually get stratification

The vortensity field in Fig. \ref{ch5_vortex5_vert_cut}  show
disturbances along contour lines at the vortex boundary, and 
closed contours within the vortex, which is associated with
anti-clockwise motion indicated by mass flux vectors in 
Fig. \ref{ch5_vortex5_stream}. This is suggestive of the convection
rolls described by \cite{meheut10}, but they found the roll
occur in pairs. It is likely the convective flow found here has been
modified by self-gravity of the vortex and/or background.  
However, despite additional vertical structure and flow, the
vortensity perturbation remains largely columnar.    

% and the
%computational domain corresponds to more than $2H$
%The
%vertical structure is reduced but not removed  

\begin{figure}[!ht]
  \centering
 \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
  0cm]{figures/vortex7_polar_dens006}\includegraphics[scale=.4,clip=true,trim=.85cm
  0.64cm 2.2cm 
  0cm]{figures/vortex7_polar_dens008}\includegraphics[scale=.4,clip=true,trim=.85cm   
  0.64cm 0.0cm
  0cm]{figures/vortex7_polar_dens010}\\
  \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
  0.69cm]{figures/vortex5_polar_dens006}\includegraphics[scale=.4,clip=true,trim=.85cm
  0.64cm 2.2cm 
  0.69cm]{figures/vortex5_polar_dens008}\includegraphics[scale=.4,clip=true,trim=.85cm   
  0.64cm 0.0cm
  0.69cm]{figures/vortex5_polar_dens010}\\
  \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
  0.69cm]{figures/vortex6_polar_dens006}\includegraphics[scale=.4,clip=true,trim=.85cm
  0.64cm 2.2cm 
  0.69cm]{figures/vortex6_polar_dens008}\includegraphics[scale=.4,clip=true,trim=.85cm   
  0.64cm 0.00cm
  0.69cm]{figures/vortex6_polar_dens010} 
  \caption{Vortex instability in self-gravitating
    3D disc models $Q_o=3$ (top), $Q_o=4$ (middle) and $Q_o=8$
    (bottom). The relative 
    density perturbation near the midplane is shown. 
    \label{ch5_vortex5_vortex6}}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    1.cm 0cm 0cm]{figures/vortex5_polarRZ_dens010_t0}\\
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    1.cm 0cm 0.99cm]{figures/vortex5_polarRZ_dens010_t10} \\
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    0.0cm 0cm 0.99cm]{figures/vortex5_vortRZ_010}
    \caption{Density perturbation relative to $t=0$ (top), to
      $t=10P_0$ (middle), and the vertical vortensity
      perturbation relative to $t=10P_0$ (bottom) in a plane 
      through the vortex, highlighted by white contour lines.   The
      disc model is $Q_o=4$ with self-gravity. 
    \label{ch5_vortex5_vert_cut}}
\end{figure}


\begin{figure}[!ht]
  \centering
  \includegraphics[scale=.67,clip=true,trim=2.4cm
  12.8cm 5.33cm 6.5cm]{figures/vortex5_stream_010}
  \caption{Mass flux corresponding to 
    Fig. \ref{ch5_vortex5_vert_cut}. 
    \label{ch5_vortex5_stream}}
\end{figure}


\subsection{Edge modes} %one simulation
The disc model $Q_o=1.5$ is used to demonstrate edge modes. 
The resolution is increased to $(N_r,
N_\theta, N_\phi) = (256,64,516)$, on account of 
reduction in effective scale-height due to vertical self-gravity.  

Fig. \ref{ch5_edge1HR} shows the development of an $m=2$ edge mode 
and Fig. \ref{ch5_edge1HR_3d} is a three-dimensional
visualisation. Perturbations are calculated relative to $t=10P_0$.   
The behaviour near the midplane is similar to 2D 
simulations. The edge mode amplitude decreases away from the 
midplane. The background density ($t=10P_0$) near $z=2H$ has been
reduced by vertical self-gravity from $t=0$. This means that perturbations high in
the atmosphere, including disturbances in addition to edge modes, appear
enhanced, but their actual densities are small compared to the
midplane. 

%Near $z=2H$, the disturbance densities,
%including those in addition to edge modes, are small compared to the
%midplane. 
%Structure in addition to the edge mode can be identified 
%near $z=2H$. The background density is
%lowered by vertical self-gravity, so disturbances high in the
%atmosphere 
%The actual densities at $z>H$ is small compared to the midplane so
%disturbances at such heights are not expected to affect the edge
%mode evolution. 

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
  0cm]{figures/edge1HR_polar_dens006_z0}\includegraphics[scale=.4,clip=true,trim=.85cm
  0.64cm 2.2cm 
  0cm]{figures/edge1HR_polar_dens008_z0}\includegraphics[scale=.4,clip=true,trim=.85cm   
  0.64cm 0.0cm
  0cm]{figures/edge1HR_polar_dens010_z0}\\
%   \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
%   0.cm]{figures/edge1HR_polar_dens006_1d5h}\includegraphics[scale=.4,clip=true,trim=.85cm
%   0.64cm 2.2cm 
%   0.cm]{figures/edge1HR_polar_dens008_1d5h}\includegraphics[scale=.4,clip=true,trim=.85cm   
%   0.64cm 0.00cm
%   0.cm]{figures/edge1HR_polar_dens010_1d5h}\\
  \includegraphics[scale=.4,clip=true,trim=.85cm 0.64cm 2.2cm 
  0.cm]{figures/edge1HR_polar_dens006_2h}\includegraphics[scale=.4,clip=true,trim=.85cm
  0.64cm 2.2cm 
  0.cm]{figures/edge1HR_polar_dens008_2h}\includegraphics[scale=.4,clip=true,trim=.85cm   
  0.64cm 0.00cm
  0.cm]{figures/edge1HR_polar_dens010_2h}
  \caption{Edge mode in the 3D disc model $Q_o=1.5$. The density
    perturbation relative to $t=10P_0$ is shown near the midplane
    (top) and $z=2H$ (bottom).  
    \label{ch5_edge1HR}}
\end{figure}

 
\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.33,clip=true,trim=0cm 1.5cm 0cm
    3cm]{figures/edge1HR_polar_dens007_3d.ps} 
    \caption{Three-dimensional visualisation the edge mode instability
      for the simulation in Fig. \ref{ch5_edge1HR}. The snapshot is
      $t=35P_0$. One of the edge mode spiral arms coincide with the
      planetary wake. The colourbar is relative density
      perturbation. 
    \label{ch5_edge1HR_3d}}
\end{figure}

%vertical cuts

Fig. \ref{ch5_edge1HR_vert_cut}---\ref{ch5_edge1HR_stream} shows the
vertical structure of the edge mode near the gap edge. 
The density 
perturbation is even more stratified than a self-gravitating vortex 
. Most of the edge mode is contained within $z<H$ and the
corresponding vortensity perturbation is no longer columnar.  
Mass flux goes into the over-density radially from either side, as well
as vertically from above. The vertical flux is likely attributable 
to both instability and vertical
self-gravity. Note that the background vortensity increases with $z$
because of stratification. Thus downwards advection 
brings high vortensity material towards lower vortensity material. 
This may be related to convective motion in
Fig. \ref{ch5_edge1HR_stream}. 



\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    1.cm 0cm 0cm]{figures/edge1HR_polarRZ_dens007_t0}\\
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    1.cm 0cm 0.99cm]{figures/edge1HR_polarRZ_dens007_t10} \\
    \includegraphics[scale=.67,clip=true,trim=0.0cm  
    0.0cm 0cm 0.99cm]{figures/edge1HR_vortRZ_007}
    \caption{Density perturbation relative to $t=0$ (top), to
      $t=10P_0$ (middle), and the vertical vortensity
      perturbation relative to $t=10P_0$ (bottom) in a vertical plane
      through the edge mode in Fig. \ref{ch5_edge1HR_3d}.% Note the
%      abscence of the high vortensity ring as edge modes destroy
%      them. 
    \label{ch5_edge1HR_vert_cut}}
\end{figure}



\begin{figure}[!ht]
  \centering
  \includegraphics[scale=.67]{figures/edge1HR_stream_007}
  \caption{Mass flux corresponding to 
    Fig. \ref{ch5_edge1HR_vert_cut}. Note the vertical axis covers
    $z<H$. 
    \label{ch5_edge1HR_stream}}
\end{figure}


\subsection{Outwards migration induced by edge modes} % one simulation
This simulation is the 3D version of the fiducial case in Chapter
\ref{edge_migration}. The disc model is $Q_o=1.7$ and the resolution
is $(N_r,N_\theta,N_\phi) = (256,32,512)$. $N_\theta$ is
reduced to enable longer simulation times. The planet mass is now $M_p =
0.002M_*$ and it is allowed to migrate for $t>20P_0$. 
Since co-rotational torques were 
found to be important inthe 2D simulations, the torque cut-off
parameter is reduced to $\epsilon_c=0.5$ (about 3.5 cells). 

Fig. \ref{ch5_edge2_migration} and Fig. \ref{ch5_edge2_migration}  shows 
the migration history and snapshots of
 density perturbation. These figures can be compared to the 2D
case, Fig. \ref{ch4_Q1d7_migration}---\ref{ch4_Q1d7_polarxy}. Whereas
the 2D disc developed $m=2$--3  edge modes, only $m=2$ was seen in
3D. This could be due to the much reduced resolution in 3D (by a
factor of 4 in $r$ and $\phi$ compared to 2D), or reduction in the
strength of self-gravity due to disc thickness. 

Despite the poor resolution,  this simulation demonstrates edge
modes can induce outwards migration in 3D discs. Outwards migration
only begins around $t=70P_0$, whereas it starts immediately in the 2D
run. The migration in 3D is also on average slower than in 2D.  
These are probably because of applied torque tapering (for  
numerical considerations). However, because the existence of edge
modes does not depend on treatment close to the planet, their
development will bring material to the planet for interaction. This is
shown in Fig. \ref{ch5_edge2_polarxy}, which is qualitatively very
similar to the 2D run. The planet is asymmetrically positioned with
respect to gap edges, and edge mode spiral arms protrude the gap,
providing a positive torque as it passes by. 


\begin{figure}
  \centering
  \includegraphics[scale=.67]{figures/edge2_orbit_ae}
  \caption{Keplerian semi-major axis $a$ and eccentricity $e$ for
    planet ($M_p=0.002M_*$) in the $Q_o=1.7$ three-dimensional disc model. 
    \label{ch5_edge2_migration}}
\end{figure}


\begin{figure} 
  \centering
  \includegraphics[scale=.5,clip=true,trim=0cm 0cm 1.7cm
  0cm]{figures/edge2_polarxy_dens020_z0}\includegraphics[scale=.5,clip=true,trim=2.21cm 0cm 1.7cm
  0cm]{figures/edge2_polarxy_dens020_h}\includegraphics[scale=.5,clip=true,trim=2.21cm 0cm 0.0cm
  0cm]{figures/edge2_polarxy_dens020_2h}  
  \caption{Logarithmic density perturbation
    $\log{\left[\rho/\rho(t=10P_0)\right]}$ at three heights, during
    outwards  migration of a planet induced by edge modes in a 3D disc. 
  \label{ch5_edge2_polarxy}}
\end{figure}

